High Pressure Phase Diagram of Beryllium from \emph{Ab Initio} Free Energy Calculations

We use first principles molecular dynamics simulations coupled to the thermodynamic integration method to study the hcp-bcc transition and melting of beryllium up to a pressure of 1600~GPa. We derive the melting line by equating solid and liquid Gibbs free energies, and represent it by a Simon Glatzel fit $T_m= 1564~\text{K} (1 + P/(15.6032 ~\text{GPa}))^{0.383}$, which is in good agreement with previous two-phase simulations below 6000~K. We also derive the hcp-bcc solid-solid phase boundary and show the quasiharmonic approximation underestimates the stability of the hcp structure, predicting lower transition pressures between hcp and bcc phases. However, our results are consistent with the stability regime predicted by the phonon quasiparticle method. We also predict that hcp-bcc-liquid triple point is located at 164.7~GPa and 4314~K. In addition, we compute the shock Hugoniot curve, and show that it is in good agreement with experiments, intersecting our derived melting curve at $\sim$235~GPa at 4900~K. Finally, we show that an isentropic compression path that intersects the melting curve at both low and high temperature in the liquid regime, can reappear in the solid after a gap as large as 7000~K. Therefore, we predict that a large section of the melting curve could be sampled, in principle, by a ramp compression experiment, where solid and liquid Be would coexist as the sample is compressed.

==> Ab_Initio Simulation of Beryllium under high pressures_Submit/tmp <==
@article{Kline2016,
abstract = {The first indirect drive implosion experiments using Beryllium (Be) capsules at the National Ignition Facility confirm the superior ablation properties and elucidate possible Be-ablator issues such as hohlraum filling by ablator material. Since the 1990s, Be has been the preferred Inertial Confinement Fusion (ICF) ablator because of its higher mass ablation rate compared to that of carbon-based ablators. This enables ICF target designs with higher implosion velocities at lower radiation temperatures and improved hydrodynamic stability through greater ablative stabilization. Recent experiments to demonstrate the viability of Be ablator target designs measured the backscattered laser energy, capsule implosion velocity, core implosion shape from self-emission, and in-flight capsule shape from backlit imaging. The laser backscatter is similar to that from comparable plastic (CH) targets under the same hohlraum conditions. Implosion velocity measurements from backlit streaked radiography show that laser energy coupling to the hohlraum wall is comparable to plastic ablators. The measured implosion shape indicates no significant reduction of laser energy from the inner laser cone beams reaching the hohlraum wall as compared with plastic and high-density carbon ablators. These results indicate that the high mass ablation rate for beryllium capsules does not significantly alter hohlraum energetics. In addition, these data, together with data for low fill-density hohlraum performance, indicate that laser power multipliers, required to reconcile simulations with experimental observations, are likely due to our limited understanding of the hohlraum rather than the capsule physics since similar multipliers are needed for both Be and CH capsules as seen in experiments.},
author = {Kline, J. L. and Yi, S. A. and Simakov, A. N. and Olson, R. E. and Wilson, D. C. and Kyrala, G. A. and Perry, T. S. and Batha, S. H. and Zylstra, A. B. and Dewald, E. L. and Tommasini, R. and Ralph, J. E. and Strozzi, D. J. and MacPhee, A. G. and Callahan, D. A. and Hinkel, D. E. and Hurricane, O. A. and Milovich, J. L. and Rygg, J. R. and Khan, S. F. and Haan, S. W. and Celliers, P. M. and Clark, D. S. and Hammel, B. A. and Kozioziemski, B. and Schneider, M. B. and Marinak, M. M. and Rinderknecht, H. G. and Robey, H. F. and Salmonson, J. D. and Patel, P. K. and Ma, T. and Edwards, M. J. and Stadermann, M. and Baxamusa, S. and Alford, C. and Wang, M. and Nikroo, A. and Rice, N. and Hoover, D. and Youngblood, K. P. and Xu, H. and Huang, H. and Sio, H.},
doi = {10.1063/1.4948277},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.4948277.pdf:pdf},
issn = {10897674},
journal = {Physics of Plasmas},
number = {5},
title = {{First beryllium capsule implosions on the National Ignition Facility}},
volume = {23},
year = {2016}
}
@article{Clark2018,
abstract = {Indirect drive implosion experiments on the National Ignition Facility (NIF) [E. I. Moses et al., Phys. Plasmas 16, 041006 (2009)] have now tested three different ablator materials: glow discharge polymer plastic, high density carbon, and beryllium. How do these different ablators compare in current and proposed implosion experiments on NIF? What are the relative advantages and disadvantages of each? This paper compares these different ablator options in capsule-only simulations of current NIF experiments and potential future designs. The simulations compare the impact of the capsule fill tube, support tent, and interface surface roughness for each case, as well as all perturbations in combination. According to the simulations, each ablator is impacted by the various perturbation sources differently, and each material poses unique challenges in the pursuit of ignition on NIF.},
author = {Clark, D. S. and Kritcher, A. L. and Yi, S. A. and Zylstra, A. B. and Haan, S. W. and Weber, C. R.},
doi = {10.1063/1.5016874},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.5016874.pdf:pdf},
issn = {10897674},
journal = {Physics of Plasmas},
number = {3},
title = {{Capsule physics comparison of National Ignition Facility implosion designs using plastic, high density carbon, and beryllium ablators}},
volume = {25},
year = {2018}
}
@article{Haan2011,
abstract = {Point design targets have been specified for the initial ignition campaign on the National Ignition Facility G. H. Miller, E. I. Moses, and C. R. Wuest, Opt. Eng. 443, 2841 (2004). The targets contain D-T fusion fuel in an ablator of either CH with Ge doping, or Be with Cu. These shells are imploded in a U or Au hohlraum with a peak radiation temperature set between 270 and 300 eV. Considerations determining the point design include laser-plasma interactions, hydrodynamic instabilities, laser operations, and target fabrication. Simulations were used to evaluate choices, and to define requirements and specifications. Simulation techniques and their experimental validation are summarized. Simulations were used to estimate the sensitivity of target performance to uncertainties and variations in experimental conditions. A formalism is described that evaluates margin for ignition, summarized in a parameter the Ignition Threshold Factor (ITF). Uncertainty and shot-to-shot variability in ITF are evaluated, and sensitivity of the margin to characteristics of the experiment. The formalism is used to estimate probability of ignition. The ignition experiment will be preceded with an experimental campaign that determines features of the design that cannot be defined with simulations alone. The requirements for this campaign are summarized. Requirements are summarized for the laser and target fabrication. {\textcopyright} 2011 American Institute of Physics.},
author = {Haan, S. W. and Lindl, J. D. and Callahan, D. A. and Clark, D. S. and Salmonson, J. D. and Hammel, B. A. and Atherton, L. J. and Cook, R. C. and Edwards, M. J. and Glenzer, S. and Hamza, A. V. and Hatchett, S. P. and Herrmann, M. C. and Hinkel, D. E. and Ho, D. D. and Huang, H. and Jones, O. S. and Kline, J. and Kyrala, G. and Landen, O. L. and MacGowan, B. J. and Marinak, M. M. and Meyerhofer, D. D. and Milovich, J. L. and Moreno, K. A. and Moses, E. I. and Munro, D. H. and Nikroo, A. and Olson, R. E. and Peterson, K. and Pollaine, S. M. and Ralph, J. E. and Robey, H. F. and Spears, B. K. and Springer, P. T. and Suter, L. J. and Thomas, C. A. and Town, R. P. and Vesey, R. and Weber, S. V. and Wilkens, H. L. and Wilson, D. C.},
doi = {10.1063/1.3592169},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.3592169.pdf:pdf},
issn = {1070664X},
journal = {Physics of Plasmas},
number = {5},
title = {{Point design targets, specifications, and requirements for the 2010 ignition campaign on the National Ignition Facility}},
volume = {18},
year = {2011}
}
@article{Clark2008,
abstract = {Inertial confinement fusion capsules are critically dependent on the integrity of their hot spots to ignite. At the time of ignition, only a certain fractional perturbation of the nominally spherical hot spot boundary can be tolerated and the capsule still achieve ignition. The degree to which the expected hot spot perturbation in any given capsule design is less than this maximum tolerable perturbation is a measure of the ignition margin or robustness of that design. Moreover, since there will inevitably be uncertainties in the initial character and implosion dynamics of any given capsule, all of which can contribute to the eventual hot spot perturbation, quantifying the robustness of that capsule against a range of parameter variations is an important consideration in the capsule design. Here, the robustness of the 300 eV indirect drive target design for the National Ignition Facility [Lindl, Phys. Plasmas 11, 339 (2004)] is studied in the parameter space of inner ice roughness, implosion velocity, and capsule scale. A suite of 2000 two-dimensional simulations, run with the radiation hydrodynamics code LASNEX, is used as the data base for the study. For each scale, an ignition region in the two remaining variables is identified and the ignition cliff is mapped. In accordance with the theoretical arguments of Levedahl and Lindl [Nucl. Fusion 37, 165 (1997)] and Kishony and Shvarts [Phys. Plasmas 8, 4925 (2001)], the location of this cliff is fitted to a power law of the capsule implosion velocity and scale. It is found that the cliff can be quite well represented in this power law form, and, using this scaling law, an assessment of the overall (one- and two-dimensional) ignition margin of the design can be made. The effect on the ignition margin of an increase or decrease in the density of the target fill gas is also assessed. {\textcopyright} 2008 American Institute of Physics.},
author = {Clark, Daniel S. and Haan, Steven W. and Salmonson, Jay D.},
doi = {10.1063/1.2890123},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.2890123.pdf:pdf},
issn = {1070664X},
journal = {Physics of Plasmas},
number = {5},
title = {{Robustness studies of ignition targets for the National Ignition Facility in two dimensions}},
volume = {15},
year = {2008}
}
@article{Simakov2014,
abstract = {For indirect drive inertial confinement fusion, Beryllium (Be) ablators offer a number of important advantages as compared with other ablator materials, e.g., plastic and high density carbon. In particular, the low opacity and relatively high density of Be lead to higher rocket efficiencies giving a higher fuel implosion velocity for a given X-ray drive; and to higher ablation velocities providing more ablative stabilization and reducing the effect of hydrodynamic instabilities on the implosion performance. Be ablator advantages provide a larger target design optimization space and can significantly improve the National Ignition Facility (NIF) [J. D. Lindl et al., Phys. Plasmas 11, 339 (2004)] ignition margin. Herein, we summarize the Be advantages, briefly review NIF Be target history, and present a modern, optimized, low adiabat, Revision 6 NIF Be target design. This design takes advantage of knowledge gained from recent NIF experiments, including more realistic levels of laser-plasma energy backscatter, degraded hohlraum-capsule coupling, and the presence of cross-beam energy transfer. {\textcopyright} 2014 AIP Publishing LLC.},
author = {Simakov, Andrei N. and Wilson, Douglas C. and Yi, Sunghwan A. and Kline, John L. and Clark, Daniel S. and Milovich, Jose L. and Salmonson, Jay D. and Batha, Steven H.},
doi = {10.1063/1.4864331},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/1.4864331.pdf:pdf},
issn = {1070664X},
journal = {Physics of Plasmas},
number = {2},
title = {{Optimized beryllium target design for indirectly driven inertial confinement fusion experiments on the national ignition facility}},
volume = {21},
year = {2014}
}
@article{Benedict2009,
author = {Benedict, Lorin X. and Ogitsu, Tadashi and Trave, Andrea and Wu, Christine J. and Sterne, Philip A. and Schwegler, Eric},
doi = {10.1103/PhysRevB.79.064106},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
mendeley-groups = {Beryllium},
number = {6},
pages = {1--9},
title = {{Calculations of high-pressure properties of beryllium: Construction of a multiphase equation of state}},
volume = {79},
year = {2009}
}

@article{Zhang2013,
author = {Zhang, Jianzhong and Zhu, Jinlong and Velisavljevic, Nenad and Wang, Liping and Zhao, Yusheng},
doi = {10.1063/1.4828886},
issn = {0021-8979},
journal = {Journal of Applied Physics},
mendeley-groups = {Beryllium},
month = {nov},
number = {17},
pages = {173509},
title = {{Thermal equation of state and thermodynamic Gr{\"{u}}neisen parameter of beryllium metal}},
url = {http://aip.scitation.org/doi/10.1063/1.4828886},
volume = {114},
year = {2013}
}

]

@article{simakov2014optimized,
  title={Optimized beryllium target design for indirectly driven inertial confinement fusion experiments on the National Ignition Facility},
  author={Simakov, Andrei N and Wilson, Douglas C and Yi, Sunghwan A and Kline, John L and Clark, Daniel S and Milovich, Jose L and Salmonson, Jay D and Batha, Steven H},
  journal={Physics of Plasmas},
  volume={21},
  number={2},
  pages={022701},
  year={2014},
  publisher={American Institute of Physics}
}
@article{Kline2016,
abstract = {The first indirect drive implosion experiments using Beryllium (Be) capsules at the National Ignition Facility confirm the superior ablation properties and elucidate possible Be-ablator issues such as hohlraum filling by ablator material. Since the 1990s, Be has been the preferred Inertial Confinement Fusion (ICF) ablator because of its higher mass ablation rate compared to that of carbon-based ablators. This enables ICF target designs with higher implosion velocities at lower radiation temperatures and improved hydrodynamic stability through greater ablative stabilization. Recent experiments to demonstrate the viability of Be ablator target designs measured the backscattered laser energy, capsule implosion velocity, core implosion shape from self-emission, and in-flight capsule shape from backlit imaging. The laser backscatter is similar to that from comparable plastic (CH) targets under the same hohlraum conditions. Implosion velocity measurements from backlit streaked radiography show that laser energy coupling to the hohlraum wall is comparable to plastic ablators. The measured implosion shape indicates no significant reduction of laser energy from the inner laser cone beams reaching the hohlraum wall as compared with plastic and high-density carbon ablators. These results indicate that the high mass ablation rate for beryllium capsules does not significantly alter hohlraum energetics. In addition, these data, together with data for low fill-density hohlraum performance, indicate that laser power multipliers, required to reconcile simulations with experimental observations, are likely due to our limited understanding of the hohlraum rather than the capsule physics since similar multipliers are needed for both Be and CH capsules as seen in experiments.},
author = {Kline, J. L. and Yi, S. A. and Simakov, A. N. and Olson, R. E. and Wilson, D. C. and Kyrala, G. A. and Perry, T. S. and Batha, S. H. and Zylstra, A. B. and Dewald, E. L. and Tommasini, R. and Ralph, J. E. and Strozzi, D. J. and MacPhee, A. G. and Callahan, D. A. and Hinkel, D. E. and Hurricane, O. A. and Milovich, J. L. and Rygg, J. R. and Khan, S. F. and Haan, S. W. and Celliers, P. M. and Clark, D. S. and Hammel, B. A. and Kozioziemski, B. and Schneider, M. B. and Marinak, M. M. and Rinderknecht, H. G. and Robey, H. F. and Salmonson, J. D. and Patel, P. K. and Ma, T. and Edwards, M. J. and Stadermann, M. and Baxamusa, S. and Alford, C. and Wang, M. and Nikroo, A. and Rice, N. and Hoover, D. and Youngblood, K. P. and Xu, H. and Huang, H. and Sio, H.},
doi = {10.1063/1.4948277},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.4948277.pdf:pdf},
issn = {10897674},
journal = {Physics of Plasmas},
number = {5},
title = {{First beryllium capsule implosions on the National Ignition Facility}},
volume = {23},
year = {2016}
}
@article{Clark2018,
abstract = {Indirect drive implosion experiments on the National Ignition Facility (NIF) [E. I. Moses et al., Phys. Plasmas 16, 041006 (2009)] have now tested three different ablator materials: glow discharge polymer plastic, high density carbon, and beryllium. How do these different ablators compare in current and proposed implosion experiments on NIF? What are the relative advantages and disadvantages of each? This paper compares these different ablator options in capsule-only simulations of current NIF experiments and potential future designs. The simulations compare the impact of the capsule fill tube, support tent, and interface surface roughness for each case, as well as all perturbations in combination. According to the simulations, each ablator is impacted by the various perturbation sources differently, and each material poses unique challenges in the pursuit of ignition on NIF.},
author = {Clark, D. S. and Kritcher, A. L. and Yi, S. A. and Zylstra, A. B. and Haan, S. W. and Weber, C. R.},
doi = {10.1063/1.5016874},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.5016874.pdf:pdf},
issn = {10897674},
journal = {Physics of Plasmas},
number = {3},
title = {{Capsule physics comparison of National Ignition Facility implosion designs using plastic, high density carbon, and beryllium ablators}},
volume = {25},
year = {2018}
}
@article{Simakov2014,
abstract = {For indirect drive inertial confinement fusion, Beryllium (Be) ablators offer a number of important advantages as compared with other ablator materials, e.g., plastic and high density carbon. In particular, the low opacity and relatively high density of Be lead to higher rocket efficiencies giving a higher fuel implosion velocity for a given X-ray drive; and to higher ablation velocities providing more ablative stabilization and reducing the effect of hydrodynamic instabilities on the implosion performance. Be ablator advantages provide a larger target design optimization space and can significantly improve the National Ignition Facility (NIF) [J. D. Lindl et al., Phys. Plasmas 11, 339 (2004)] ignition margin. Herein, we summarize the Be advantages, briefly review NIF Be target history, and present a modern, optimized, low adiabat, Revision 6 NIF Be target design. This design takes advantage of knowledge gained from recent NIF experiments, including more realistic levels of laser-plasma energy backscatter, degraded hohlraum-capsule coupling, and the presence of cross-beam energy transfer. {\textcopyright} 2014 AIP Publishing LLC.},
author = {Simakov, Andrei N. and Wilson, Douglas C. and Yi, Sunghwan A. and Kline, John L. and Clark, Daniel S. and Milovich, Jose L. and Salmonson, Jay D. and Batha, Steven H.},
doi = {10.1063/1.4864331},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/1.4864331.pdf:pdf},
issn = {1070664X},
journal = {Physics of Plasmas},
number = {2},
title = {{Optimized beryllium target design for indirectly driven inertial confinement fusion experiments on the national ignition facility}},
volume = {21},
year = {2014}
}
@article{Haan2011,
abstract = {Point design targets have been specified for the initial ignition campaign on the National Ignition Facility G. H. Miller, E. I. Moses, and C. R. Wuest, Opt. Eng. 443, 2841 (2004). The targets contain D-T fusion fuel in an ablator of either CH with Ge doping, or Be with Cu. These shells are imploded in a U or Au hohlraum with a peak radiation temperature set between 270 and 300 eV. Considerations determining the point design include laser-plasma interactions, hydrodynamic instabilities, laser operations, and target fabrication. Simulations were used to evaluate choices, and to define requirements and specifications. Simulation techniques and their experimental validation are summarized. Simulations were used to estimate the sensitivity of target performance to uncertainties and variations in experimental conditions. A formalism is described that evaluates margin for ignition, summarized in a parameter the Ignition Threshold Factor (ITF). Uncertainty and shot-to-shot variability in ITF are evaluated, and sensitivity of the margin to characteristics of the experiment. The formalism is used to estimate probability of ignition. The ignition experiment will be preceded with an experimental campaign that determines features of the design that cannot be defined with simulations alone. The requirements for this campaign are summarized. Requirements are summarized for the laser and target fabrication. {\textcopyright} 2011 American Institute of Physics.},
author = {Haan, S. W. and Lindl, J. D. and Callahan, D. A. and Clark, D. S. and Salmonson, J. D. and Hammel, B. A. and Atherton, L. J. and Cook, R. C. and Edwards, M. J. and Glenzer, S. and Hamza, A. V. and Hatchett, S. P. and Herrmann, M. C. and Hinkel, D. E. and Ho, D. D. and Huang, H. and Jones, O. S. and Kline, J. and Kyrala, G. and Landen, O. L. and MacGowan, B. J. and Marinak, M. M. and Meyerhofer, D. D. and Milovich, J. L. and Moreno, K. A. and Moses, E. I. and Munro, D. H. and Nikroo, A. and Olson, R. E. and Peterson, K. and Pollaine, S. M. and Ralph, J. E. and Robey, H. F. and Spears, B. K. and Springer, P. T. and Suter, L. J. and Thomas, C. A. and Town, R. P. and Vesey, R. and Weber, S. V. and Wilkens, H. L. and Wilson, D. C.},
doi = {10.1063/1.3592169},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.3592169.pdf:pdf},
issn = {1070664X},
journal = {Physics of Plasmas},
number = {5},
title = {{Point design targets, specifications, and requirements for the 2010 ignition campaign on the National Ignition Facility}},
volume = {18},
year = {2011}
}
@article{Lu2017b,
abstract = {Beryllium (Be) is an important material with wide applications ranging from aerospace components to x-ray equipment. Yet a precise understanding of its phase diagram remains elusive. We have investigated the phase stability of Be using a recently developed hybrid free energy computation method that accounts for anharmonic effects by invoking phonon quasiparticles. We find that the hcp → bcc transition occurs near the melting curve at 0 {\textless} P {\textless} 11 GPa with a positive Clapeyron slope of 41 ± 4 K / GPa , which is more consistent with recent experimental measurements. This work also demonstrates the validity of this theoretical framework based on the phonon quasiparticle to study the structural stability and phase transitions in strongly anharmonic materials.},
author = {Lu, Y. and Sun, T. and Zhang, Ping and Zhang, P. and Zhang, D. B. and Wentzcovitch, R. M.},
doi = {10.1103/PhysRevLett.118.145702},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Lu et al. - 2017 - Premelting hcp to bcc Transition in Beryllium.pdf:pdf},
issn = {10797114},
journal = {Physical Review Letters},
number = {14},
title = {{Premelting hcp to bcc Transition in Beryllium}},
url = {https://journals.aps.org/prl/pdf/10.1103/PhysRevLett.118.145702},
volume = {118},
year = {2017}
}
@article{Palanivel2000,
abstract = {High-pressure electronic properties of Be have been investigated theoretically be means of ab initio electronic structure calculations. The calculations have been carried out by the semi-relativistic full-potential, linear muffin-tin orbital (FPLMTO) method, within the local density approximation. The crystal structure stability among the hcp, bcc and orthorhombic (distorted hcp) phases has been studied as a function of compression. The bcc structure is found to be energetically stable at pressures above 180 GPa. From the results of our calculations, the orthorhombic phase cannot occur as an intermediate phase between the ambient pressure hcp phase and the high-pressure bcc structure. Our work thus suggests the need for more accurate high-pressure x-ray data.},
author = {Palanivel, B. and Rao, R. S. and Godwal, B. K. and Sikka, S. K.},
doi = {10.1088/0953-8984/12/41/309},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/B{\_}Palanivel{\_}2000{\_}J.{\_}Phys.{\_}{\_}Condens.{\_}Matter{\_}12{\_}8831.pdf:pdf},
issn = {09538984},
journal = {Journal of Physics Condensed Matter},
number = {41},
pages = {8831--8836},
title = {{On the relative stability of orthorhombic and hcp phases of beryllium at high pressures}},
volume = {12},
year = {2000}
}
@article{Sinko2005a,
abstract = {Ab initio electronic-structure calculations, based on the density-functional theory and the full-potential linear-muffin-tin-orbital method, were used to predict crystal-sructure phase stabilities and elastic constants of beryllium under compression. Specific energies, pressures, elastic constants, and Debye temperatures for three crystal structures, hcp, bcc, and fcc, were calculated over a wide volume range. In agreement with experiments and previous theoretical calculations, the hcp ground state is obtained at ambient conditions and the bcc ground state is found at high pressure and ambient temperature, with the predicted hcp→bcc phase transition at about 2.7 Mbar. A possible phase diagram of beryllium, including hcp, bcc, and fcc phases is constructed in the (P,T) plane.},
author = {Sin'ko, G. V. and Smirnov, N. A.},
doi = {10.1103/PhysRevB.71.214108},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Sin'ko, Smirnov - 2005 - Relative stability and elastic properties of hcp, bcc, and fcc beryllium under pressure.pdf:pdf},
issn = {1098-0121},
journal = {Physical Review B},
month = {jun},
number = {21},
pages = {214108},
title = {{Relative stability and elastic properties of hcp, bcc, and fcc beryllium under pressure}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.71.214108},
volume = {71},
year = {2005}
}


@inproceedings{Robert2006a,
  title={Equation of state and elastic properties of beryllium from first principles calculations},
  author={Robert, G and Sollier, A},
  booktitle={Journal de Physique IV (Proceedings)},
  volume={134},
  pages={257--262},
  year={2006},
  organization={EDP sciences}
}

@article{Luo2012,
abstract = {We investigate the phase transition, elastic constants, phonon dispersion curves, and thermal properties of beryllium (Be) at high pressures and high temperatures using density functional theory. By comparing the Gibbs free energy, in the quasiharmonic approximation (QHA), of hexagonal-closed-packed (hcp) with those of the face-centered cubic (fcc) and body-centered-cubic (bcc) we find that the hcp Be is stable up to 390 GPa, and then transforms to the bcc Be. The calculated phonon dispersion curves are in excellent agreement with experiments. Under compression, the phonon dispersion curves of hcp Be do not show any anomaly or instability. At low pressure the phonon dispersion of bcc Be display imaginary along $\Omega$-N in the T 1 branches. Within the quasiharmonic approximation, we predict the thermal equation of state and other properties including the thermal expansion coefficient, Hugoniot curves, heat capacity, Gr{\"{u}}neisen parameter, and Debye temperature. {\textcopyright} 2012 American Institute of Physics.},
author = {Luo, Fen and Cai, Ling Cang and Chen, Xiang Rong and Jing, Fu Qian and Alf, Dario},
doi = {10.1063/1.3688344},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Luo et al. - 2012 - Ab initio calculation of lattice dynamics and thermodynamic properties of beryllium.pdf:pdf},
issn = {00218979},
journal = {Journal of Applied Physics},
number = {5},
title = {{Ab initio calculation of lattice dynamics and thermodynamic properties of beryllium}},
volume = {111},
year = {2012}
}

@article{Song2007,
author = {Song, Hai Feng and Liu, Hai Feng},
doi = {10.1103/PhysRevB.75.245126},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {24},
pages = {1--7},
title = {{Modified mean-field potential approach to thermodynamic properties of a low-symmetry crystal: Beryllium as a prototype}},
volume = {75},
year = {2007}
}


@article{Robert2010,
author = {Robert, G. and Legrand, P. and Bernard, S.},
doi = {10.1103/PhysRevB.82.104118},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Robert, Legrand, Bernard - 2010 - Multiphase equation of state and elastic moduli of solid beryllium from first principles.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {10},
title = {{Multiphase equation of state and elastic moduli of solid beryllium from first principles}},
url = {https://journals.aps.org/prb/pdf/10.1103/PhysRevB.82.104118},
volume = {82},
year = {2010}
}

@article{Xian2019b,
author = {Xian, Jia Wei and Yan, Jun and Liu, Hai Feng and Sun, Tao and Zhang, Gong Mu and Gao, Xing Yu and Song, Hai Feng},
doi = {10.1103/PhysRevB.99.064102},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Xian et al. - 2019 - Effect of anharmonicity on the hcp to bcc transition in beryllium at high-pressure and high-temperature conditions.pdf:pdf},
issn = {24699969},
journal = {Physical Review B},
keywords = {doi:10.1103/PhysRevB.99.064102 url:https://doi.org},
number = {6},
pages = {1--12},
publisher = {American Physical Society},
title = {{Effect of anharmonicity on the hcp to bcc transition in beryllium at high-pressure and high-temperature conditions}},
volume = {99},
year = {2019}
}
@article{Clark2008,
abstract = {Inertial confinement fusion capsules are critically dependent on the integrity of their hot spots to ignite. At the time of ignition, only a certain fractional perturbation of the nominally spherical hot spot boundary can be tolerated and the capsule still achieve ignition. The degree to which the expected hot spot perturbation in any given capsule design is less than this maximum tolerable perturbation is a measure of the ignition margin or robustness of that design. Moreover, since there will inevitably be uncertainties in the initial character and implosion dynamics of any given capsule, all of which can contribute to the eventual hot spot perturbation, quantifying the robustness of that capsule against a range of parameter variations is an important consideration in the capsule design. Here, the robustness of the 300 eV indirect drive target design for the National Ignition Facility [Lindl, Phys. Plasmas 11, 339 (2004)] is studied in the parameter space of inner ice roughness, implosion velocity, and capsule scale. A suite of 2000 two-dimensional simulations, run with the radiation hydrodynamics code LASNEX, is used as the data base for the study. For each scale, an ignition region in the two remaining variables is identified and the ignition cliff is mapped. In accordance with the theoretical arguments of Levedahl and Lindl [Nucl. Fusion 37, 165 (1997)] and Kishony and Shvarts [Phys. Plasmas 8, 4925 (2001)], the location of this cliff is fitted to a power law of the capsule implosion velocity and scale. It is found that the cliff can be quite well represented in this power law form, and, using this scaling law, an assessment of the overall (one- and two-dimensional) ignition margin of the design can be made. The effect on the ignition margin of an increase or decrease in the density of the target fill gas is also assessed. {\textcopyright} 2008 American Institute of Physics.},
author = {Clark, Daniel S. and Haan, Steven W. and Salmonson, Jay D.},
doi = {10.1063/1.2890123},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.2890123.pdf:pdf},
issn = {1070664X},
journal = {Physics of Plasmas},
number = {5},
title = {{Robustness studies of ignition targets for the National Ignition Facility in two dimensions}},
volume = {15},
year = {2008}
}

@article{Martin1959,
author = {Martin, A.J. and Moore, A.},
doi = {10.1016/0022-5088(59)90045-1},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Unknown - 1959 - to sudden changes in furnace voltage , and also served to cut down convection currents in the argon atmosphere . Heati.pdf:pdf},
issn = {00225088},
journal = {Journal of the Less Common Metals},
month = {apr},
number = {2},
pages = {85--93},
title = {{The structure of beryllium, with particular reference to temperatures above 1200$^{\text{o}}$C}},
url = {https://linkinghub.elsevier.com/retrieve/pii/0022508859900451},
volume = {1},
year = {1959}
}
@article{Ming1984a,
abstract = {In situ high-pressure X-ray diffraction data for polycrystalline beryllium to 28.3 GPA at ambient temperature show that beryllium is transformed from the HCP phase (I) into a slightly distorted HCP phase (II) at pressures between 8.6 and 14.5 GPa. The volume change for the transition is extremely small ( approximately 0.4{\%}); the effect of pressure on the c/a ratio for both the Be(I) and Be(II) phases is also very small.},
author = {Ming, L. C. and Manghnani, M. H.},
doi = {10.1088/0305-4608/14/1/001},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/L{\_}C{\_}Ming{\_}1984{\_}J.{\_}Phys.{\_}F{\_}{\_}Met.{\_}Phys.{\_}14{\_}L1.pdf:pdf},
issn = {03054608},
journal = {Journal of Physics F: Metal Physics},
number = {1},
title = {{Isothermal compression and phase transition in beryllium to 28.3 GPa}},
volume = {14},
year = {1984}
}

@article{Vijayakumar1984b,
abstract = {The metal beryllium (Be) has been studied under high pressure using an electrical resistivity technique with in situ pressure calibration. A sluggish phase transition at 12 GPa is observed which the authors identify as the HCP to distorted HCP phase transition reported in a recent high-pressure X-ray diffraction study. However, a reanalysis of the X-ray data on the high-pressure phase Be(II) indicates that a smaller orthorhombic cell with four atoms fits the observed interplanar spacings. The observed intensity ratios of the diffraction lines can be explained reasonably well on the basis of the space group P2 1 2 1 2 with four Be atoms occupying 4c positions.},
author = {Vijayakumar, V. and Godwal, B. K. and Vohra, Y. K. and Sikka, S. K. and Chidambaram, R.},
doi = {10.1088/0305-4608/14/5/002},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Vijayakumar et al. - 1984 - On the high-pressure phase transition in beryllium metal.pdf:pdf},
issn = {03054608},
journal = {Journal of Physics F: Metal Physics},
number = {5},
title = {{On the high-pressure phase transition in beryllium metal}},
volume = {14},
year = {1984}
}

@article{Lazicki2012b,
author = {Lazicki, Amy and Dewaele, Agn{\`{e}}s and Loubeyre, Paul and Mezouar, Mohamed},
doi = {10.1103/PhysRevB.86.174118},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Lazicki et al. - 2012 - High-pressure-temperature phase diagram and the equation of state of beryllium.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {17},
pages = {1--10},
title = {{High-pressure-temperature phase diagram and the equation of state of beryllium}},
volume = {86},
year = {2012}
}


@article{Nakano2002b,
author = {Nakano, Kazutaka and Akahama, Yuichi and Kawamura, Haruki},
doi = {10.1088/0953-8984/14/44/334},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Nakano, Akahama, Kawamura - 2002 - X-ray diffraction study of Be to megabar pressure.pdf:pdf},
issn = {09538984},
journal = {Journal of Physics Condensed Matter},
number = {44 SPEC ISS.},
pages = {10569--10573},
title = {{X-ray diffraction study of Be to megabar pressure}},
volume = {14},
year = {2002}
}


@article{McCoy2019a,
author = {McCoy, Chad A. and Knudson, Marcus D. and Desjarlais, Michael P.},
doi = {10.1103/PhysRevB.100.054107},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevB.100.054107.pdf:pdf},
issn = {24699969},
journal = {Physical Review B},
keywords = {doi:10.1103/PhysRevB.100.054107 url:https://doi.or},
number = {5},
pages = {1--13},
publisher = {American Physical Society},
title = {{Sound velocity, shear modulus, and shock melting of beryllium along the Hugoniot}},
volume = {100},
year = {2019}
}

@article{Brown2014a,
abstract = {A magnetohydrodynamic loading technique was used to shocklessly compress beryllium to peak longitudinal stresses of 19-110 GPa and, subsequently, unload in order to determine both the compressive response and also the shear stress supported upon release. Loading strain rates were on the order of 10 6s-1, while the unloading rates were nearly constant at 3 × 105s-1. Velocimetry was used to monitor the ramp and release behavior of a beryllium/lithium fluoride window interface. After applying window corrections to infer in situ beryllium velocities, a Lagrangian analysis was employed to determine the material response. The Lagrangian wavespeed-particle velocity response is integrated to generate the stress-strain path, average change in shear stress over the elastic unloading, and estimates of the shear modulus at peak compression. These data are used to infer the pressure dependence of the flow strength at the unloading rate. Comparisons to several strength models reveal good agreement to 45 GPa, but the data indicate 20{\%}-30{\%} higher strength near 100 GPa. {\textcopyright} 2014 AIP Publishing LLC.},
author = {Brown, J. L. and Knudson, M. D. and Alexander, C. S. and Asay, J. R.},
doi = {10.1063/1.4890232},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/1.4890232.pdf:pdf},
issn = {10897550},
journal = {Journal of Applied Physics},
number = {3},
title = {{Shockless compression and release behavior of beryllium to 110 GPa}},
url = {http://dx.doi.org/10.1063/1.4890232},
volume = {116},
year = {2014}
}
@article{Wang2013a,
abstract = {We have calculated the equations of state, the viscosity and self-diffusion coefficients, and electronic transport coefficients of beryllium in the warm dense regime for densities from 4.0 to 6.0 g/cm3 and temperatures from 1.0 to 10.0 eV by using quantum molecular dynamics simulations. The principal Hugoniot curve is in agreement with underground nuclear explosive and high-power laser experimental results up to ∼20 Mbar. The calculated viscosity and self-diffusion coefficients are compared with the one-component plasma model, using effective charges given by the average-atom model. The Stokes-Einstein relationship, which connects viscosity and self-diffusion coefficients, is found to hold fairly well in the strong coupling regime. The Lorenz number, which is the ratio between thermal and electrical conductivities, is computed via Kubo-Greenwood formula and compared to the well-known Wiedemann-Franz law in the warm dense region. {\textcopyright} 2013 American Physical Society.},
author = {Wang, Cong and Long, Yao and Tian, Ming Feng and He, Xian Tu and Zhang, Ping},
doi = {10.1103/PhysRevE.87.043105},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevE.87.043105.pdf:pdf},
issn = {15393755},
journal = {Physical Review E - Statistical, Nonlinear, and Soft Matter Physics},
number = {4},
pages = {1--6},
title = {{Equations of state and transport properties of warm dense beryllium: A quantum molecular dynamics study}},
volume = {87},
year = {2013}
}




@article{Evans2005a,
abstract = {We report combined x-ray and Raman studies of beryllium in helium and argon pressure media at pressures approaching 200 GPa. Our results are generally consistent with recent studies confirming the stability of the hexagonal close-packed phase to the highest pressures. However, the quasihydrostatic conditions of our studies lead to a stiffer equation of state (K0=109.88, K′0=3.59) and a gradual approach toward a more ideal c∕a ratio of 1.60 at 180 GPa. Combining our Raman and equation of state data, we are able to evaluate the pressure dependence of the elastic shear modulus (C44=109.3, C′44=1.959). We discuss the comparison of our results with measurements using ultrasonic and dynamic techniques.},
author = {Evans, W. J. and Lipp, M. J. and Cynn, H. and Yoo, C. S. and Somayazulu, M. and H{\"{a}}usermann, D. and Shen, G. and Prakapenka, V.},
doi = {10.1103/PhysRevB.72.094113},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Evans et al. - 2005 - X-ray diffraction and Raman studies of beryllium Static and elastic properties at high pressures.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {9},
pages = {1--6},
title = {{X-ray diffraction and Raman studies of beryllium: Static and elastic properties at high pressures}},
volume = {72},
year = {2005}
}




@article{Nellis2003b,
author = {Nellis, W. J. and Mitchell, A. C. and Young, D. A.},
doi = {10.1063/1.1529071},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/1.1529071.pdf:pdf},
issn = {00218979},
journal = {Journal of Applied Physics},
number = {1},
pages = {304--310},
title = {{Equation-of-state measurements for aluminum, copper, and tantalum in the pressure range 80-440 GPa (0.8-4.4 Mbar)}},
volume = {93},
year = {2003}
}


@article{Velisavljevic2002a,
abstract = {The structural and electrical properties of alkaline-earth metal beryllium were studied to 66 GPa using designer diamond anvils. The ambient pressure hexagonal close-packed phase was found to be stable to the highest pressure of 66 GPa and the measured static equation of state differs substantially from the one derived from the existing shock wave data. The electrical resistance data at high pressure shows a gradual decrease in resistance to pressure up to 25 GPa followed by a slight increase to 53 Gpa. The axial ratio (c/a) remains strongly nonideal with c/a = 1.562 at V/V 0  = 0.708, indicating that deviations from nearly free electron behavior are still dominant at high compressions.},
author = {Velisavljevic, Nenad and Chesnut, Gary N. and Vohra, Yogesh K. and Weir, Samuel T. and Malba, Vincent and Akella, Jagannadham},
doi = {10.1103/PhysRevB.65.172107},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Velisavljevic et al. - 2002 - Structural and electrical properties of beryllium metal to 66 GPa studied using designer diamond anvils.pdf:pdf},
issn = {01631829},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {17},
pages = {1721071--1721074},
title = {{Structural and electrical properties of beryllium metal to 66 GPa studied using designer diamond anvils}},
volume = {65},
year = {2002}
}


@article{Cauble1998b,
  title={Absolute equation-of-state data in the 10--40 Mbar (1--4 TPa) regime},
  author={Cauble, R and Perry, TS and Bach, DR and Budil, KS and Hammel, BA and Collins, GW and Gold, DM and Dunn, J and Celliers, P and Da Silva, LB and others},
  journal={Physical review letters},
  volume={80},
  number={6},
  pages={1248},
  year={1998},
  publisher={APS}
}

@article{Boivineau1993a,
abstract = {A submillisecond resistive heating technique under high pressure (0.12 GPa) has been used to measure selected thermophysical properties of both solid and liquid beryllium. Data have been obtained between room temperature and 2900 K. Results on enthalpy, volume expansion, electrical resistivity, and sound velocity measurements are presented. {\textcopyright} 1993 Plenum Publishing Corporation.},
author = {Boivineau, M. and Arl{\'{e}}s, L. and Vermeulen, J. M. and Th{\'{e}}venin, Th},
doi = {10.1007/BF00566042},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Boivineau1993{\_}Article{\_}ThermophysicalPropertiesOfSoli.pdf:pdf},
issn = {0195928X},
journal = {International Journal of Thermophysics},
keywords = {beryllium,electrical resistivity,enthalpy,high pressure,high temperature,isobaric expansion,liquid metals,sound velocity},
number = {3},
pages = {427--439},
title = {{Thermophysical properties of solid and liquid beryllium}},
volume = {14},
year = {1993}
}
@article{Swenson1991a,
abstract = {Linear thermal expansivity measurements from 4.2 to 302 K and heat capacity measurements from 4.6 to 108 K have been made on HIP (hot isostatic pressing) beryllium metal. The heat capacity data are in good agreement with previous data from 1.4 to 30 K for high purity single crystals. Our $\Theta$0 = 1485(5) K also agrees well with that calculated from high-pressure elastic constant results. The linear thermal expansivity decreases rapidly with decreasing temperature from 1.13 × 10-5 K-1 at 293 K, as would be expected for the large $\Theta$0, and becomes very small ({\textless} 10-7 K-1) below 50 K. The expansivities below 108 K are consistent with a constant $\gamma$lat0 = 1.15 and with $\gamma$lat0 = 0.91 from the high-pressure elastic constant results.},
author = {Swenson, C. A.},
doi = {10.1063/1.349336},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/1.349336.pdf:pdf},
issn = {00218979},
journal = {Journal of Applied Physics},
number = {6},
pages = {3046--3051},
title = {{HIP beryllium: Thermal expansivity from 4 to 300 K and heat capacity from 1 to 108 K}},
volume = {70},
year = {1991}
}


@article{Ragan1982b,
abstract = {A shock wave generated by an underground nuclear explosion was used to perform impedance-matching experiments for several different materials at pressures from 1 to 7 TPa. The nearly planar shock passed through a 180-mm-diam by 12-mm-thick molybdenum standard and into stacks of 10-mm-thick samples of the following adjacent pairs of materials: LiD-Be, Be-LiD, Al-Mo, Pb-quartz, W-Mo (low density, 0=8.29 g cm-3), U-Mo, and Fe. An array of 75 electrical contact pins was used to determine the shape of the shock front and the shock velocities in the standard and in the samples with uncertainties ranging from 1.5 to 2.5{\%}. The measured shock velocity of 27.30 km/s (1.5{\%}) in the molybdenum standard corresponds to a pressure of 4.95 TPa (3.5{\%}) based on a theoretical equation of state (EOS) that includes electronic-shell-structure effects. An impedance-matching analysis was performed for each sample stack to obtain Hugoniot data for all samples except those in the U-Mo stack; neutron-induced fission heating in the uranium perturbed the initial state and produced inconclusive results. Predictions, based on the SESAME EOS library, of shock velocities in most samples agree with the experimental results within the uncertainties. For the quartz and low-density molybdenum, the SESAME-predicted shock velocities are too large by 5 to 10{\%}. The following Hugoniot points in pressure (P)-particle-velocity (u) coordinates were determined for the indicated samples: LiD (p=0.946 TPa, u=29.39 km/s), Be (1.46, 22.69); Be (1.79, 25.42), LiD (1.038, 31.23); Al (2.23, 23.89), Mo (4.03, 16.05); Pb (4.80, 17.84), quartz (1.66, 23.64); W (6.51, 15.10), and Mo (0=8.29 g cm-3) (3.68, 18.27). The results for iron have a larger uncertainty but are consistent with the SESAME predictions. {\textcopyright} 1982 The American Physical Society.},
author = {Ragan, Charles E.},
doi = {10.1103/PhysRevA.25.3360},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevA.25.3360.pdf:pdf},
issn = {10502947},
journal = {Physical Review A},
number = {6},
pages = {3360--3375},
title = {{Shock compression measurements at 1 to 7 TPa}},
volume = {25},
year = {1982}
}

@inproceedings{Wise1982b,
author = {Wise, J. L. and Chhabildas, L. C. and Asay, J. R.},
booktitle = {AIP Conference Proceeding Volume 78},
doi = {10.1063/1.33350},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/1.33350.pdf:pdf},
pages = {417--421},
publisher = {AIP},
title = {{Shock compression of beryllium}},
url = {http://aip.scitation.org/doi/abs/10.1063/1.33350},
volume = {417},
year = {1982}
}


@article{Walsh1957b,
author = {Walsh, John M. and Rice, Melvin H. and McQueen, Robert G. and Yarger, Frederick L.},
doi = {10.1103/PhysRev.108.196},
issn = {0031899X},
journal = {Physical Review},
number = {2},
pages = {196--216},
title = {{Shock-wave compressions of twenty-seven metals. equations of state of metals}},
volume = {108},
year = {1957}
}
@article{Gordon1949a,
abstract = {A high temperature precision x-ray camera has been designed and constructed by modification of the familiar back-reflection symmetrical focusing type of camera. The camera, specimen, and furnace are used within a vacuum chamber to avoid oxidation. The apparatus in its present form has been employed at temperatures up to 1000°C, but higher temperatures could be easily attained by making a few minor changes in the furnace materials. The lattice parameters of beryllium have been measured up to 1000°C. The derived coefficients of thermal expansion, both linear and bulk, are presented as a function of temperature. In addition, the data present strong evidence that the hexagonal close packed form of beryllium which exists at room temperature is stable up to at least 1000°C, contrary to several reports in the literature.},
author = {Gordon, Paul},
doi = {10.1063/1.1698252},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/1.1698252.pdf:pdf},
issn = {00218979},
journal = {Journal of Applied Physics},
number = {10},
pages = {908--917},
title = {{A high temperature precision x-ray camera: Some measurements of the thermal coefficients of expansion of beryllium}},
volume = {20},
year = {1949}
}
@article{Wang1991a,
abstract = {For a uniform electron gas of density n=n+n=3/4rs3=ks6/192 and spin polarization =(n-n)/n, we study the Fourier transform c(k,rs,) of the correlation hole, as well as the correlation energy c(rs,)=F0dk c/. In the high-density (rs0) limit, we find a simple scaling relation ksc/g2f(z,), where z=k/gks, g=[(1+)2/3+(1-)2/3]/2, and f(z,1)=f(z,0). The function f(z,) is only weakly dependent, and its small-z expansion -3z/2+4 3 z2/2+... is also the exact small-wave-vector (k0) expansion for any rs or. Motivated by these considerations, and by a discussion of the large-wave-vector and low-density limits, we present two Pad{\'{e}} representations for c at any k, rs, or ,one within and one beyond the random-phase approximation (RPA). We also show that cRPA obeys a generalization of Misawas spin-scaling relation for cRPA, and that the low-density (rs) limit of cRPA is rs-3/4. {\textcopyright} 1991 The American Physical Society.},
author = {Wang, Yue and Perdew, John P.},
doi = {10.1103/PhysRevB.44.13298},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/caratio high pressure/PhysRevB.44.13298.pdf:pdf},
issn = {01631829},
journal = {Physical Review B},
number = {24},
pages = {13298--13307},
title = {{Correlation hole of the spin-polarized electron gas, with exact small-wave-vector and high-density scaling}},
volume = {44},
year = {1991}
}
@article{Kresse1996f,
abstract = {We present a detailed description and comparison of algorithms for performing ab-initio quantum-mechanical calculations using pseudopotentials and a plane-wave basis set. We will discuss: (a) partial occupancies within the framework of the linear tetrahedron method and the finite temperature density-functional theory, (b) iterative methods for the diagonalization of the Konn-Sham Hamiltonian and a discussion of an efficient iterative method based on the ideas of Pulay's residual minimization, which is close to an order N2atoms scaling even for relatively large systems, (c) efficient Broyden-like and Pulay-like mixing methods for the charge density including a new special 'preconditioning' optimized for a plane-wave basis set, (d) conjugate gradient methods for minimizing the electronic free energy with respect to all degrees of freedom simultaneously. We have implemented these algorithms within a powerful package called VAMP (Vienna ab-initio molecular-dynamics package). The program and the techniques have been used successfully for a large number of different systems (liquid and amorphous semiconductors, liquid simple and transition metals, metallic and semi-conducting surfaces, phonons in simple metals, transition metals and semiconductors) and turned out to be very reliable.},
author = {Kresse, G. and Furthm{\"{u}}ller, J.},
doi = {10.1016/0927-0256(96)00008-0},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/1-s2.0-0927025696000080-main (1).pdf:pdf},
issn = {09270256},
journal = {Computational Materials Science},
number = {1},
pages = {15--50},
title = {{Efficiency of ab-initio total energy calculations for metals and semiconductors using a plane-wave basis set}},
volume = {6},
year = {1996}
}
@article{Vanderbilt1990a,
abstract = {These instructions indicate how to prepare a manuscript for rapid publication in GASTROENTEHOLOGY and exemplify the exact format to follow. {\textcopyright} 1977, The Williams {\&} Wilkins Co.. All rights reserved.},
author = {Vanderbilt, David},
doi = {10.1103/PhysRevB.41.7892},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevB.41.7892.pdf:pdf},
issn = {0163-1829},
journal = {Physical Review B},
month = {apr},
number = {11},
pages = {7892--7895},
pmid = {18235770},
title = {{Soft self-consistent pseudopotentials in a generalized eigenvalue formalism}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.41.7892},
volume = {41},
year = {1990}
}
@article{Kresse1999b,
abstract = {The formal relationship between ultrasoft (US) Vanderbilt-type pseudopotentials and Bl{\"{o}}chl's projector augmented wave (PAW) method is derived. It is shown that the total energy functional for US pseudopotentials can be obtained by linearization of two terms in a slightly modified PAW total energy functional. The Hamilton operator, the forces, and the stress tensor are derived for this modified PAW functional. A simple way to implement the PAW method in existing plane-wave codes supporting US pseudopotentials is pointed out. In addition, critical tests are presented to compare the accuracy and efficiency of the PAW and the US pseudopotential method with relaxed core all electron methods. These tests include small molecules (Formula presented) and several bulk systems (diamond, Si, V, Li, Ca, (Formula presented) Fe, Co, Ni). Particular attention is paid to the bulk properties and magnetic energies of Fe, Co, and Ni. {\textcopyright} 1999 The American Physical Society.},
author = {Kresse, G. and Joubert, D.},
doi = {10.1103/PhysRevB.59.1758},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevB.59.1758.pdf:pdf},
issn = {0163-1829},
journal = {Physical Review B},
month = {jan},
number = {3},
pages = {1758--1775},
title = {{From ultrasoft pseudopotentials to the projector augmented-wave method}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.59.1758},
volume = {59},
year = {1999}
}
@article{Kresse1996e,
abstract = {We present an efficient scheme for calculating the Kohn-Sham ground state of metallic systems using pseudopotentials and a plane-wave basis set. In the first part the application of Pulay's DIIS method (direct inversion in the iterative subspace) to the iterative diagonalization of large matrices will be discussed. Our approach is stable, reliable, and minimizes the number of order (Formula presented) operations. In the second part, we will discuss an efficient mixing scheme also based on Pulay's scheme. A special “metric” and a special “preconditioning” optimized for a plane-wave basis set will be introduced. Scaling of the method will be discussed in detail for non-self-consistent and self-consistent calculations. It will be shown that the number of iterations required to obtain a specific precision is almost independent of the system size. Altogether an order (Formula presented) scaling is found for systems containing up to 1000 electrons. If we take into account that the number of k points can be decreased linearly with the system size, the overall scaling can approach (Formula presented). We have implemented these algorithms within a powerful package called VASP (Vienna ab initio simulation package). The program and the techniques have been used successfully for a large number of different systems (liquid and amorphous semiconductors, liquid simple and transition metals, metallic and semiconducting surfaces, phonons in simple metals, transition metals, and semiconductors) and turned out to be very reliable. {\textcopyright} 1996 The American Physical Society.},
author = {Kresse, G. and Furthm{\"{u}}ller, J.},
doi = {10.1103/PhysRevB.54.11169},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevB.54.11169.pdf:pdf},
issn = {1550235X},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {16},
pages = {11169--11186},
pmid = {9984901},
title = {{Efficient iterative schemes for ab initio total-energy calculations using a plane-wave basis set}},
volume = {54},
year = {1996}
}

@article{P.E.Blochl1994c,
author = {P.E.Bl{\"{o}}chl},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/P.E.Bl{\"{o}}chl - 1994 - Projector augmented-wave method.pdf:pdf},
journal = {Physical Review B},
number = {24},
pages = {17953--17979},
title = {{Projector augmented-wave method}},
volume = {50},
year = {1994}
}
@article{Monkhorst1976b,
abstract = {It is again emphasized that for all cubic lattices the method of Monkhorst and Pack generates not only point sets identical to those obtained by Chadi and Cohen, but also intermediate sets with the same properties. In addition, a comparison of these two methods for the hexagonal lattice reveals our method to be more flexible and efficient. {\textcopyright} 1977 The American Physical Society.},
author = {Monkhorst, Hendrik J. and Pack, James D.},
doi = {10.1103/PhysRevB.13.5188},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevB.13.5188.pdf:pdf},
issn = {0556-2805},
journal = {Physical Review B},
month = {jun},
number = {12},
pages = {5188--5192},
title = {{Special points for Brillouin-zone integrations}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.16.1748 https://link.aps.org/doi/10.1103/PhysRevB.13.5188},
volume = {13},
year = {1976}
}
@article{Perdew1996,
author = {Perdew, John P and Burke, Kieron and Ernzerhof, Matthias},
doi = {10.1103/PhysRevLett.77.3865},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Perdew, Burke, Ernzerhof - 1996 - Generalized Gradient Approximation Made Simple.pdf:pdf},
issn = {0031-9007},
journal = {Physical Review Letters},
month = {oct},
number = {18},
pages = {3865--3868},
title = {{Generalized Gradient Approximation Made Simple}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.77.3865},
volume = {77},
year = {1996}
}
@article{Nose1984a,
abstract = {Three recently proposed constant temperature molecular dynamics methods by: (i) Nos{\'{e}} (Mol. Phys., to be published); (ii) Hoover et al. [Phys. Rev. Lett. 48, 1818 (1982)], and Evans and Morriss [Chem. Phys. 77, 63 (1983)]; and (iii) Haile and Gupta [J. Chem. Phys. 79, 3067 (1983)] are examined analytically via calculating the equilibrium distribution functions and comparing them with that of the canonical ensemble. Except for effects due to momentum and angular momentum conservation, method (i) yields the rigorous canonical distribution in both momentum and coordinate space. Method (ii) can be made rigorous in coordinate space, and can be derived from method (i) by imposing a specific constraint. Method (iii) is not rigorous and gives a deviation of order N -1/2 from the canonical distribution (N the number of particles). The results for the constant temperature-constant pressure ensemble are similar to the canonical ensemble case. {\textcopyright} 1984 American Institute of Physics.},
author = {Nos{\'{e}}, Shuichi},
doi = {10.1063/1.447334},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Nose/1.447334.pdf:pdf},
issn = {00219606},
journal = {The Journal of Chemical Physics},
number = {1},
pages = {511--519},
title = {{A unified formulation of the constant temperature molecular dynamics methods}},
volume = {81},
year = {1984}
}
@article{Nose1991,
author = {Nos{\'{e}}, Shuichi},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Nose/103-1.pdf:pdf},
journal = {Progress of Theoretical Physics Supplement},
number = {103},
pages = {1--46},
title = {{Constant Temperature Molecular Dynamics Methods Limitations in simulations in the microcanonical ensemble}},
year = {1991}
}

@article{Polson2000a,
author = {Polson, J. M. and Trizac, E. and Pronk, S. and Frenkel, D.},
doi = {10.1063/1.481102},
file = {:Users/wjz8597/Library/Mobile Documents/3L68KQB4HG{\~{}}com{\~{}}readdle{\~{}}CommonDocuments/Documents/Computational Chemistry/1.481102.pdf:pdf},
issn = {00219606},
journal = {Journal of Chemical Physics},
number = {12},
pages = {5339--5342},
title = {{Finite-size corrections to the free energies of crystalline solids}},
volume = {112},
year = {2000}
}

@article{Frenkel1984,
author = {Frenkel, Daan and Ladd, Anthony J. C.},
doi = {10.1063/1.448024},
file = {:Users/wjz8597/Library/Mobile Documents/3L68KQB4HG{\~{}}com{\~{}}readdle{\~{}}CommonDocuments/Documents/Computational Chemistry/1.448024.pdf:pdf},
issn = {0021-9606},
journal = {The Journal of Chemical Physics},
month = {oct},
number = {7},
pages = {3188--3193},
title = {{New Monte Carlo method to compute the free energy of arbitrary solids. Application to the fcc and hcp phases of hard spheres}},
url = {http://aip.scitation.org/doi/10.1063/1.448024},
volume = {81},
year = {1984}
}


@article{Riffet2020,
author = {Riffet, Vanessa and Amadon, Bernard and Bruzy, Nicolas and Denoual, Christophe},
doi = {10.1103/PhysRevMaterials.4.063609},
issn = {2475-9953},
journal = {Physical Review Materials},
keywords = {doi:10.1103/PhysRevMaterials.4.063609 url:https://},
mendeley-groups = {Beryllium},
month = {jun},
number = {6},
pages = {063609},
publisher = {American Physical Society},
title = {{Role of dislocations in the bcc-hcp transition under high pressure: A first-principles approach in beryllium}},
url = {https://link.aps.org/doi/10.1103/PhysRevMaterials.4.063609},
volume = {4},
year = {2020}
}


@article{Dremov2015,
author = {Dremov, V. V. and Rykounov, A. A. and Sapozhnikov, F. A. and Karavaev, A. V. and Yakovlev, S. V. and Ionov, G. V. and Ryzhkov, M. V.},
doi = {10.1063/1.4923430},
issn = {0021-8979},
journal = {Journal of Applied Physics},
mendeley-groups = {Beryllium},
month = {jul},
number = {3},
pages = {035901},
title = {{Cold melting of beryllium: Atomistic view on Z-machine experiments}},
url = {http://dx.doi.org/10.1063/1.4923430 http://aip.scitation.org/doi/10.1063/1.4923430},
volume = {118},
year = {2015}
}


@inproceedings{Thompson2012,
author = {Thompson, Aidan P. and Lane, J. Matthew D and Desjarlais, Michael},
booktitle = {AIP Conference Proceedings},
doi = {10.1063/1.3686522},
file = {:Users/fgonzalez/Library/Application Support/Mendeley Desktop/Downloaded/Thompson, Lane, Desjarlais - 2012 - AIP Conference Proceedings.pdf:pdf},
isbn = {9780735410060},
issn = {0094243X},
keywords = {MEAM,Molecular dynamics,thermodynamic and mechanical properties},
mendeley-groups = {Beryllium},
pages = {1311--1314},
title = {{Molecular dynamics simulation of dynamic response of beryllium}},
url = {http://aip.scitation.org/doi/abs/10.1063/1.3686522},
volume = {1426},
year = {2012}
}

@article{Karavaev2016,
author = {Karavaev, A V and Dremov, V V and Pravishkina, T A},
doi = {http://dx.doi.org/10.1016/j.commatsci.2016.08.014},
file = {:Users/fgonzalez/Library/Application Support/Mendeley Desktop/Downloaded/Karavaev, Dremov, Pravishkina - 2016 - Computational Materials Science.pdf:pdf},
issn = {0927-0256},
journal = {Computational Materials Science},
keywords = {Liquid-solid coexistence},
mendeley-groups = {Z-method,Melting Iron,Beryllium},
pages = {335--343},
publisher = {Elsevier B.V.},
title = {{Precise calculation of melting curves by molecular dynamics}},
url = {http://www.sciencedirect.com/science/article/pii/S0927025616303846},
volume = {124},
year = {2016}
}


@article{Guo2014,
author = {Guo, Zhi-Cheng and Luo, Fen and Cheng, Yan},
doi = {10.1016/j.commatsci.2013.12.013},
file = {:Users/fgonzalez/Library/Application Support/Mendeley Desktop/Downloaded/Pu et al. - 2015 - Computational Materials Science.pdf:pdf},
issn = {09270256},
journal = {Computational Materials Science},
keywords = {First-principles calculations,Phase transition,Thermodynamic properties},
mendeley-groups = {Beryllium},
month = {mar},
pages = {139--144},
publisher = {Elsevier B.V.},
title = {{Phase transition and thermodynamic properties of beryllium from first-principles calculations}},
url = {http://dx.doi.org/10.1016/j.commatsci.2013.12.013 https://linkinghub.elsevier.com/retrieve/pii/S0927025615000737 https://linkinghub.elsevier.com/retrieve/pii/S0927025613007623},
volume = {84},
year = {2014}
}



@article{Li2014,
author = {Li, Dafang and Zhang, Ping and Yan, Jun},
doi = {10.1038/srep04707},
file = {:Users/fgonzalez/Library/Application Support/Mendeley Desktop/Downloaded/Li, Zhang, Yan - 2014 - Scientific reports.pdf:pdf},
issn = {2045-2322},
journal = {Scientific Reports},
mendeley-groups = {Z-method,Beryllium},
month = {may},
number = {1},
pages = {4707},
pmid = {24759594},
title = {{Ab initio molecular dynamics study of high-pressure melting of beryllium oxide}},
url = {http://www.pubmedcentral.nih.gov/articlerender.fcgi?artid=3998012&tool=pmcentrez&rendertype=abstract http://www.nature.com/articles/srep04707},
volume = {4},
year = {2015}
}



@inproceedings{Coe2020,
author = {Coe, Joshua D and Rudin, Sven P and Maiorov, Boris},
booktitle = {AIP Conference Proceedings},
doi = {10.1063/12.0000902},
file = {:Users/fgonzalez/Library/Application Support/Mendeley Desktop/Downloaded/12.0000902.pdf:pdf},
isbn = {9780735440005},
mendeley-groups = {Beryllium},
pages = {070009},
title = {{Multiphase equation of state and thermoelastic data for polycrystalline beryllium}},
url = {http://aip.scitation.org/doi/abs/10.1063/12.0000902},
volume = {070009},
year = {2020}
}



@article{Gonzalez-Cataldo2016,
author = {Gonz{\'{a}}lez-Cataldo, Felipe and Davis, Sergio and Guti{\'{e}}rrez, Gonzalo},
journal = {Scientific Reports},
month = {may},
number = {October 2014},
pages = {26537},
publisher = {Nature Publishing Group},
title = {{Melting curve of SiO$_2$ at multimegabar pressures: implications for gas giants and super-Earths}},
url = {http://dx.doi.org/10.1038/srep26537 http://www.nature.com/articles/srep26537},
volume = {6},
year = {2016}
}

@article{Soubiran2020,
author = {Soubiran, Fran{\c{c}}ois and Militzer, Burkhard},
doi = {10.1103/PhysRevLett.125.175701},
issn = {0031-9007},
journal = {Physical Review Letters},
keywords = {doi:10.1103/PhysRevLett.125.175701 url:https://doi},
mendeley-groups = {MgO},
month = {oct},
number = {17},
pages = {175701},
publisher = {American Physical Society},
title = {{Anharmonicity and Phase Diagram of Magnesium Oxide in the Megabar Regime}},
url = {https://doi.org/10.1103/PhysRevLett.125.175701 https://link.aps.org/doi/10.1103/PhysRevLett.125.175701},
volume = {125},
year = {2020}
}

@article{Bouchet2019,
author = {Bouchet, J. and Bottin, F. and Recoules, V. and Remus, F. and Morard, G. and Bolis, R. M. and Benuzzi-Mounaix, A.},
doi = {10.1103/PhysRevB.99.094113},
issn = {2469-9950},
journal = {Physical Review B - Condensed Matter and Materials Physics},
keywords = {doi:10.1103/PhysRevB.99.094113 url:https://doi.org},
mendeley-groups = {MgSiO3,MgO},
month = {mar},
number = {9},
pages = {094113},
publisher = {American Physical Society},
title = {{Ab initio calculations of the B1-B2 phase transition in MgO}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.99.094113},
volume = {99},
year = {2019}
}

@article{Simon1953melting,
  title={The melting of iron at high pressures},
  author={Simon, FE},
  journal={Nature},
  volume={172},
  number={4382},
  pages={746--747},
  year={1953},
  publisher={Nature Publishing Group}
}

@inproceedings{Hanshaw2012,
author = {Hanshaw, Heath and Martin, Matthew R. and Desjarlais, Michael and Lemke, Raymond W.},
booktitle = {AIP Conference Proceedings},
doi = {10.1063/1.3686428},
file = {:Users/fgonzalez/Library/Application Support/Mendeley Desktop/Downloaded/1.3686428.pdf:pdf},
isbn = {9780735410060},
issn = {0094243X},
keywords = {Z,aluminum,double shock,quartz},
mendeley-groups = {Beryllium},
pages = {921--924},
title = {{Double shock experiments on the sandia z machine}},
url = {http://aip.scitation.org/doi/abs/10.1063/1.3686428},
volume = {1426},
year = {2012}
}
@article{Migliori2004b,
author = {Migliori, Albert and Ledbetter, Hassel and Thoma, D. J. and Darling, T. W.},
doi = {10.1063/1.1644633},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.1644633.pdf:pdf},
issn = {00218979},
journal = {Journal of Applied Physics},
number = {5},
pages = {2436--2440},
title = {{Beryllium's monocrystal and polycrystal elastic constants}},
volume = {95},
year = {2004}
}
@article{Wilson1998,
abstract = {Capsules with beryllium ablators have long been considered as alternatives to plastic for the National Ignition Facility laser [J. A. Paisner et al., Laser Focus World 30, 75 (1994)]; now the superior performance of beryllium is becoming well substantiated. Beryllium capsules have the advantages of high density, low opacity, high tensile strength, and high thermal conductivity. Three-dimensional (3-D) calculations with the HYDRA code [NTIS Document No. DE-96004569 (M. M. Marinak et al. in UCRL-LR-105821-95-3)] confirm two-dimensional (2-D) LASNEX [G. B. Zimmerman and W. L. Kruer, Comments Plasmas Phys. Controlled Thermonucl. Fusion 2, 51 (1975)] results that particular beryllium capsule designs are several times less sensitive than the CH point design to instability growth from deuterium-tritium (DT) ice roughness. These capsule designs contain more ablator mass and leave some beryllium unablated at ignition. By adjusting the level of copper dopant, the unablated mass can increase or decrease, with a corresponding decrease or increase in sensitivity to perturbations. A plastic capsule with the same ablator mass as the beryllium and leaving the same unablated mass also shows this reduced perturbation sensitivity. Beryllium's low opacity permits the creation of 250 eV capsule designs. Its high tensile strength allows it to contain DT fuel at room temperature. Its high thermal conductivity simplifies cryogenic fielding. {\textcopyright} 1998 American Institute of Physics.},
author = {Wilson, Douglas C. and Bradley, Paul A. and Hoffman, Nelson M. and Swenson, Fritz J. and Smitherman, David P. and Chrien, Robert E. and Margevicius, Robert W. and Thoma, D. J. and Foreman, Larry R. and Hoffer, James K. and Goldman, S. Robert and Caldwell, Stephen E. and Dittrich, Thomas R. and Haan, Steven W. and Marinak, Michael M. and Pollaine, Stephen M. and Sanchez, Jorge J.},
doi = {10.1063/1.872865},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.872865.pdf:pdf},
issn = {1070664X},
journal = {Physics of Plasmas},
number = {5 PART 1},
pages = {1953--1959},
title = {{The development and advantages of beryllium capsules for the National Ignition Facility}},
volume = {5},
year = {1998}
}



@inproceedings{Swift2004b,
  title={Equation of state measurements for beryllium in the ICF capsule regime},
  author={Swift, Damian and Paisley, Dennis and Knudson, Marcus},
  booktitle={AIP Conference Proceedings},
  volume={706},
  pages={119--122},
  year={2004},
  organization={American Institute of Physics}
}


@inproceedings{Chhabildas2009,
author = {Chhabildas, L. C. and Wise, J. L. and Asay, J. R.},
booktitle = {AIP Conference Proceeding Volume 78},
doi = {10.1063/1.33351},
isbn = {7804220553},
pages = {422--426},
publisher = {AIP},
title = {{Reshock and release behavior of beryllium}},
url = {http://aip.scitation.org/doi/abs/10.1063/1.33350 http://aip.scitation.org/doi/abs/10.1063/1.33351},
volume = {422},
year = {1982}
}

@inproceedings{Wise2009,
author = {Wise, J. L. and Chhabildas, L. C. and Asay, J. R.},
booktitle = {AIP Conference Proceeding Volume 78},
doi = {10.1063/1.33350},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.33350.pdf:pdf},
pages = {417--421},
publisher = {AIP},
title = {{Shock compression of beryllium}},
url = {http://aip.scitation.org/doi/abs/10.1063/1.33350},
volume = {417},
year = {1982}
}


@article{DeWijs1998,
abstract = {The melting properties of aluminum are calculated from first-principles molecular-dynamics simulations using density-functional theory in the local-density approximation. We calculate a melting temperature of 890 K at zero pressure, to be compared to the experimental value of 933 K. An elaborate discussion of the techniques employed is presented. The solid- and liquid-state free energies are obtained via coupling constant integration. The respective reference systems are the quasiharmonic crystal and the Lennard-Jones fluid. Good quality of the Brillouin zone sampling is shown to be crucial. The strategy followed is expected to be applicable to a wide range of liquid metals. {\textcopyright} 1998 The American Physical Society.},
author = {de Wijs, Gilles A. and Kresse, Georg and Gillan, Michael J.},
doi = {10.1103/PhysRevB.57.8223},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevB.57.8223.pdf:pdf},
issn = {1550235X},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {14},
pages = {8223--8234},
title = {{First-order phase transitions by first-principles free-energy calculations: The melting of Al}},
volume = {57},
year = {1998}
}


@article{Izvekov2004a,
author = {Izvekov, Sergei and Parrinello, Michele and Bumham, Christian J. and Voth, Gregory A.},
doi = {10.1063/1.1739396},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/TDI/1.1739396.pdf:pdf},
issn = {00219606},
journal = {Journal of Chemical Physics},
number = {23},
pages = {10896--10913},
title = {{Effective force fields for condensed phase systems from ab initio molecular dynamics simulation: A new method for force-matching}},
volume = {120},
year = {2004}
}


@inproceedings{GonzalezMilitzer2020,
archivePrefix = {arXiv},
arxivId = {2002.12163},
author = {Gonz{\'{a}}lez-Cataldo, Felipe and Militzer, Burkhard},
booktitle = {AIP Conference Proceedings},
doi = {10.1063/12.0000793},
eprint = {2002.12163},
file = {:Users/fgonzalez/Library/Application Support/Mendeley Desktop/Downloaded/12.0000793.pdf:pdf},
isbn = {9780735440005},
pages = {090001},
title = {{Thermal and pressure ionization in warm, dense MgSiO$_3$ studied with first-principles computer simulations}},
url = {http://arxiv.org/abs/2002.12163 http://aip.scitation.org/doi/abs/10.1063/12.0000793},
volume = {2272},
year = {2020}
}

@article{Gonzalez-Cataldo2014,
author = {Gonz{\'{a}}lez-Cataldo, Felipe and Wilson, Hugh F. and Militzer, Burkhard},
doi = {10.1088/0004-637X/787/1/79},
issn = {0004-637X},
journal = {The Astrophysical Journal},
keywords = {color figures,dynamical evolution and stability,individual,interiors,jupiter,online-only material,planets and satellites,saturn},
mendeley-groups = {Metallic H,SiO2 Solubility,Free Energy},
month = {may},
number = {1},
pages = {79},
title = {{Ab Initio Free Energy Calculations of the Solubility of Silica in Metallic Hydrogen and Application To Giant Planet Cores}},
url = {http://stacks.iop.org/0004-637X/787/i=1/a=79?key=crossref.8ed04244b9a9a55eefbe9b400819222b},
volume = {787},
year = {2014}
}

@article{Militzer2020,
author = {Militzer, Burkhard and Gonz{\'{a}}lez-Cataldo, Felipe and Zhang, Shuai and Whitley, Heather D and Swift, Damian C and Millot, Marius},
doi = {10.1063/5.0023232},
issn = {0021-9606},
journal = {The Journal of Chemical Physics},
month = {nov},
number = {18},
pages = {184101},
publisher = {AIP Publishing, LLC},
title = {{Nonideal mixing effects in warm dense matter studied with first-principles computer simulations}},
url = {https://doi.org/10.1063/5.0023232 http://aip.scitation.org/doi/10.1063/5.0023232},
volume = {153},
year = {2020}
}

@article{Gonzalez-Cataldo2020,
archivePrefix = {arXiv},
arxivId = {2008.08459},
author = {Gonz{\'{a}}lez-Cataldo, Felipe and Soubiran, Fran{\c{c}}ois and Militzer, Burkhard},
doi = {10.1063/5.0017555},
eprint = {2008.08459},
issn = {1070-664X},
journal = {Physics of Plasmas},
mendeley-groups = {PIMC},
month = {sep},
number = {9},
pages = {092706},
publisher = {AIP Publishing LLC},
title = {{Equation of state of hot, dense magnesium derived with first-principles computer simulations}},
url = {http://aip.scitation.org/doi/10.1063/5.0017555 http://arxiv.org/abs/2008.08459},
volume = {27},
year = {2020}
}


@article{Soubiran2019,
author = {Soubiran, Fran{\c{c}}ois and Gonz{\'{a}}lez-Cataldo, Felipe and Driver, Kevin P and Zhang, Shuai and Militzer, Burkhard},
doi = {10.1063/1.5126624},
issn = {0021-9606},
journal = {The Journal of Chemical Physics},
mendeley-groups = {MgO},
month = {dec},
number = {21},
pages = {214104},
publisher = {AIP Publishing, LLC},
title = {{Magnesium oxide at extreme temperatures and pressures studied with first-principles simulations}},
url = {https://doi.org/10.1063/1.5126624 http://aip.scitation.org/doi/10.1063/1.5126624},
volume = {151},
year = {2019}
}



@article{Gonzalez2020,
author = {Gonz{\'{a}}lez-Cataldo, Felipe and Soubiran, Fran{\c{c}}ois and Peterson, Henry and Militzer, Burkhard},
doi = {10.1103/PhysRevB.101.024107},
issn = {2469-9950},
journal = {Physical Review B},
mendeley-groups = {MgSiO3},
month = {jan},
number = {2},
pages = {024107},
title = {{Path integral Monte Carlo and density functional molecular dynamics simulations of warm dense MgSiO$_3$}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.101.024107},
volume = {101},
year = {2020}
}


@inproceedings{Gonzalez-Cataldo2018,
author = {Gonz{\'{a}}lez-Cataldo, Felipe and Corvacho, Fernando and Guti{\'{e}}rrez, Gonzalo},
booktitle = {Journal of Physics: Conference Series},
doi = {10.1088/1742-6596/1043/1/012038},
file = {:Users/fgonzalez/Library/Application Support/Mendeley Desktop/Downloaded/Gonz{\'{a}}lez-Cataldo, Corvacho, Guti{\'{e}}rrez - 2018 - Journal of Physics Conference Series.pdf:pdf},
issn = {1742-6588},
mendeley-groups = {LPMD,Melting Si},
month = {jun},
pages = {012038},
title = {{Melting curve of Si by means of the Z-method}},
url = {http://stacks.iop.org/1742-6596/1043/i=1/a=012038?key=crossref.9e5375dd24819db67a210b37d1a22de3},
volume = {1043},
year = {2018}
}



@Book{allen-tildesley-87,
   Author = {Allen, M.P. and Tildesley, D.J.},
   Title = {{Computer Simulation of Liquids}},
   Publisher = {Oxford: Clarendon Pr},
   Year = {1987}
}


@book{dfrenkel96:mc,
  abstract = {An advanced text on the physics and computation of
                  atomistic simulations. Chapter titles are:
                  introduction; statistical mechanics; Monte Carlo
                  simulations; molecular dynamics simulations; Monte
                  Carlo simulations in various ensembles; molecular
                  dynamics in various ensembles; free energy
                  calculations; the Gibbs ensemble; other methods to
                  study coexistence; free energies of solids; free
                  energy of chain molecules; long-range interactions;
                  biased Monte Carlo schemes; accelerating Monte Carlo
                  sampling; tackling time-scale problems; rare events;
                  dissipative particle dynamics. Appendices are
                  entitled: (the) Lagrangian and Hamiltonian;
                  non-Hamiltonian dynamics; linear response theory;
                  statistical errors; integration schemes; saving CPU
                  time; reference states; statistical mechanics of the
                  Gibbs ``ensemble''; overlapping distribution for
                  polymers; some general purpose algorithms; small
                  research projects; hints for programming.},
  added-at = {2013-03-21T02:24:53.000+0100},
  address = {San Diego},
  annote = {Series editors: D. Frenkel, M. Klein, M. Parrinello                  and B. Smit. First edition published in 1996.},
  author = {Frenkel, Daan and Smit, Berend},
  biburl = {https://www.bibsonomy.org/bibtex/27058bda2c1d06e4718bf4fe7a9e5b1d0/drmatusek},
  edition = {Second},
  interhash = {3e1272dc52ef1545e92ab3973adf0f18},
  intrahash = {7058bda2c1d06e4718bf4fe7a9e5b1d0},
  keywords = {Carlo Monte dynamics fortran mechanics molecular physics programming statistical},
  publisher = {Academic Press},
  series = {Computational Science Series},
  timestamp = {2013-03-21T02:24:54.000+0100},
  title = {Understanding Molecular Simulation: From Algorithms to
                  Applications},
  volume = 1,
  year = 2002
}


@article{Militzer2021,
  title = {First-principles equation of state database for warm dense matter computation},
  author = {Militzer, Burkhard and Gonz\'alez-Cataldo, Felipe and Zhang, Shuai and Driver, Kevin P. and Soubiran, Fran\ifmmode \mbox{\c{c}}\else \c{c}\fi{}ois},
  journal = {Phys. Rev. E},
  volume = {103},
  issue = {1},
  pages = {013203},
  numpages = {13},
  year = {2021},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.103.013203},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.103.013203}
}

@inproceedings{knudson2012megaamps,
  title={Megaamps, megagauss, and megabars: Using the Sandia Z Machine to perform extreme material dynamics experiments},
  author={Knudson, Marcus D},
  booktitle={AIP Conference Proceedings},
  volume={1426},
  pages={35--42},
  year={2012},
  organization={American Institute of Physics}
}

@article{Baskes1987a,
abstract = {The embedded-atom method, a semiempirical theory of metal bonding, is investigated as a method to calculate the bonding in a covalent material. A simple first-neighbor embedded-atom method model is sufficient to explain the geometry and structure of many metastable phases of silicon, but not its shear behavior. To obtain realistic shear behavior of silicon, an angle-dependent electron density is included to model the effects of bond bending. This model uses only the experimental bulk properties of silicon. Calculated properties of metastable phases and point defects are presented. {\textcopyright} 1987 The American Physical Society.},
author = {Baskes, M. I.},
doi = {10.1103/PhysRevLett.59.2666},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevLett.59.2666.pdf:pdf},
issn = {00319007},
journal = {Physical Review Letters},
number = {23},
pages = {2666--2669},
title = {{Application of the Embedded-Atom Method to Covalent Materials: A Semiempirical Potential for Silicon}},
volume = {59},
year = {1987}
}
@article{Baskes1989a,
abstract = {Semiempirical potentials for silicon, germanium, and their alloys are derived with use of the modified-embedded-atom-method formalism. Following Baskes [Phys. Rev. Lett. 59, 2666 (1987)], it is found that the host electron density which is a linear superposition of atomic densities in the embedded-atom method (EAM) must have an angular modification in order to properly describe the bond-bending forces in the diamond-cubic structure. The angular dependence of this host electron density was found to be in qualitative agreement with the density of a first-principles calculation. As in the EAM, the potential functions are determined by using the measured lattice constants, sublimation energies, elastic constants, and alloying energies of silicon and germanium. In addition, first-principles calculations of structural energies are used. The potentials are used to calculate the energetics and geometrics of point defects, surfaces, metastable structures, and small clusters. In all cases, the calculations have been compared to first-principles calculations and experiment when available. The calculations predict that the vacancy mechanism is the dominant diffusion mechanism in both silicon and germanium. Surface energies and relaxations of the low-index faces of Si and Ge are compared with first-principles calculations. {\textcopyright} 1989 The American Physical Society.},
author = {Baskes, M. I. and Nelson, J. S. and Wright, A. F.},
doi = {10.1103/PhysRevB.40.6085},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevB.40.6085.pdf:pdf},
issn = {01631829},
journal = {Physical Review B},
number = {9},
pages = {6085--6100},
title = {{Semiempirical modified embedded-atom potentials for silicon and germanium}},
volume = {40},
year = {1989}
}
@article{Baskes1992,
abstract = {In a comprehensive study, the modified embedded-atom method is extended to a variety of cubic materials and impurities. In this extension, all functions are analytic and computationally simple. The basic equations of the method are developed and applied to 26 elements: ten fcc, ten bcc, three diamond cubic, and three gaseous materials. The materials modeled include metals, semiconductors, and diatomic gases, all of which exhibit different types of bonding. Properties of these materials, including equation of state, elastic moduli, structural energies and lattice constants, simple defects, and surfaces, are calculated. The formalism for applying the method to combinations of these elements is developed and applied to the calculation of dilute heats of solution. In all cases, comparison is made to experiment or higher-level calculations when possible. {\textcopyright} 1992 The American Physical Society.},
author = {Baskes, M. I.},
doi = {10.1103/PhysRevB.46.2727},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/VirtualMelting/MEAM/PhysRevB.46.2727.pdf:pdf},
issn = {01631829},
journal = {Physical Review B},
number = {5},
pages = {2727--2742},
title = {{Modified embedded-atom potentials for cubic materials and impurities}},
volume = {46},
year = {1992}
}
@article{He2013,
abstract = {We perform large-scale molecular dynamics simulations to study shock-induced melting transition of idealized hexagonal columnar nanocrystalline Cu. The as-constructed nanocrystalline Cu consists of unrotated (reference) and rotated columnar crystals, relative to the columnar axis. Shock loading is applied along three principal directions of the columnar Cu: two transverse (zigzag and armchair) and one longitudinal directions. Dynamic local melting processes are highly anisotropic with respect to the shock directions. For the transverse directions, hotspot effect and disparate dynamic responses of grains with different orientations may lead to partial or complete premelting of the initially rotated grains, which in turn leads to transient supercooling and heterogeneous recrystallization, and thus, the formation of nanocrystalline solids with modified grain structures or solid-liquid mixtures, depending on the extent of supercooling. With increasing shock strengths, the reference grains melt heterogeneously at interfaces and homogeneously inside. Conversely, "bulk" premelting of the rotated grains is absent for the longitudinal direction, except for grain boundary melting. The progression of recrystallization or heterogenous melting diminishes and eventually eliminates the transient premelting or superheating of the system via latent heat and thermal diffusion. Premelting or superheating appears unlikely for bulk melting or well-defined Hugoniot states, if the thermal and mechanical equilibria are achieved, and the thermodynamic melting curve coincides with the partial melting Hugoniot states of a polycrystalline solid. {\textcopyright} 2013 AIP Publishing LLC.},
author = {He, A. M. and Duan, S. Q. and Shao, J. L. and Wang, P. and Luo, S. N.},
doi = {10.1063/1.4818336},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/VirtualMelting/1.4818336.pdf:pdf},
issn = {00219606},
journal = {Journal of Chemical Physics},
number = {7},
title = {{Local and bulk melting of shocked columnar nanocrystalline Cu: Dynamics, anisotropy, premelting, superheating, supercooling, and re-crystallization}},
volume = {139},
year = {2013}
}

@article{Budzevich2012,
author = {Budzevich, Mikalai M. and Zhakhovsky, Vasily V. and White, Carter T. and Oleynik, Ivan I.},
doi = {10.1103/PhysRevLett.109.125505},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/VirtualMelting/PhysRevLett.109.125505.pdf:pdf},
issn = {00319007},
journal = {Physical Review Letters},
number = {12},
pages = {1--5},
title = {{Evolution of shock-induced orientation-dependent metastable states in crystalline aluminum}},
volume = {109},
year = {2012}
}
@article{He2014,
abstract = {Solid-liquid phase transitions in single crystal Cu during shock and subsequent release are studied with large-scale classical molecular dynamics simulations. During shock compression, although the equilibrium states far behind shock front converge to the same Hugoniot, the pathways from metastable states right behind the shock front to the final equilibrium states and the resulting microstructures are orientation-dependent. Premelting is followed by recrystallization of supercooled melt into a polycrystalline solid for the [110] and [111] shocks, and a superheated, more ordered, solid is observed prior to shock melting for the [100] shock. The differences in the microstructure in the behind-shock region in turn give rise to different release melting behaviors (including premelting and superheating) along different release paths for these loading orientations. {\textcopyright} 2014 AIP Publishing LLC.},
author = {He, A. M. and Wang, P. and Shao, J. L. and Duan, S. Q. and Zhao, F. P. and Luo, S. N.},
doi = {10.1063/1.4871230},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/VirtualMelting/1.4871230.pdf:pdf},
issn = {10897550},
journal = {Journal of Applied Physics},
number = {14},
title = {{Solid-liquid phase transitions in single crystal Cu under shock and release conditions}},
volume = {115},
year = {2014}
}
@article{Levitas2012,
author = {Levitas, Valery I. and Ravelo, Ramon},
doi = {10.1073/pnas.1203285109},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/VirtualMelting/Font2015{\_}Article{\_}AMathematicalModelForNanoparti.pdf:pdf},
issn = {00278424},
journal = {Proceedings of the National Academy of Sciences of the United States of America},
keywords = {High strain-rate plasticity,Relaxation of non-hydrostatic stresses,Thermodynamics under uniaxial straining},
number = {33},
pages = {13204--13207},
title = {{Virtual melting as a new mechanism of stress relaxation under high strain rate loading}},
volume = {109},
year = {2012}
}
@article{Simak2000,
abstract = {A study was carried out to explore the structural competition between the high symmetry fcc and low symmetry bct structure for the IIIA metals Al, Ga, and In. It was found that the competition originates from electronic properties. As a result, the high pressure behavior of the metals appears reversed to the corresponding-states rule.},
author = {Simak, S. I. and H{\"{a}}ussermann, U. and Ahuja, R. and Lidin, S. and Johansson, B.},
doi = {10.1103/PhysRevLett.85.142},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/caratio/1.1698252-annotated.pdf:pdf},
issn = {00319007},
journal = {Physical Review Letters},
number = {1},
pages = {142--145},
title = {{Gallium and indium under high pressure}},
volume = {85},
year = {2000}
}
@article{Haussermann2001a,
abstract = {The origin of the (formula presented) variation in hcp divalent metals (Be, Mg, Zn, and Cd), which ranges from 1.568 to 1.886, has been investigated by first-principles full-potential calculations in the framework of the density functional theory. We find that the ideal hcp structure (formula presented) is electronically unstable to (formula presented) distortions for all elements, however the distortion driving band energy is countered by the electrostatic part of the total energy, which favors the ideal close packing. In particular, Zn and Cd with (formula presented) ratios (formula presented) ideal follow the bonding principle of optimum hybridization between s and p valence bands, a situation similar to the metallic elements in the neighboring group-IIIa in the Periodic Table. For Mg the electronic instability is not effective because the electrostatic part of the total energy dominates over the band energy. However, under expansion a distortion to (formula presented) ratios (formula presented) ideal occurs. Finally, Be represents a special case. Typically of second-row elements, s and p valence bands mix intimately which creates an electronic structure quite distinguished from the other divalent metals. A (formula presented) distortion cannot improve (formula presented) band hybridization but (formula presented) bonding is increased for (formula presented) ideal. {\textcopyright} 2001 The American Physical Society.},
author = {H{\"{a}}ussermann, U. and Simak, S. I.},
doi = {10.1103/PhysRevB.64.245114},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevB.64.245114.pdf:pdf},
issn = {1550235X},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {24},
pages = {1--10},
title = {{Origin of the (formula presented) variation in hexagonal close-packed divalent metals}},
volume = {64},
year = {2001}
}

@article{Pistorius1976,
author = {Pistorius, Carl W.F.T.},
doi = {10.1016/0079-6786(76)90012-1},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Exp/1-s2.0-0079678676900121-main.pdf:pdf},
issn = {00796786},
journal = {Progress in Solid State Chemistry},
number = {PART 1},
pages = {1--151},
title = {{Phase relations and structures of solids at high pressures}},
volume = {11},
year = {1976}
}


@inproceedings{mcmahan1982alpha,
  title={{The $\alpha$-$\beta$ transition in $T= O$ high pressure beryllium}},
  author={McMahan, AK},
  booktitle={AIP Conference Proceedings},
  volume={78},
  pages={340--344},
  year={1982},
  organization={American Institute of Physics}
}


@article{Meyer-Ter-Vehn1988,
abstract = {This paper is concerned with the effect of atomic-shell structure on the cold pressure of highly compressed matter up to 1 Gbar and above. The method is to compare band-structure calculations based on augmented spherical waves with results of the quantum-statistical model. Elements treated explicitly are Li, He, Be, Al, and K. No indication for anomalies due to pressure ionization is found. However, an oscillatory behavior of cold-pressure curves is systematically obtained due to isostructural electronic transitions. They are traced back to pressure-induced band shifts and electron redistribution from bands of low angular momentum (typically s and p waves) to bands of higher angular momentum (typically d and f waves). The shifts are shown to occur generally when squeezing normal matter with extended atoms into highly degenerate matter. The anomalies are particularly pronounced for alkali metals: Strong pressure flattening is found for Li at fivefold compression and 510 Mbar, and very sharply for K somewhat below fivefold compression and 500 kbar. The oscillations are much weaker for Be and Al. Metallization of He is obtained at 12.1 g/cm3 and 110 Mbar. For Be, a structural hcp bcc transition at 2 Mbar is predicted. {\textcopyright} 1988 The American Physical Society.},
author = {Meyer-Ter-Vehn, J. and Zittel, W.},
doi = {10.1103/PhysRevB.37.8674},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Theoretical Predictions/hybridisation/PhysRevB.37.8674.pdf:pdf},
issn = {01631829},
journal = {Physical Review B},
number = {15},
pages = {8674--8688},
title = {{Electronic structure of matter at high compression: Isostructural transitions and approach of the fermi-gas limit}},
volume = {37},
year = {1988}
}

@article{Lam1984,
abstract = {Beryllium is known to undergo a HCP-BCC transition at about 1530K and ambient pressure. This transition is studied theoretically by comparing the Gibbs free energies for the HCP, FCC and BCC modifications of Be. The static lattice energy is calculated using the ab initio pseudopotential method. The photon energy and entropy are estimated from the calculated elastic constants. A mechanism for this transition is proposed based on the results of the calculations. At high temperature, the BCC modification is found to be stabilised by the large entropy for this phase caused by the presence of soft phonon modes. Possible pressure-induced phase transitions are examined. At about 1-2 Mbar the FCC and BCC phases are both more stable than the HCP phase. The regions of FCC and BCC stability lie too close to be separated in the present calculation.},
author = {Lam, P. K. and Chou, M. Y. and Cohen, M. L.},
doi = {10.1088/0022-3719/17/12/006},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/P{\_}K{\_}Lam{\_}1984{\_}J.{\_}Phys.{\_}C{\_}{\_}Solid{\_}State{\_}Phys.{\_}17{\_}2065.pdf:pdf},
issn = {00223719},
journal = {Journal of Physics C: Solid State Physics},
number = {12},
pages = {2065--2073},
title = {{Temperature- and pressure-induced crystal phase transitions in Be}},
volume = {17},
year = {1984}
}
@article{francois1965conference,
  title={Conference Internationale sur la Metallurgie du Beryllium},
  author={Francois, M and Contre, M},
  journal={Universite de France, Grenoble, Paris},
  year={1965}
}
@techreport{abey1984pressure,
  title={Pressure phase lines and enthalpies for the. cap alpha.-. beta. and. beta.-liquid transitions in beryllium},
  author={Abey, Albert},
  year={1984},
  institution={Lawrence Livermore National Lab., CA (USA)}
}

@article{Olijnyk2000,
abstract = {Raman spectra of Be were studied at room temperature at pressures up to 23 GPa. The transverse-optical (TO) zone-centre phonon mode of hcp Be could be observed to maximum pressure. Neither new modes nor anomalies in the pressure shift were observed in the pressure range of 8.6-14.5 GPa where a phase transition has been reported. The TO mode frequency and its pressure dependence are discussed in terms of the elastic properties of Be.},
author = {Olijnyk, H. and Jephcoat, A. P.},
doi = {10.1088/0953-8984/12/41/317},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Exp/H{\_}Olijnyk{\_}2000{\_}J.{\_}Phys.{\_}{\_}Condens.{\_}Matter{\_}12{\_}8913.pdf:pdf},
issn = {09538984},
journal = {Journal of Physics Condensed Matter},
number = {41},
pages = {8913--8918},
title = {{Raman spectra of beryllium to 23 GPa}},
volume = {12},
year = {2000}
}
@article{kadas2007structural,
  title={Structural stability of $\beta$-beryllium},
  author={K{\'a}das, Krisztina and Vitos, Levente and Johansson, B{\"o}rje and Koll{\'a}r, J},
  journal={Physical Review B},
  volume={75},
  number={3},
  pages={035132},
  year={2007},
  publisher={APS}
}
@article{Peterson2014,
abstract = {Defects on inertial confinement fusion capsule surfaces can seed hydrodynamic instability growth and adversely affect capsule performance. The dynamics of shocks launched during the early period of x-ray driven National Ignition Facility (NIF) implosions determine whether perturbations will grow inward or outward at peak implosion velocity and final compression. In particular, the strength of the first shock, launched at the beginning of the laser pulse, plays an important role in determining Richtmyer-Meshkov (RM) oscillations on the ablation front. These surface oscillations can couple to the capsule interior through subsequent shocks before experiencing Rayleigh-Taylor (RT) growth. We compare radiation hydrodynamic simulations of NIF implosions to analytic theories of the ablative RM and RT instabilities to illustrate how early time laser strength can alter peak velocity growth. We develop a model that couples the RM and RT implosion phases and captures key features of full simulations. We also show how three key parameters can control the modal demarcation between outward and inward growth.},
author = {Peterson, J. L. and Clark, D. S. and Masse, L. P. and Suter, L. J.},
doi = {10.1063/1.4896708},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.4896708.pdf:pdf},
issn = {10897674},
journal = {Physics of Plasmas},
number = {9},
title = {{The effects of early time laser drive on hydrodynamic instability growth in National Ignition Facility implosions}},
url = {http://dx.doi.org/10.1063/1.4896708},
volume = {21},
year = {2014}
}
@article{Duff2015c,
abstract = {Thermodynamic properties of ZrC are calculated up to the melting point (Tmelt≈3700K), using density functional theory (DFT) to obtain the fully anharmonic vibrational contribution, and including electronic excitations. A significant improvement is found in comparison to results calculated within the quasiharmonic approximation. The calculated thermal expansion is in better agreement with experiment and the heat capacity reproduces rather closely a CALPHAD estimate. The calculations are presented as an application of a development of the upsampled thermodynamic integration using Langevin dynamics (UP-TILD) approach. This development, referred to here as two-stage upsampled thermodynamic integration using Langevin dynamics (TU-TILD), is the inclusion of tailored interatomic potentials to characterize an intermediate reference state of anharmonic vibrations on a two-stage path of thermodynamic integration between the original DFT quasiharmonic free energy and the fully anharmonic DFT free energy. This approach greatly accelerates the convergence of the calculation, giving a factor of improvement in efficiency of ∼50 in the present case compared to the original UP-TILD approach, and it can be applied to a wide range of materials.},
author = {Duff, Andrew Ian and Davey, Theresa and Korbmacher, Dominique and Glensk, Albert and Grabowski, Blazej and Neugebauer, J{\"{o}}rg and Finnis, Michael W.},
doi = {10.1103/PhysRevB.91.214311},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevB.91.214311.pdf:pdf},
issn = {1550235X},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {21},
pages = {1--8},
title = {{Improved method of calculating ab initio high-temperature thermodynamic properties with application to ZrC}},
volume = {91},
year = {2015}
}
@article{bzel1966physics,
  title={Physics of shock waves and high temperature hydrodinamic phenomena Academic Press},
  author={BZel’dovic, Ya and Raizer, Yu P},
  journal={New York},
  year={1966}
}
@article{Monserrat2013b,
abstract = {A unified approach is used to study vibrational properties of periodic systems with first-principles methods and including anharmonic effects. Our approach provides a theoretical basis for the determination of phonon-dependent quantities at finite temperatures. The low-energy portion of the Born-Oppenheimer energy surface is mapped and used to calculate the total vibrational energy including anharmonic effects, electron-phonon coupling, and the vibrational contribution to the stress tensor. We report results for the temperature dependence of the electronic band gap and the linear coefficient of thermal expansion of diamond, lithium hydride, and lithium deuteride.},
author = {Monserrat, Bartomeu and Drummond, N. D. and Needs, R. J.},
doi = {10.1103/PhysRevB.87.144302},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Monserrat, Drummond, Needs - 2013 - Anharmonic vibrational properties in periodic systems Energy, electron-phonon coupling, and stress.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {14},
pages = {1--10},
title = {{Anharmonic vibrational properties in periodic systems: Energy, electron-phonon coupling, and stress}},
volume = {87},
year = {2013}
}

@article{wallace1972thermodynamics,
  title={Thermodynamics of crystals},
  author={Wallace, Duane C},
  journal={American Journal of Physics},
  volume={40},
  number={11},
  pages={1718--1719},
  year={1972},
  publisher={American Association of Physics Teachers}
}
@article{rudindensity,
  title={Density Functional Theory Calculations on EOS and Phase Stability of Beryllium},
  author={Rudin, Sven P and Jones, MD and Johnson, JD},
  journal={Joint 20th AIRAPT--43th EHPRG, June}
}
@article{flyvbjerg1989error,
  title={Error estimates on averages of correlated data},
  author={Flyvbjerg, Henrik and Petersen, Henrik Gordon},
  journal={The Journal of Chemical Physics},
  volume={91},
  number={1},
  pages={461--466},
  year={1989},
  publisher={American Institute of Physics}
}
@article{Graf2004,
abstract = {The lattice vibrations are determined in the quasi-harmonic approximation for elemental Au and Cu to twice their normal density by first-principles electronic band-structure calculations. It is found for these materials that the important moments of the phonon density of states can be obtained to high accuracy from short-ranged force constant models. We discuss the implications for the Grueneisen parameters on the basis of calculated phonon moments and their approximations by using bulk moduli and Debye-Waller factors.},
author = {Graf, Matthias J.},
doi = {10.1063/1.1780185},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/GruneisenPhononMoment/1.1780185.pdf:pdf},
isbn = {0735401810},
number = {August 2004},
pages = {65--68},
title = {{High-Pressure Debye-Waller and Gr{\"{u}}neisen Parameters of Gold and Copper}},
volume = {65},
year = {2004}
}


@article{Navascues2010,
author = {Navascu{\'{e}}s, G. and Velasco, E.},
issn = {0021-9606},
journal = {The Journal of Chemical Physics},
mendeley-groups = {Free Energy},
month = {apr},
number = {13},
pages = {134106},
title = {{Free-energy correction due to center-of-mass constraint in crystals}},
url = {http://aip.scitation.org/doi/10.1063/1.3372805},
volume = {132},
year = {2010}
}



@article{anderson2000calculated,
  title={Calculated melting curves for phases of iron},
  author={Anderson, Orson L and Isaak, Donald G},
  journal={American Mineralogist},
  volume={85},
  number={2},
  pages={376--385},
  year={2000},
  publisher={Mineralogical Society of America}
}
@article{gilvarry1956lindemann,
  title={The Lindemann and Gr{\"u}neisen laws},
  author={Gilvarry, John James},
  journal={Physical Review},
  volume={102},
  number={2},
  pages={308},
  year={1956},
  publisher={APS}
}
@article{mermin1965thermal,
  title={Thermal properties of the inhomogeneous electron gas},
  author={Mermin, N David},
  journal={Physical Review},
  volume={137},
  number={5A},
  pages={A1441},
  year={1965},
  publisher={APS}
}
@article{baroni2001phonons,
  title={Phonons and related crystal properties from density-functional perturbation theory},
  author={Baroni, Stefano and De Gironcoli, Stefano and Dal Corso, Andrea and Giannozzi, Paolo},
  journal={Reviews of modern Physics},
  volume={73},
  number={2},
  pages={515},
  year={2001},
  publisher={APS}
}

@article{hellman2011lattice,
  title={Lattice dynamics of anharmonic solids from first principles},
  author={Hellman, Olle and Abrikosov, IA and Simak, SI},
  journal={Physical Review B},
  volume={84},
  number={18},
  pages={180301},
  year={2011},
  publisher={APS}
}


@article{Migliori2004c,
author = {Migliori, Albert and Ledbetter, Hassel and Thoma, D. J. and Darling, T. W.},
doi = {10.1063/1.1644633},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Exp/1.1644633.pdf:pdf},
issn = {00218979},
journal = {Journal of Applied Physics},
number = {5},
pages = {2436--2440},
title = {{Beryllium's monocrystal and polycrystal elastic constants}},
volume = {95},
year = {2004}
}

@article{lyon1992sesame,
  title={Sesame: the Los Alamos National Laboratory equation of state database},
  author={Lyon, Stanford P},
  journal={Los Alamos National Laboratory report LA-UR-92-3407},
  year={1992}
}
@article{PhysRevLett.104.121101,
  title = {Sequestration of Noble Gases in Giant Planet Interiors},
  author = {Wilson, Hugh F. and Militzer, Burkhard},
  journal = {Phys. Rev. Lett.},
  volume = {104},
  issue = {12},
  pages = {121101},
  numpages = {4},
  year = {2010},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.104.121101},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.104.121101}
}
@article{Grabowski2009a,
abstract = {We propose a fully ab initio based integrated approach to determine the volume and temperature dependent free-energy surface of nonmagnetic crystalline solids up to the melting point. The approach is based on density-functional theory calculations with a controlled numerical accuracy of better than 1 meV/atom. It accounts for all relevant excitation mechanisms entering the free energy including electronic, quasiharmonic, anharmonic, and structural excitations such as vacancies. To achieve the desired accuracy of {\textless}1 meV/atom for the anharmonic free-energy contribution without losing the ability to perform these calculations on standard present-day computer platforms, we develop a numerically highly efficient technique: we propose a hierarchical scheme-called upsampled thermodynamic integration using Langevin dynamics-which allows for a significant reduction in the number of computationally expensive ab initio configurations compared to a standard molecular dynamics scheme. As for the vacancy contribution, concentration-dependent pressure effects had to be included to achieve the desired accuracy. Applying the integrated approach gives us direct access to the free-energy surface F (V,T) for aluminum and derived quantities such as the thermal expansion coefficient or the isobaric heat capacity and allows a direct comparison with experiment. A detailed analysis enables us to tackle the long-standing debate over which excitation mechanism (anharmonicity vs vacancies) is dominant close to the melting point. {\textcopyright} 2009 The American Physical Society.},
author = {Grabowski, B. and Ismer, L. and Hickel, T. and Neugebauer, J.},
doi = {10.1103/PhysRevB.79.134106},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevB.79.134106.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {13},
pages = {1--16},
title = {{Ab initio up to the melting point: Anharmonicity and vacancies in aluminum}},
volume = {79},
year = {2009}
}

@article {phonopy,
     Journal = {Scr. Mater.},
     Year = {2015},
     Title = {First principles phonon calculations in materials science},
     Author = {Togo, A and Tanaka, I},
     Pages = {1--5},
     Volume = {108},
     Month = {Nov}
}
@article{sun2010lattice,
  title={Lattice thermal conductivity: Computations and theory of the high-temperature breakdown of the phonon-gas model},
  author={Sun, Tao and Allen, Philip B},
  journal={Physical Review B},
  volume={82},
  number={22},
  pages={224305},
  year={2010},
  publisher={APS}
}
@article{zhang2014phonon,
  title={Phonon quasiparticles and anharmonic free energy in complex systems},
  author={Zhang, Dong-Bo and Sun, Tao and Wentzcovitch, Renata M},
  journal={Physical review letters},
  volume={112},
  number={5},
  pages={058501},
  year={2014},
  publisher={APS}
}
@article{carreras2017dynaphopy,
  title={Dynaphopy: A code for extracting phonon quasiparticles from molecular dynamics simulations},
  author={Carreras, Abel and Togo, Atsushi and Tanaka, Isao},
  journal={Computer Physics Communications},
  volume={221},
  pages={221--234},
  year={2017},
  publisher={Elsevier}
}


@article{Musella2019,
abstract = {Using ab initio molecular dynamics simulations, we calculate the physical properties of MgO at conditions extending from the ones encountered in the Earth mantle up to the ones anticipated in giant planet interiors such as Jupiter. We pay particular attention to the high-pressure melting temperature throughout this large density range as this is a key ingredient for building accurate planetary interior models with a realistic description of their inner cores. We compare our simulation results with previous ab initio calculations that have been so far limited to the pressure range corresponding to the Earth mantle and the B1-B2 transition around 6 Mbar. We provide our results for both the equation of state and high-pressure melting curve in parametric forms for direct use in planetary models. Finally, we compare our predictions of the high-pressure melting temperature with various planetary interior profiles to deduce the state of differentiated layer within the core made of MgO in differentiated cores of various types of planets and exoplanets.},
archivePrefix = {arXiv},
arxivId = {1805.12439},
author = {Musella, R. and Mazevet, S. and Guyot, F.},
doi = {10.1103/PhysRevB.99.064110},
eprint = {1805.12439},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Core formation/MgO/PhysRevB.99.064110.pdf:pdf},
issn = {24699969},
journal = {Physical Review B},
keywords = {doi:10.1103/PhysRevB.99.064110 url:https://doi.org/10.1103/PhysRevB.99.064110},
number = {6},
pages = {1--8},
publisher = {American Physical Society},
title = {{Physical properties of MgO at deep planetary conditions}},
volume = {99},
year = {2019}
}

@article{Taniuchi2018,
abstract = {The melting curve of MgO is extended up to 4 TPa, corresponding to the Jovian core pressure, based on the one-step thermodynamic integration method implemented on ab initio molecular dynamics. The calculated melting temperatures are 3100 and 16 000 K at 0 and 500 GPa, respectively, which are consistent with previous experimental results, and 20 600 K at 3900 GPa, which is inconsistent with a recent experimental extrapolation, which implies the molten Jovian core. A quite small Clapeyron slope () of is found at 3900 GPa due to comparable densities of the liquid and B2 phases under extreme compression. The Mg-O coordination number in the liquid phase is saturated at around 7.5 above 1 TPa and remains smaller than that in the B2 phase (8) even at 4 TPa, suggesting no density crossover between liquid and crystal and thus no further denser crystalline phases. Dynamical properties (atomic diffusivity and viscosity) are also investigated along the melting curve to understand these behaviors in greater detail.},
author = {Taniuchi, Takashi and Tsuchiya, Taku},
doi = {10.1088/1361-648X/aaac96},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Core formation/MgO/Taniuchi{\_}2018{\_}J.{\_}Phys.{\_}{\_}Condens.{\_}Matter{\_}30{\_}114003.pdf:pdf},
issn = {1361648X},
journal = {Journal of Physics Condensed Matter},
keywords = {MgO,ab initio calculation,melting curve,thermodynamic integration},
number = {11},
pmid = {29393072},
publisher = {IOP Publishing},
title = {{The melting points of MgO up to 4 TPa predicted based on ab initio thermodynamic integration molecular dynamics}},
volume = {30},
year = {2018}
}


@book{german1996sintering,
  title={Sintering theory and practice},
  author={German, Randall M},
  year={1996}
}

@book{yefimov2009handbook,
  title={Handbook of non-ferrous metal powders: technologies and applications},
  author={Yefimov, NA},
  year={2009},
  publisher={Elsevier}
}
@article{Miyanishi2015,
abstract = {Magnesium oxide has been experimentally and computationally investigated in the warm-dense solid and liquid ranges from 200 GPa to 1 TPa along the principal Hugoniot. The linear approximation between shock velocity and particle velocity is validated up to a shock velocity of 15 km/s from the experimental data, this suggesting that the MgO B1 structure is stable up to the corresponding shock pressure of ∼350 GPa. Moreover, our Hugoniot data, combined with ab initio simulations, show two crossovers between MgO Hugoniot and the extrapolation of the linear approximation line, occurring at a shock pressures of approximately 350 and 650 GPa, with shock temperatures of 8000 and 14 000 K, respectively. These crossover regions are consistent with the solid-solid (B1-B2) and the solid-liquid (B2-melt) phase boundaries predicted by the ab initio calculations.},
author = {Miyanishi, K. and Tange, Y. and Ozaki, N. and Kimura, T. and Sano, T. and Sakawa, Y. and Tsuchiya, T. and Kodama, R.},
doi = {10.1103/PhysRevE.92.023103},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Core formation/MgO/PhysRevE.92.023103.pdf:pdf},
issn = {15502376},
journal = {Physical Review E - Statistical, Nonlinear, and Soft Matter Physics},
number = {2},
pages = {1--5},
title = {{Laser-shock compression of magnesium oxide in the warm-dense-matter regime}},
volume = {92},
year = {2015}
}
@article{Root2015,
abstract = {The moon-forming impact and the subsequent evolution of the proto-Earth is strongly dependent on the properties of materials at the extreme conditions generated by this violent collision. We examine the high pressure behavior of MgO, one of the dominant constituents in Earth's mantle, using high-precision, plate impact shock compression experiments performed on Sandia National Laboratories' Z Machine and extensive quantum calculations using density functional theory (DFT) and quantum Monte Carlo (QMC) methods. The combined data span from ambient conditions to 1.2 TPa and 42 000 K, showing solid-solid and solid-liquid phase boundaries. Furthermore our results indicate that under impact the solid and liquid phases coexist for more than 100 GPa, pushing complete melting to pressures in excess of 600 GPa. The high pressure required for complete shock melting has implications for a broad range of planetary collision events.},
author = {Root, Seth and Shulenburger, Luke and Lemke, Raymond W. and Dolan, Daniel H. and Mattsson, Thomas R. and Desjarlais, Michael P.},
doi = {10.1103/PhysRevLett.115.198501},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Core formation/MgO/PhysRevLett.115.198501.pdf:pdf},
issn = {10797114},
journal = {Physical Review Letters},
number = {19},
pages = {1--6},
title = {{Shock Response and Phase Transitions of MgO at Planetary Impact Conditions}},
volume = {115},
year = {2015}
}
@article{Cebulla2014,
abstract = {We determined the phase diagram of magnesium oxide with finite-temperature density functional theory molecular dynamics simulations up to temperatures and pressures as relevant for the deep interior of super-Earths and in rocky cores of giant planets such as Jupiter. The equation of state data, the Hugoniot, and a ramp compression curve are computed and compared to earlier results from diamond anvil cell and (decaying) shock wave experiments. In addition, the dynamical electrical conductivity and the reflectivity along the experimental Hugoniot curve are calculated in order to characterize electronic structure changes under compression. The structural properties of MgO are identified using pair correlation functions and self-diffusion coefficients. The solid-solid coexistence line is calculated by comparing the free enthalpies of the B1 and the B2 phase. The free energy of the solid phases is determined via thermodynamic relations using the ab initio simulation results and phonon calculations in the harmonic approximation. Our results indicate that the solid B2 phase of MgO does not occur in the interior of the Earth but may play an important role in super-Earths and in rocky planetary cores. {\textcopyright} 2014 American Physical Society.},
author = {Cebulla, Daniel and Redmer, Ronald},
doi = {10.1103/PhysRevB.89.134107},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Core formation/MgO/PhysRevB.89.134107.pdf:pdf},
issn = {1550235X},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {13},
pages = {1--10},
title = {{Ab initio simulations of MgO under extreme conditions}},
volume = {89},
year = {2014}
}
@article{Boates2013,
abstract = {The phase diagrams of MgSiO3 and MgO are studied from first-principles theory for pressures and temperatures up to 600 GPa and 20 000 K. Through the evaluation of finite-temperature Gibbs free energies, using density-functional theory within the generalized gradient approximation as well as with hybrid exchange-correlation functionals, we find evidence for a vast pressure-temperature regime where molten MgSiO3 decomposes into liquid SiO2 and solid MgO, with a volume change of approximately 1.2{\%}. The demixing transition is driven by the crystallization of MgO—the reaction only occurs below the high-pressure MgO melting curve. The predicted transition pressure at 10 000 K is in close proximity to an anomaly reported in recent laser-driven shock experiments of MgSiO3. We also present new results for the high-pressure melting curve of MgO and its B1-B2 solid phase transition, with a triple point at 364 GPa and 12 000 K.},
author = {Boates, Brian and Bonev, Stanimir A.},
doi = {10.1103/PhysRevLett.110.135504},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Boates, Bonev - 2013 - Demixing instability in dense molten MgSiO3and the phase diagram of MgO.pdf:pdf},
issn = {00319007},
journal = {Physical Review Letters},
number = {13},
pages = {1--5},
title = {{Demixing instability in dense molten MgSiO3and the phase diagram of MgO}},
volume = {110},
year = {2013}
}
@article{Belonoshko2010a,
abstract = {Recent laser-initiated strong shockwave measurements at Livermore provide the opportunity for verification of the MgO phase diagram at extreme pressures and temperatures. This calls for a comprehensive study of the MgO phase diagram. The phase diagram is obtained by ab initio molecular dynamics (two phase and Z method) and phonon-based thermodynamic calculations. Energies and forces are computed from first principles projector augmented wave method. The B1 transforms to B2 phase at about 490 GPa. Melting temperatures of B1 are consistent with the two-phase melting curve (Alfe, 2005). The triple point B1-B2-liquid is located at about 2.4 Mbar and 9000 K. The melting curve of the B2 phase rises rather steeply from the triple point. The Hugoniot is likely to cross the B1-B2 boundary first and then to cross the melting curve of B2, therefore, the melting curve of periclase is not relevant for the Hugoniot. MgO melts between 11.3 and 12.5 thousand K and 4.3 and 5 Mbar along the Hugoniot from the B2 phase. The two-phase melting curves of B1 computed with various semiempirical potentials are remarkably close to each other and are consistent with the B1 first principles melting curve at low pressure. This suggests the MgO melting temperatures to be in the close proximity of this determination. The search for new phases of MgO by first principles metadynamics has not produced unknown phases. Therefore, the suggested discontinuity of the Hugoniot at 170 GPa and 3000 K remains enigmatic.},
author = {Belonoshko, A. B. and Arapan, S. and Martonak, R. and Rosengren, A.},
doi = {10.1103/PhysRevB.81.054110},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Belonoshko et al. - 2010 - MgO phase diagram from first principles in a wide pressure-temperature range.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {5},
pages = {1--9},
title = {{MgO phase diagram from first principles in a wide pressure-temperature range}},
volume = {81},
year = {2010}
}
@article{Alfe2005a,
abstract = {We report diffusion Monte Carlo (DMC) calculations on MgO in the rock-salt and CsCl structures. The calculations are based on Hartree-Fock pseudopotentials, with the single-particle orbitals entering the correlated wave function being represented by a systematically convergeable cubic-spline basis. Systematic tests are presented on system-size errors using periodically repeating cells of up to over 600 atoms. The equilibrium lattice parameter of the rocksalt structure obtained within DMC is almost identical to the Hartree-Fock result, which is close to the experimental value. The DMC result for the bulk modulus is also in good agreement with the experimental value. The B1-B2 transition pressure (between the rocksalt and CsCl structures) is predicted to be just below 600 GPa, which is beyond the experimentally accessible range, in accord with other predictions based on Hartree-Fock and density functional theories. {\textcopyright} 2005 The American Physical Society.},
author = {Alf{\`{e}}, D. and Alfredsson, M. and Brodholt, J. and Gillan, M. J. and Towler, M. D. and Needs, R. J.},
doi = {10.1103/PhysRevB.72.014114},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Core formation/MgO/PhysRevB.72.014114.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {1},
pages = {1--7},
title = {{Quantum Monte Carlo calculations of the structural properties and the B1-B2 phase transition of MgO}},
volume = {72},
year = {2005}
}


@article{Militzer2013d,
author = {Militzer, Burkhard},
doi = {10.1016/j.hedp.2012.11.006},
issn = {15741818},
journal = {High Energy Density Physics},
keywords = {ab initio simulations,density functional molecular dynamics},
mendeley-groups = {MgSiO3},
month = {mar},
number = {1},
pages = {152--157},
publisher = {Elsevier Ltd},
title = {{Ab initio investigation of a possible liquid–liquid phase transition in MgSiO3 at megabar pressures}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S1574181812001322},
volume = {9},
year = {2013}
}

@article{Davies2020,
arxivId = {2002.00998},
author = {Davies, E. J. and Carter, P. J. and Root, S. and Kraus, R. G. and Spaulding, D. K. and Stewart, S. T. and Jacobsen, S. B.},
doi = {10.1029/2019JE006227},
eprint = {2002.00998},
file = {:Users/fgonzalez/Library/Application Support/Mendeley Desktop/Downloaded/2019JE006227.pdf:pdf},
issn = {21699100},
journal = {Journal of Geophysical Research: Planets},
keywords = {impacts,isentrope,melting,shock wave physics,thermodynamics,vaporization},
mendeley-groups = {Diamond},
number = {2},
pages = {1--17},
title = {{Silicate Melting and Vaporization During Rocky Planet Formation}},
volume = {125},
year = {2020}
}


@article{Swift2008,
  title={Shock formation and the ideal shape of ramp compression waves},
  author={Swift, Damian C and Kraus, Richard G and Loomis, Eric N and Hicks, Damien G and McNaney, James M and Johnson, Randall P},
  journal={Physical Review E},
  volume={78},
  number={6},
  pages={066115},
  year={2008},
  publisher={APS}
}
@article{desgranges2007controlling,
  title={Controlling polymorphism during the crystallization of an atomic fluid},
  author={Desgranges, Caroline and Delhommelle, Jerome},
  journal={Physical review letters},
  volume={98},
  number={23},
  pages={235502},
  year={2007},
  publisher={APS}
}
@article{sadigh2021metastable,
  title={Metastable--solid phase diagrams derived from polymorphic solidification kinetics},
  author={Sadigh, Babak and Zepeda-Ruiz, Luis and Belof, Jonathan L},
  journal={Proceedings of the National Academy of Sciences},
  volume={118},
  number={9},
  year={2021},
  publisher={National Acad Sciences}
}

@article{turnbull1950formation,
  title={Formation of crystal nuclei in liquid metals},
  author={Turnbull, D},
  journal={Journal of Applied Physics},
  volume={21},
  number={10},
  pages={1022--1028},
  year={1950},
  publisher={American Institute of Physics}
}

@article{Sun2018,
author = {Sun, Tao and Brodholt, John and Li, Yunguo and Vo{\v{c}}adlo, Lidunka},
doi = {10.1103/PhysRevB.98.224301},
issn = {2469-9950},
journal = {Physical Review B - Condensed Matter and Materials Physics},
mendeley-groups = {Melting Iron},
number = {22},
pages = {224301},
title = {{Melting properties from <i>ab initio</i> free energy calculations: Iron at the Earth's inner-core boundary}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.98.224301},
volume = {98},
year = {2018}
}
@article{sun2004crystal,
  title={Crystal-melt interfacial free energies in metals: fcc versus bcc},
  author={Sun, DY and Asta, M and Hoyt, JJ and Mendelev, MI and Srolovitz, DJ},
  journal={Physical Review B},
  volume={69},
  number={2},
  pages={020102},
  year={2004},
  publisher={APS}
}@article{Lazicki2012b,
abstract = {X-ray diffraction of beryllium in a laser-heated diamond anvil cell provides experimental insight into its behavior at high pressure and temperature. We measure the cold compression of Be in helium and NaCl pressure media up 192 GPa, and its thermal expansion up to 82 GPa and 2630 K. The new measurements form a P−V−T{\textless}math{\textgreater}{\textless}mrow{\textgreater}{\textless}mi{\textgreater}P{\textless}mo{\textgreater}-{\textless}mi{\textgreater}V{\textless}mo{\textgreater}-{\textless}mi{\textgreater}T data set which is fit by the Vinet-Debye form to establish a Be experimental equation of state. We compare the results to several theoretical models. The crystal structure of Be is determined up to 205 GPa and 4000 K; no evidence for the predicted high-temperature transition to a cubic phase is found. Finally, the maximum temperature stability of the solid phase along isobaric heating ramps gives a lower bound for the melting curve.},
author = {Lazicki, Amy and Dewaele, Agn{\`{e}}s and Loubeyre, Paul and Mezouar, Mohamed},
doi = {10.1103/PhysRevB.86.174118},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Lazicki et al. - 2012 - High-pressure-temperature phase diagram and the equation of state of beryllium.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {17},
pages = {1--10},
title = {{High-pressure-temperature phase diagram and the equation of state of beryllium}},
volume = {86},
year = {2012}
}
@article{Velisavljevic2002a,
abstract = {The structural and electrical properties of alkaline-earth metal beryllium were studied to 66 GPa using designer diamond anvils. The ambient pressure hexagonal close-packed phase was found to be stable to the highest pressure of 66 GPa and the measured static equation of state differs substantially from the one derived from the existing shock wave data. The electrical resistance data at high pressure shows a gradual decrease in resistance to pressure up to 25 GPa followed by a slight increase to 53 Gpa. The axial ratio (c/a) remains strongly nonideal with c/a = 1.562 at V/V 0  = 0.708, indicating that deviations from nearly free electron behavior are still dominant at high compressions.},
author = {Velisavljevic, Nenad and Chesnut, Gary N. and Vohra, Yogesh K. and Weir, Samuel T. and Malba, Vincent and Akella, Jagannadham},
doi = {10.1103/PhysRevB.65.172107},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Velisavljevic et al. - 2002 - Structural and electrical properties of beryllium metal to 66 GPa studied using designer diamond anvils.pdf:pdf},
issn = {01631829},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {17},
pages = {1721071--1721074},
title = {{Structural and electrical properties of beryllium metal to 66 GPa studied using designer diamond anvils}},
volume = {65},
year = {2002}
}
@article{Nakano2002b,
author = {Nakano, Kazutaka and Akahama, Yuichi and Kawamura, Haruki},
doi = {10.1088/0953-8984/14/44/334},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Nakano, Akahama, Kawamura - 2002 - X-ray diffraction study of Be to megabar pressure.pdf:pdf},
issn = {09538984},
journal = {Journal of Physics Condensed Matter},
number = {44 SPEC ISS.},
pages = {10569--10573},
title = {{X-ray diffraction study of Be to megabar pressure}},
volume = {14},
year = {2002}
}
@article{Evans2005a,
abstract = {We report combined x-ray and Raman studies of beryllium in helium and argon pressure media at pressures approaching 200 GPa. Our results are generally consistent with recent studies confirming the stability of the hexagonal close-packed phase to the highest pressures. However, the quasihydrostatic conditions of our studies lead to a stiffer equation of state (K0=109.88, K′0=3.59) and a gradual approach toward a more ideal c∕a ratio of 1.60 at 180 GPa. Combining our Raman and equation of state data, we are able to evaluate the pressure dependence of the elastic shear modulus (C44=109.3, C′44=1.959). We discuss the comparison of our results with measurements using ultrasonic and dynamic techniques.},
author = {Evans, W. J. and Lipp, M. J. and Cynn, H. and Yoo, C. S. and Somayazulu, M. and H{\"{a}}usermann, D. and Shen, G. and Prakapenka, V.},
doi = {10.1103/PhysRevB.72.094113},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Evans et al. - 2005 - X-ray diffraction and Raman studies of beryllium Static and elastic properties at high pressures.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {9},
pages = {1--6},
title = {{X-ray diffraction and Raman studies of beryllium: Static and elastic properties at high pressures}},
volume = {72},
year = {2005}
}
@article{Martin1959,
author = {Martin, A.J. and Moore, A.},
doi = {10.1016/0022-5088(59)90045-1},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Unknown - 1959 - to sudden changes in furnace voltage , and also served to cut down convection currents in the argon atmosphere . Heati.pdf:pdf},
issn = {00225088},
journal = {Journal of the Less Common Metals},
month = {apr},
number = {2},
pages = {85--93},
title = {{The structure of beryllium, with particular reference to temperatures above 1200°C}},
url = {https://linkinghub.elsevier.com/retrieve/pii/0022508859900451},
volume = {1},
year = {1959}
}
@article{Ming1984a,
abstract = {In situ high-pressure X-ray diffraction data for polycrystalline beryllium to 28.3 GPA at ambient temperature show that beryllium is transformed from the HCP phase (I) into a slightly distorted HCP phase (II) at pressures between 8.6 and 14.5 GPa. The volume change for the transition is extremely small ( approximately 0.4{\%}); the effect of pressure on the c/a ratio for both the Be(I) and Be(II) phases is also very small.},
author = {Ming, L. C. and Manghnani, M. H.},
doi = {10.1088/0305-4608/14/1/001},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/L{\_}C{\_}Ming{\_}1984{\_}J.{\_}Phys.{\_}F{\_}{\_}Met.{\_}Phys.{\_}14{\_}L1.pdf:pdf},
issn = {03054608},
journal = {Journal of Physics F: Metal Physics},
number = {1},
title = {{Isothermal compression and phase transition in beryllium to 28.3 GPa}},
volume = {14},
year = {1984}
}
@article{Lu2017b,
abstract = {Beryllium (Be) is an important material with wide applications ranging from aerospace components to x-ray equipment. Yet a precise understanding of its phase diagram remains elusive. We have investigated the phase stability of Be using a recently developed hybrid free energy computation method that accounts for anharmonic effects by invoking phonon quasiparticles. We find that the hcp → bcc transition occurs near the melting curve at 0 {\textless} P {\textless} 11 GPa with a positive Clapeyron slope of 41 ± 4 K / GPa , which is more consistent with recent experimental measurements. This work also demonstrates the validity of this theoretical framework based on the phonon quasiparticle to study the structural stability and phase transitions in strongly anharmonic materials.},
author = {Lu, Y. and Sun, T. and Zhang, Ping and Zhang, P. and Zhang, D. B. and Wentzcovitch, R. M.},
doi = {10.1103/PhysRevLett.118.145702},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Lu et al. - 2017 - Premelting hcp to bcc Transition in Beryllium.pdf:pdf},
issn = {10797114},
journal = {Physical Review Letters},
number = {14},
title = {{Premelting hcp to bcc Transition in Beryllium}},
url = {https://journals.aps.org/prl/pdf/10.1103/PhysRevLett.118.145702},
volume = {118},
year = {2017}
}
@article{Palanivel2000,
abstract = {High-pressure electronic properties of Be have been investigated theoretically be means of ab initio electronic structure calculations. The calculations have been carried out by the semi-relativistic full-potential, linear muffin-tin orbital (FPLMTO) method, within the local density approximation. The crystal structure stability among the hcp, bcc and orthorhombic (distorted hcp) phases has been studied as a function of compression. The bcc structure is found to be energetically stable at pressures above 180 GPa. From the results of our calculations, the orthorhombic phase cannot occur as an intermediate phase between the ambient pressure hcp phase and the high-pressure bcc structure. Our work thus suggests the need for more accurate high-pressure x-ray data.},
author = {Palanivel, B. and Rao, R. S. and Godwal, B. K. and Sikka, S. K.},
doi = {10.1088/0953-8984/12/41/309},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/B{\_}Palanivel{\_}2000{\_}J.{\_}Phys.{\_}{\_}Condens.{\_}Matter{\_}12{\_}8831.pdf:pdf},
issn = {09538984},
journal = {Journal of Physics Condensed Matter},
number = {41},
pages = {8831--8836},
title = {{On the relative stability of orthorhombic and hcp phases of beryllium at high pressures}},
volume = {12},
year = {2000}
}
@article{Sinko2005a,
abstract = {Ab initio electronic-structure calculations, based on the density-functional theory and the full-potential linear-muffin-tin-orbital method, were used to predict crystal-sructure phase stabilities and elastic constants of beryllium under compression. Specific energies, pressures, elastic constants, and Debye temperatures for three crystal structures, hcp, bcc, and fcc, were calculated over a wide volume range. In agreement with experiments and previous theoretical calculations, the hcp ground state is obtained at ambient conditions and the bcc ground state is found at high pressure and ambient temperature, with the predicted hcp→bcc phase transition at about 2.7 Mbar. A possible phase diagram of beryllium, including hcp, bcc, and fcc phases is constructed in the (P,T) plane.},
author = {Sin'ko, G. V. and Smirnov, N. A.},
doi = {10.1103/PhysRevB.71.214108},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Sin'ko, Smirnov - 2005 - Relative stability and elastic properties of hcp, bcc, and fcc beryllium under pressure.pdf:pdf},
issn = {1098-0121},
journal = {Physical Review B},
month = {jun},
number = {21},
pages = {214108},
title = {{Relative stability and elastic properties of hcp, bcc, and fcc beryllium under pressure}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.71.214108},
volume = {71},
year = {2005}
}
@article{Robert2006a,
abstract = {The electronic and structural properties of beryllium were investigated under high pressure using first principle pseudopotential calculations within the generalized gradient approximation (GGA). Our results including pressures, elastic constants, Debye temperatures for two crystal structures ($\alpha$ hexagonal close packed and $\beta$ body-centred cubic) are compared with the experimental and other theoretical data over a wide density range. Calculated phonon spectra allow us to explain the anomalous behavior of the hcp-bcc transition under pressure. An equation of state (EOS) for the hep phase at finite temperatures is derived taking into account the anharmonicity effects of thermal lattice vibrations. The resulting 300 K isotherm and Hugoniot curve, as well as the evolution of the shear modulus under pressure and temperature, are in good agreement with available experimental and theoretical data. {\textcopyright} EDP Sciences.},
author = {Robert, G. and Sollier, A.},
doi = {10.1051/jp4:2006134039},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/jp4134039.pdf:pdf},
isbn = {2868839444},
issn = {11554339},
journal = {Journal De Physique. IV : JP},
pages = {257--262},
title = {{Equation of state and elastic properties of beryllium from first principles calculations}},
volume = {134},
year = {2006}
}
@article{Luo2012,
abstract = {We investigate the phase transition, elastic constants, phonon dispersion curves, and thermal properties of beryllium (Be) at high pressures and high temperatures using density functional theory. By comparing the Gibbs free energy, in the quasiharmonic approximation (QHA), of hexagonal-closed-packed (hcp) with those of the face-centered cubic (fcc) and body-centered-cubic (bcc) we find that the hcp Be is stable up to 390 GPa, and then transforms to the bcc Be. The calculated phonon dispersion curves are in excellent agreement with experiments. Under compression, the phonon dispersion curves of hcp Be do not show any anomaly or instability. At low pressure the phonon dispersion of bcc Be display imaginary along $\Omega$-N in the T 1 branches. Within the quasiharmonic approximation, we predict the thermal equation of state and other properties including the thermal expansion coefficient, Hugoniot curves, heat capacity, Gr{\"{u}}neisen parameter, and Debye temperature. {\textcopyright} 2012 American Institute of Physics.},
author = {Luo, Fen and Cai, Ling Cang and Chen, Xiang Rong and Jing, Fu Qian and Alf, Dario},
doi = {10.1063/1.3688344},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Luo et al. - 2012 - Ab initio calculation of lattice dynamics and thermodynamic properties of beryllium.pdf:pdf},
issn = {00218979},
journal = {Journal of Applied Physics},
number = {5},
title = {{Ab initio calculation of lattice dynamics and thermodynamic properties of beryllium}},
volume = {111},
year = {2012}
}
@article{Song2007,
abstract = {We extend the mean-field potential (MFP) approach for evaluating the vibrational contribution of the lattice ion of high-symmetry metals, and present a modified MFP approach which can be applied to low-symmetry or complex structure crystals. Based on the modified MFP approach in which the effect of the structural parameters on the free energy is taken into account, a first-principles scheme for calculating thermodynamic properties of a crystal dependent on the crystal structure is developed. By taking hexagonal close-packed beryllium as a prototype, we demonstrate that our scheme is suitable for investigating the structural properties and equation of state of low-symmetry crystals. {\textcopyright} 2007 The American Physical Society.},
author = {Song, Hai Feng and Liu, Hai Feng},
doi = {10.1103/PhysRevB.75.245126},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Song, Liu - 2007 - Modified mean-field potential approach to thermodynamic properties of a low-symmetry crystal Beryllium as a prototype.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {24},
pages = {1--7},
title = {{Modified mean-field potential approach to thermodynamic properties of a low-symmetry crystal: Beryllium as a prototype}},
volume = {75},
year = {2007}
}
@article{Benedict2009,
abstract = {We describe the construction of a three-phase equation of state for elemental beryllium. The phases considered are: the ambient hcp phase, the high-temperature bcc phase, and the liquid. The free energies of the solid phases are constructed from cold, ion-thermal, and electron-thermal components derived from ab initio electronic structure-based calculations. We find that the bcc phase is unstable near ambient conditions and that even at high pressures at which the bcc phase is stable, the bcc-hcp energy barrier can be as small as a few hundred kelvins. The liquid free energy is based on a model of Chisolm and Wallace and is constrained by using the melt curve (determined by ab initio two-phase simulations) as a reference. The high-temperature plasma limit is addressed with an average-atom-in-jellium model. Comparisons to experimental results, both for the ambient hcp phase and for the phase diagram as a whole, are discussed.},
author = {Benedict, Lorin X. and Ogitsu, Tadashi and Trave, Andrea and Wu, Christine J. and Sterne, Philip A. and Schwegler, Eric},
doi = {10.1103/PhysRevB.79.064106},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Benedict et al. - 2009 - Calculations of high-pressure properties of beryllium Construction of a multiphase equation of state.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {6},
pages = {1--9},
title = {{Calculations of high-pressure properties of beryllium: Construction of a multiphase equation of state}},
volume = {79},
year = {2009}
}
@article{Robert2010,
abstract = {Based on ab initio calculations, we provide a consistent modeling in pressure and temperature of the solid phases of beryllium, including theoretical phase diagram, multiphase equation of state (EOS), and elastic moduli. The quasiharmonic approximation (QHA) allows us to determine the whole theoretical phase diagram: at room temperature, QHA predicts the hexagonal compact ($\alpha$-hcp) phase as the most stable structure up to 400 GPa, where a transition toward the body-centered-cubic ($\beta$-bcc) phase occurs. However, the QHA does not account for the low-pressure-high-temperature bcc phase found experimentally. Combining frozen phonon and density-functional perturbation theory methods, we show that soft phonon modes as reservoirs of entropy may stabilize the low-pressure bcc phase. However the thermodynamic stability of this phase has still to be established. We provide the QHA multiphase EOS in analytic form and an evaluation of the uncertainties on the QHA solid-solid and solid-liquid phase boundaries. Then, we calculate the density and temperature dependence of elastic constants by determining the free energies of strained structures. Consistency between the polycrystalline (i.e., averaged over the elastic constants) and the EOS isothermal bulk moduli is achieved for both phases. Our results are in fair agreement with the most recent experimental data and permit us to raise questions on some experimental moduli.},
author = {Robert, G. and Legrand, P. and Bernard, S.},
doi = {10.1103/PhysRevB.82.104118},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Robert, Legrand, Bernard - 2010 - Multiphase equation of state and elastic moduli of solid beryllium from first principles.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {10},
title = {{Multiphase equation of state and elastic moduli of solid beryllium from first principles}},
url = {https://journals.aps.org/prb/pdf/10.1103/PhysRevB.82.104118},
volume = {82},
year = {2010}
}
@article{Xian2019b,
author = {Xian, Jia Wei and Yan, Jun and Liu, Hai Feng and Sun, Tao and Zhang, Gong Mu and Gao, Xing Yu and Song, Hai Feng},
doi = {10.1103/PhysRevB.99.064102},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Xian et al. - 2019 - Effect of anharmonicity on the hcp to bcc transition in beryllium at high-pressure and high-temperature conditions.pdf:pdf},
issn = {24699969},
journal = {Physical Review B},
keywords = {doi:10.1103/PhysRevB.99.064102 url:https://doi.org},
number = {6},
pages = {1--12},
publisher = {American Physical Society},
title = {{Effect of anharmonicity on the hcp to bcc transition in beryllium at high-pressure and high-temperature conditions}},
volume = {99},
year = {2019}
}
@article{Ming1984a,
abstract = {In situ high-pressure X-ray diffraction data for polycrystalline beryllium to 28.3 GPA at ambient temperature show that beryllium is transformed from the HCP phase (I) into a slightly distorted HCP phase (II) at pressures between 8.6 and 14.5 GPa. The volume change for the transition is extremely small ( approximately 0.4{\%}); the effect of pressure on the c/a ratio for both the Be(I) and Be(II) phases is also very small.},
author = {Ming, L. C. and Manghnani, M. H.},
doi = {10.1088/0305-4608/14/1/001},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/L{\_}C{\_}Ming{\_}1984{\_}J.{\_}Phys.{\_}F{\_}{\_}Met.{\_}Phys.{\_}14{\_}L1.pdf:pdf},
issn = {03054608},
journal = {Journal of Physics F: Metal Physics},
number = {1},
title = {{Isothermal compression and phase transition in beryllium to 28.3 GPa}},
volume = {14},
year = {1984}
}
@article{Vijayakumar1984b,
abstract = {The metal beryllium (Be) has been studied under high pressure using an electrical resistivity technique with in situ pressure calibration. A sluggish phase transition at 12 GPa is observed which the authors identify as the HCP to distorted HCP phase transition reported in a recent high-pressure X-ray diffraction study. However, a reanalysis of the X-ray data on the high-pressure phase Be(II) indicates that a smaller orthorhombic cell with four atoms fits the observed interplanar spacings. The observed intensity ratios of the diffraction lines can be explained reasonably well on the basis of the space group P2 1 2 1 2 with four Be atoms occupying 4c positions.},
author = {Vijayakumar, V. and Godwal, B. K. and Vohra, Y. K. and Sikka, S. K. and Chidambaram, R.},
doi = {10.1088/0305-4608/14/5/002},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Vijayakumar et al. - 1984 - On the high-pressure phase transition in beryllium metal.pdf:pdf},
issn = {03054608},
journal = {Journal of Physics F: Metal Physics},
number = {5},
title = {{On the high-pressure phase transition in beryllium metal}},
volume = {14},
year = {1984}
}


==> tmp <==
@article{Kline2016,
abstract = {The first indirect drive implosion experiments using Beryllium (Be) capsules at the National Ignition Facility confirm the superior ablation properties and elucidate possible Be-ablator issues such as hohlraum filling by ablator material. Since the 1990s, Be has been the preferred Inertial Confinement Fusion (ICF) ablator because of its higher mass ablation rate compared to that of carbon-based ablators. This enables ICF target designs with higher implosion velocities at lower radiation temperatures and improved hydrodynamic stability through greater ablative stabilization. Recent experiments to demonstrate the viability of Be ablator target designs measured the backscattered laser energy, capsule implosion velocity, core implosion shape from self-emission, and in-flight capsule shape from backlit imaging. The laser backscatter is similar to that from comparable plastic (CH) targets under the same hohlraum conditions. Implosion velocity measurements from backlit streaked radiography show that laser energy coupling to the hohlraum wall is comparable to plastic ablators. The measured implosion shape indicates no significant reduction of laser energy from the inner laser cone beams reaching the hohlraum wall as compared with plastic and high-density carbon ablators. These results indicate that the high mass ablation rate for beryllium capsules does not significantly alter hohlraum energetics. In addition, these data, together with data for low fill-density hohlraum performance, indicate that laser power multipliers, required to reconcile simulations with experimental observations, are likely due to our limited understanding of the hohlraum rather than the capsule physics since similar multipliers are needed for both Be and CH capsules as seen in experiments.},
author = {Kline, J. L. and Yi, S. A. and Simakov, A. N. and Olson, R. E. and Wilson, D. C. and Kyrala, G. A. and Perry, T. S. and Batha, S. H. and Zylstra, A. B. and Dewald, E. L. and Tommasini, R. and Ralph, J. E. and Strozzi, D. J. and MacPhee, A. G. and Callahan, D. A. and Hinkel, D. E. and Hurricane, O. A. and Milovich, J. L. and Rygg, J. R. and Khan, S. F. and Haan, S. W. and Celliers, P. M. and Clark, D. S. and Hammel, B. A. and Kozioziemski, B. and Schneider, M. B. and Marinak, M. M. and Rinderknecht, H. G. and Robey, H. F. and Salmonson, J. D. and Patel, P. K. and Ma, T. and Edwards, M. J. and Stadermann, M. and Baxamusa, S. and Alford, C. and Wang, M. and Nikroo, A. and Rice, N. and Hoover, D. and Youngblood, K. P. and Xu, H. and Huang, H. and Sio, H.},
doi = {10.1063/1.4948277},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.4948277.pdf:pdf},
issn = {10897674},
journal = {Physics of Plasmas},
number = {5},
title = {{First beryllium capsule implosions on the National Ignition Facility}},
volume = {23},
year = {2016}
}
@article{Clark2018,
abstract = {Indirect drive implosion experiments on the National Ignition Facility (NIF) [E. I. Moses et al., Phys. Plasmas 16, 041006 (2009)] have now tested three different ablator materials: glow discharge polymer plastic, high density carbon, and beryllium. How do these different ablators compare in current and proposed implosion experiments on NIF? What are the relative advantages and disadvantages of each? This paper compares these different ablator options in capsule-only simulations of current NIF experiments and potential future designs. The simulations compare the impact of the capsule fill tube, support tent, and interface surface roughness for each case, as well as all perturbations in combination. According to the simulations, each ablator is impacted by the various perturbation sources differently, and each material poses unique challenges in the pursuit of ignition on NIF.},
author = {Clark, D. S. and Kritcher, A. L. and Yi, S. A. and Zylstra, A. B. and Haan, S. W. and Weber, C. R.},
doi = {10.1063/1.5016874},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.5016874.pdf:pdf},
issn = {10897674},
journal = {Physics of Plasmas},
number = {3},
title = {{Capsule physics comparison of National Ignition Facility implosion designs using plastic, high density carbon, and beryllium ablators}},
volume = {25},
year = {2018}
}
@article{Haan2011,
abstract = {Point design targets have been specified for the initial ignition campaign on the National Ignition Facility G. H. Miller, E. I. Moses, and C. R. Wuest, Opt. Eng. 443, 2841 (2004). The targets contain D-T fusion fuel in an ablator of either CH with Ge doping, or Be with Cu. These shells are imploded in a U or Au hohlraum with a peak radiation temperature set between 270 and 300 eV. Considerations determining the point design include laser-plasma interactions, hydrodynamic instabilities, laser operations, and target fabrication. Simulations were used to evaluate choices, and to define requirements and specifications. Simulation techniques and their experimental validation are summarized. Simulations were used to estimate the sensitivity of target performance to uncertainties and variations in experimental conditions. A formalism is described that evaluates margin for ignition, summarized in a parameter the Ignition Threshold Factor (ITF). Uncertainty and shot-to-shot variability in ITF are evaluated, and sensitivity of the margin to characteristics of the experiment. The formalism is used to estimate probability of ignition. The ignition experiment will be preceded with an experimental campaign that determines features of the design that cannot be defined with simulations alone. The requirements for this campaign are summarized. Requirements are summarized for the laser and target fabrication. {\textcopyright} 2011 American Institute of Physics.},
author = {Haan, S. W. and Lindl, J. D. and Callahan, D. A. and Clark, D. S. and Salmonson, J. D. and Hammel, B. A. and Atherton, L. J. and Cook, R. C. and Edwards, M. J. and Glenzer, S. and Hamza, A. V. and Hatchett, S. P. and Herrmann, M. C. and Hinkel, D. E. and Ho, D. D. and Huang, H. and Jones, O. S. and Kline, J. and Kyrala, G. and Landen, O. L. and MacGowan, B. J. and Marinak, M. M. and Meyerhofer, D. D. and Milovich, J. L. and Moreno, K. A. and Moses, E. I. and Munro, D. H. and Nikroo, A. and Olson, R. E. and Peterson, K. and Pollaine, S. M. and Ralph, J. E. and Robey, H. F. and Spears, B. K. and Springer, P. T. and Suter, L. J. and Thomas, C. A. and Town, R. P. and Vesey, R. and Weber, S. V. and Wilkens, H. L. and Wilson, D. C.},
doi = {10.1063/1.3592169},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.3592169.pdf:pdf},
issn = {1070664X},
journal = {Physics of Plasmas},
number = {5},
title = {{Point design targets, specifications, and requirements for the 2010 ignition campaign on the National Ignition Facility}},
volume = {18},
year = {2011}
}
@article{Clark2008,
abstract = {Inertial confinement fusion capsules are critically dependent on the integrity of their hot spots to ignite. At the time of ignition, only a certain fractional perturbation of the nominally spherical hot spot boundary can be tolerated and the capsule still achieve ignition. The degree to which the expected hot spot perturbation in any given capsule design is less than this maximum tolerable perturbation is a measure of the ignition margin or robustness of that design. Moreover, since there will inevitably be uncertainties in the initial character and implosion dynamics of any given capsule, all of which can contribute to the eventual hot spot perturbation, quantifying the robustness of that capsule against a range of parameter variations is an important consideration in the capsule design. Here, the robustness of the 300 eV indirect drive target design for the National Ignition Facility [Lindl, Phys. Plasmas 11, 339 (2004)] is studied in the parameter space of inner ice roughness, implosion velocity, and capsule scale. A suite of 2000 two-dimensional simulations, run with the radiation hydrodynamics code LASNEX, is used as the data base for the study. For each scale, an ignition region in the two remaining variables is identified and the ignition cliff is mapped. In accordance with the theoretical arguments of Levedahl and Lindl [Nucl. Fusion 37, 165 (1997)] and Kishony and Shvarts [Phys. Plasmas 8, 4925 (2001)], the location of this cliff is fitted to a power law of the capsule implosion velocity and scale. It is found that the cliff can be quite well represented in this power law form, and, using this scaling law, an assessment of the overall (one- and two-dimensional) ignition margin of the design can be made. The effect on the ignition margin of an increase or decrease in the density of the target fill gas is also assessed. {\textcopyright} 2008 American Institute of Physics.},
author = {Clark, Daniel S. and Haan, Steven W. and Salmonson, Jay D.},
doi = {10.1063/1.2890123},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.2890123.pdf:pdf},
issn = {1070664X},
journal = {Physics of Plasmas},
number = {5},
title = {{Robustness studies of ignition targets for the National Ignition Facility in two dimensions}},
volume = {15},
year = {2008}
}
@article{Simakov2014,
abstract = {For indirect drive inertial confinement fusion, Beryllium (Be) ablators offer a number of important advantages as compared with other ablator materials, e.g., plastic and high density carbon. In particular, the low opacity and relatively high density of Be lead to higher rocket efficiencies giving a higher fuel implosion velocity for a given X-ray drive; and to higher ablation velocities providing more ablative stabilization and reducing the effect of hydrodynamic instabilities on the implosion performance. Be ablator advantages provide a larger target design optimization space and can significantly improve the National Ignition Facility (NIF) [J. D. Lindl et al., Phys. Plasmas 11, 339 (2004)] ignition margin. Herein, we summarize the Be advantages, briefly review NIF Be target history, and present a modern, optimized, low adiabat, Revision 6 NIF Be target design. This design takes advantage of knowledge gained from recent NIF experiments, including more realistic levels of laser-plasma energy backscatter, degraded hohlraum-capsule coupling, and the presence of cross-beam energy transfer. {\textcopyright} 2014 AIP Publishing LLC.},
author = {Simakov, Andrei N. and Wilson, Douglas C. and Yi, Sunghwan A. and Kline, John L. and Clark, Daniel S. and Milovich, Jose L. and Salmonson, Jay D. and Batha, Steven H.},
doi = {10.1063/1.4864331},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/1.4864331.pdf:pdf},
issn = {1070664X},
journal = {Physics of Plasmas},
number = {2},
title = {{Optimized beryllium target design for indirectly driven inertial confinement fusion experiments on the national ignition facility}},
volume = {21},
year = {2014}
}
@article{Benedict2009,
author = {Benedict, Lorin X. and Ogitsu, Tadashi and Trave, Andrea and Wu, Christine J. and Sterne, Philip A. and Schwegler, Eric},
doi = {10.1103/PhysRevB.79.064106},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
mendeley-groups = {Beryllium},
number = {6},
pages = {1--9},
title = {{Calculations of high-pressure properties of beryllium: Construction of a multiphase equation of state}},
volume = {79},
year = {2009}
}

@article{Zhang2013,
author = {Zhang, Jianzhong and Zhu, Jinlong and Velisavljevic, Nenad and Wang, Liping and Zhao, Yusheng},
doi = {10.1063/1.4828886},
issn = {0021-8979},
journal = {Journal of Applied Physics},
mendeley-groups = {Beryllium},
month = {nov},
number = {17},
pages = {173509},
title = {{Thermal equation of state and thermodynamic Gr{\"{u}}neisen parameter of beryllium metal}},
url = {http://aip.scitation.org/doi/10.1063/1.4828886},
volume = {114},
year = {2013}
}

]

@article{simakov2014optimized,
  title={Optimized beryllium target design for indirectly driven inertial confinement fusion experiments on the National Ignition Facility},
  author={Simakov, Andrei N and Wilson, Douglas C and Yi, Sunghwan A and Kline, John L and Clark, Daniel S and Milovich, Jose L and Salmonson, Jay D and Batha, Steven H},
  journal={Physics of Plasmas},
  volume={21},
  number={2},
  pages={022701},
  year={2014},
  publisher={American Institute of Physics}
}
@article{Kline2016,
abstract = {The first indirect drive implosion experiments using Beryllium (Be) capsules at the National Ignition Facility confirm the superior ablation properties and elucidate possible Be-ablator issues such as hohlraum filling by ablator material. Since the 1990s, Be has been the preferred Inertial Confinement Fusion (ICF) ablator because of its higher mass ablation rate compared to that of carbon-based ablators. This enables ICF target designs with higher implosion velocities at lower radiation temperatures and improved hydrodynamic stability through greater ablative stabilization. Recent experiments to demonstrate the viability of Be ablator target designs measured the backscattered laser energy, capsule implosion velocity, core implosion shape from self-emission, and in-flight capsule shape from backlit imaging. The laser backscatter is similar to that from comparable plastic (CH) targets under the same hohlraum conditions. Implosion velocity measurements from backlit streaked radiography show that laser energy coupling to the hohlraum wall is comparable to plastic ablators. The measured implosion shape indicates no significant reduction of laser energy from the inner laser cone beams reaching the hohlraum wall as compared with plastic and high-density carbon ablators. These results indicate that the high mass ablation rate for beryllium capsules does not significantly alter hohlraum energetics. In addition, these data, together with data for low fill-density hohlraum performance, indicate that laser power multipliers, required to reconcile simulations with experimental observations, are likely due to our limited understanding of the hohlraum rather than the capsule physics since similar multipliers are needed for both Be and CH capsules as seen in experiments.},
author = {Kline, J. L. and Yi, S. A. and Simakov, A. N. and Olson, R. E. and Wilson, D. C. and Kyrala, G. A. and Perry, T. S. and Batha, S. H. and Zylstra, A. B. and Dewald, E. L. and Tommasini, R. and Ralph, J. E. and Strozzi, D. J. and MacPhee, A. G. and Callahan, D. A. and Hinkel, D. E. and Hurricane, O. A. and Milovich, J. L. and Rygg, J. R. and Khan, S. F. and Haan, S. W. and Celliers, P. M. and Clark, D. S. and Hammel, B. A. and Kozioziemski, B. and Schneider, M. B. and Marinak, M. M. and Rinderknecht, H. G. and Robey, H. F. and Salmonson, J. D. and Patel, P. K. and Ma, T. and Edwards, M. J. and Stadermann, M. and Baxamusa, S. and Alford, C. and Wang, M. and Nikroo, A. and Rice, N. and Hoover, D. and Youngblood, K. P. and Xu, H. and Huang, H. and Sio, H.},
doi = {10.1063/1.4948277},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.4948277.pdf:pdf},
issn = {10897674},
journal = {Physics of Plasmas},
number = {5},
title = {{First beryllium capsule implosions on the National Ignition Facility}},
volume = {23},
year = {2016}
}
@article{Clark2018,
abstract = {Indirect drive implosion experiments on the National Ignition Facility (NIF) [E. I. Moses et al., Phys. Plasmas 16, 041006 (2009)] have now tested three different ablator materials: glow discharge polymer plastic, high density carbon, and beryllium. How do these different ablators compare in current and proposed implosion experiments on NIF? What are the relative advantages and disadvantages of each? This paper compares these different ablator options in capsule-only simulations of current NIF experiments and potential future designs. The simulations compare the impact of the capsule fill tube, support tent, and interface surface roughness for each case, as well as all perturbations in combination. According to the simulations, each ablator is impacted by the various perturbation sources differently, and each material poses unique challenges in the pursuit of ignition on NIF.},
author = {Clark, D. S. and Kritcher, A. L. and Yi, S. A. and Zylstra, A. B. and Haan, S. W. and Weber, C. R.},
doi = {10.1063/1.5016874},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.5016874.pdf:pdf},
issn = {10897674},
journal = {Physics of Plasmas},
number = {3},
title = {{Capsule physics comparison of National Ignition Facility implosion designs using plastic, high density carbon, and beryllium ablators}},
volume = {25},
year = {2018}
}
@article{Simakov2014,
abstract = {For indirect drive inertial confinement fusion, Beryllium (Be) ablators offer a number of important advantages as compared with other ablator materials, e.g., plastic and high density carbon. In particular, the low opacity and relatively high density of Be lead to higher rocket efficiencies giving a higher fuel implosion velocity for a given X-ray drive; and to higher ablation velocities providing more ablative stabilization and reducing the effect of hydrodynamic instabilities on the implosion performance. Be ablator advantages provide a larger target design optimization space and can significantly improve the National Ignition Facility (NIF) [J. D. Lindl et al., Phys. Plasmas 11, 339 (2004)] ignition margin. Herein, we summarize the Be advantages, briefly review NIF Be target history, and present a modern, optimized, low adiabat, Revision 6 NIF Be target design. This design takes advantage of knowledge gained from recent NIF experiments, including more realistic levels of laser-plasma energy backscatter, degraded hohlraum-capsule coupling, and the presence of cross-beam energy transfer. {\textcopyright} 2014 AIP Publishing LLC.},
author = {Simakov, Andrei N. and Wilson, Douglas C. and Yi, Sunghwan A. and Kline, John L. and Clark, Daniel S. and Milovich, Jose L. and Salmonson, Jay D. and Batha, Steven H.},
doi = {10.1063/1.4864331},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/1.4864331.pdf:pdf},
issn = {1070664X},
journal = {Physics of Plasmas},
number = {2},
title = {{Optimized beryllium target design for indirectly driven inertial confinement fusion experiments on the national ignition facility}},
volume = {21},
year = {2014}
}
@article{Haan2011,
abstract = {Point design targets have been specified for the initial ignition campaign on the National Ignition Facility G. H. Miller, E. I. Moses, and C. R. Wuest, Opt. Eng. 443, 2841 (2004). The targets contain D-T fusion fuel in an ablator of either CH with Ge doping, or Be with Cu. These shells are imploded in a U or Au hohlraum with a peak radiation temperature set between 270 and 300 eV. Considerations determining the point design include laser-plasma interactions, hydrodynamic instabilities, laser operations, and target fabrication. Simulations were used to evaluate choices, and to define requirements and specifications. Simulation techniques and their experimental validation are summarized. Simulations were used to estimate the sensitivity of target performance to uncertainties and variations in experimental conditions. A formalism is described that evaluates margin for ignition, summarized in a parameter the Ignition Threshold Factor (ITF). Uncertainty and shot-to-shot variability in ITF are evaluated, and sensitivity of the margin to characteristics of the experiment. The formalism is used to estimate probability of ignition. The ignition experiment will be preceded with an experimental campaign that determines features of the design that cannot be defined with simulations alone. The requirements for this campaign are summarized. Requirements are summarized for the laser and target fabrication. {\textcopyright} 2011 American Institute of Physics.},
author = {Haan, S. W. and Lindl, J. D. and Callahan, D. A. and Clark, D. S. and Salmonson, J. D. and Hammel, B. A. and Atherton, L. J. and Cook, R. C. and Edwards, M. J. and Glenzer, S. and Hamza, A. V. and Hatchett, S. P. and Herrmann, M. C. and Hinkel, D. E. and Ho, D. D. and Huang, H. and Jones, O. S. and Kline, J. and Kyrala, G. and Landen, O. L. and MacGowan, B. J. and Marinak, M. M. and Meyerhofer, D. D. and Milovich, J. L. and Moreno, K. A. and Moses, E. I. and Munro, D. H. and Nikroo, A. and Olson, R. E. and Peterson, K. and Pollaine, S. M. and Ralph, J. E. and Robey, H. F. and Spears, B. K. and Springer, P. T. and Suter, L. J. and Thomas, C. A. and Town, R. P. and Vesey, R. and Weber, S. V. and Wilkens, H. L. and Wilson, D. C.},
doi = {10.1063/1.3592169},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.3592169.pdf:pdf},
issn = {1070664X},
journal = {Physics of Plasmas},
number = {5},
title = {{Point design targets, specifications, and requirements for the 2010 ignition campaign on the National Ignition Facility}},
volume = {18},
year = {2011}
}
@article{Lu2017b,
abstract = {Beryllium (Be) is an important material with wide applications ranging from aerospace components to x-ray equipment. Yet a precise understanding of its phase diagram remains elusive. We have investigated the phase stability of Be using a recently developed hybrid free energy computation method that accounts for anharmonic effects by invoking phonon quasiparticles. We find that the hcp → bcc transition occurs near the melting curve at 0 {\textless} P {\textless} 11 GPa with a positive Clapeyron slope of 41 ± 4 K / GPa , which is more consistent with recent experimental measurements. This work also demonstrates the validity of this theoretical framework based on the phonon quasiparticle to study the structural stability and phase transitions in strongly anharmonic materials.},
author = {Lu, Y. and Sun, T. and Zhang, Ping and Zhang, P. and Zhang, D. B. and Wentzcovitch, R. M.},
doi = {10.1103/PhysRevLett.118.145702},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Lu et al. - 2017 - Premelting hcp to bcc Transition in Beryllium.pdf:pdf},
issn = {10797114},
journal = {Physical Review Letters},
number = {14},
title = {{Premelting hcp to bcc Transition in Beryllium}},
url = {https://journals.aps.org/prl/pdf/10.1103/PhysRevLett.118.145702},
volume = {118},
year = {2017}
}
@article{Palanivel2000,
abstract = {High-pressure electronic properties of Be have been investigated theoretically be means of ab initio electronic structure calculations. The calculations have been carried out by the semi-relativistic full-potential, linear muffin-tin orbital (FPLMTO) method, within the local density approximation. The crystal structure stability among the hcp, bcc and orthorhombic (distorted hcp) phases has been studied as a function of compression. The bcc structure is found to be energetically stable at pressures above 180 GPa. From the results of our calculations, the orthorhombic phase cannot occur as an intermediate phase between the ambient pressure hcp phase and the high-pressure bcc structure. Our work thus suggests the need for more accurate high-pressure x-ray data.},
author = {Palanivel, B. and Rao, R. S. and Godwal, B. K. and Sikka, S. K.},
doi = {10.1088/0953-8984/12/41/309},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/B{\_}Palanivel{\_}2000{\_}J.{\_}Phys.{\_}{\_}Condens.{\_}Matter{\_}12{\_}8831.pdf:pdf},
issn = {09538984},
journal = {Journal of Physics Condensed Matter},
number = {41},
pages = {8831--8836},
title = {{On the relative stability of orthorhombic and hcp phases of beryllium at high pressures}},
volume = {12},
year = {2000}
}
@article{Sinko2005a,
abstract = {Ab initio electronic-structure calculations, based on the density-functional theory and the full-potential linear-muffin-tin-orbital method, were used to predict crystal-sructure phase stabilities and elastic constants of beryllium under compression. Specific energies, pressures, elastic constants, and Debye temperatures for three crystal structures, hcp, bcc, and fcc, were calculated over a wide volume range. In agreement with experiments and previous theoretical calculations, the hcp ground state is obtained at ambient conditions and the bcc ground state is found at high pressure and ambient temperature, with the predicted hcp→bcc phase transition at about 2.7 Mbar. A possible phase diagram of beryllium, including hcp, bcc, and fcc phases is constructed in the (P,T) plane.},
author = {Sin'ko, G. V. and Smirnov, N. A.},
doi = {10.1103/PhysRevB.71.214108},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Sin'ko, Smirnov - 2005 - Relative stability and elastic properties of hcp, bcc, and fcc beryllium under pressure.pdf:pdf},
issn = {1098-0121},
journal = {Physical Review B},
month = {jun},
number = {21},
pages = {214108},
title = {{Relative stability and elastic properties of hcp, bcc, and fcc beryllium under pressure}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.71.214108},
volume = {71},
year = {2005}
}


@inproceedings{Robert2006a,
  title={Equation of state and elastic properties of beryllium from first principles calculations},
  author={Robert, G and Sollier, A},
  booktitle={Journal de Physique IV (Proceedings)},
  volume={134},
  pages={257--262},
  year={2006},
  organization={EDP sciences}
}

@article{Luo2012,
abstract = {We investigate the phase transition, elastic constants, phonon dispersion curves, and thermal properties of beryllium (Be) at high pressures and high temperatures using density functional theory. By comparing the Gibbs free energy, in the quasiharmonic approximation (QHA), of hexagonal-closed-packed (hcp) with those of the face-centered cubic (fcc) and body-centered-cubic (bcc) we find that the hcp Be is stable up to 390 GPa, and then transforms to the bcc Be. The calculated phonon dispersion curves are in excellent agreement with experiments. Under compression, the phonon dispersion curves of hcp Be do not show any anomaly or instability. At low pressure the phonon dispersion of bcc Be display imaginary along $\Omega$-N in the T 1 branches. Within the quasiharmonic approximation, we predict the thermal equation of state and other properties including the thermal expansion coefficient, Hugoniot curves, heat capacity, Gr{\"{u}}neisen parameter, and Debye temperature. {\textcopyright} 2012 American Institute of Physics.},
author = {Luo, Fen and Cai, Ling Cang and Chen, Xiang Rong and Jing, Fu Qian and Alf, Dario},
doi = {10.1063/1.3688344},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Luo et al. - 2012 - Ab initio calculation of lattice dynamics and thermodynamic properties of beryllium.pdf:pdf},
issn = {00218979},
journal = {Journal of Applied Physics},
number = {5},
title = {{Ab initio calculation of lattice dynamics and thermodynamic properties of beryllium}},
volume = {111},
year = {2012}
}

@article{Song2007,
author = {Song, Hai Feng and Liu, Hai Feng},
doi = {10.1103/PhysRevB.75.245126},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {24},
pages = {1--7},
title = {{Modified mean-field potential approach to thermodynamic properties of a low-symmetry crystal: Beryllium as a prototype}},
volume = {75},
year = {2007}
}


@article{Robert2010,
author = {Robert, G. and Legrand, P. and Bernard, S.},
doi = {10.1103/PhysRevB.82.104118},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Robert, Legrand, Bernard - 2010 - Multiphase equation of state and elastic moduli of solid beryllium from first principles.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {10},
title = {{Multiphase equation of state and elastic moduli of solid beryllium from first principles}},
url = {https://journals.aps.org/prb/pdf/10.1103/PhysRevB.82.104118},
volume = {82},
year = {2010}
}

@article{Xian2019b,
author = {Xian, Jia Wei and Yan, Jun and Liu, Hai Feng and Sun, Tao and Zhang, Gong Mu and Gao, Xing Yu and Song, Hai Feng},
doi = {10.1103/PhysRevB.99.064102},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Xian et al. - 2019 - Effect of anharmonicity on the hcp to bcc transition in beryllium at high-pressure and high-temperature conditions.pdf:pdf},
issn = {24699969},
journal = {Physical Review B},
keywords = {doi:10.1103/PhysRevB.99.064102 url:https://doi.org},
number = {6},
pages = {1--12},
publisher = {American Physical Society},
title = {{Effect of anharmonicity on the hcp to bcc transition in beryllium at high-pressure and high-temperature conditions}},
volume = {99},
year = {2019}
}
@article{Clark2008,
abstract = {Inertial confinement fusion capsules are critically dependent on the integrity of their hot spots to ignite. At the time of ignition, only a certain fractional perturbation of the nominally spherical hot spot boundary can be tolerated and the capsule still achieve ignition. The degree to which the expected hot spot perturbation in any given capsule design is less than this maximum tolerable perturbation is a measure of the ignition margin or robustness of that design. Moreover, since there will inevitably be uncertainties in the initial character and implosion dynamics of any given capsule, all of which can contribute to the eventual hot spot perturbation, quantifying the robustness of that capsule against a range of parameter variations is an important consideration in the capsule design. Here, the robustness of the 300 eV indirect drive target design for the National Ignition Facility [Lindl, Phys. Plasmas 11, 339 (2004)] is studied in the parameter space of inner ice roughness, implosion velocity, and capsule scale. A suite of 2000 two-dimensional simulations, run with the radiation hydrodynamics code LASNEX, is used as the data base for the study. For each scale, an ignition region in the two remaining variables is identified and the ignition cliff is mapped. In accordance with the theoretical arguments of Levedahl and Lindl [Nucl. Fusion 37, 165 (1997)] and Kishony and Shvarts [Phys. Plasmas 8, 4925 (2001)], the location of this cliff is fitted to a power law of the capsule implosion velocity and scale. It is found that the cliff can be quite well represented in this power law form, and, using this scaling law, an assessment of the overall (one- and two-dimensional) ignition margin of the design can be made. The effect on the ignition margin of an increase or decrease in the density of the target fill gas is also assessed. {\textcopyright} 2008 American Institute of Physics.},
author = {Clark, Daniel S. and Haan, Steven W. and Salmonson, Jay D.},
doi = {10.1063/1.2890123},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.2890123.pdf:pdf},
issn = {1070664X},
journal = {Physics of Plasmas},
number = {5},
title = {{Robustness studies of ignition targets for the National Ignition Facility in two dimensions}},
volume = {15},
year = {2008}
}

@article{Martin1959,
author = {Martin, A.J. and Moore, A.},
doi = {10.1016/0022-5088(59)90045-1},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Unknown - 1959 - to sudden changes in furnace voltage , and also served to cut down convection currents in the argon atmosphere . Heati.pdf:pdf},
issn = {00225088},
journal = {Journal of the Less Common Metals},
month = {apr},
number = {2},
pages = {85--93},
title = {{The structure of beryllium, with particular reference to temperatures above 1200$^{\text{o}}$C}},
url = {https://linkinghub.elsevier.com/retrieve/pii/0022508859900451},
volume = {1},
year = {1959}
}
@article{Ming1984a,
abstract = {In situ high-pressure X-ray diffraction data for polycrystalline beryllium to 28.3 GPA at ambient temperature show that beryllium is transformed from the HCP phase (I) into a slightly distorted HCP phase (II) at pressures between 8.6 and 14.5 GPa. The volume change for the transition is extremely small ( approximately 0.4{\%}); the effect of pressure on the c/a ratio for both the Be(I) and Be(II) phases is also very small.},
author = {Ming, L. C. and Manghnani, M. H.},
doi = {10.1088/0305-4608/14/1/001},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/L{\_}C{\_}Ming{\_}1984{\_}J.{\_}Phys.{\_}F{\_}{\_}Met.{\_}Phys.{\_}14{\_}L1.pdf:pdf},
issn = {03054608},
journal = {Journal of Physics F: Metal Physics},
number = {1},
title = {{Isothermal compression and phase transition in beryllium to 28.3 GPa}},
volume = {14},
year = {1984}
}

@article{Vijayakumar1984b,
abstract = {The metal beryllium (Be) has been studied under high pressure using an electrical resistivity technique with in situ pressure calibration. A sluggish phase transition at 12 GPa is observed which the authors identify as the HCP to distorted HCP phase transition reported in a recent high-pressure X-ray diffraction study. However, a reanalysis of the X-ray data on the high-pressure phase Be(II) indicates that a smaller orthorhombic cell with four atoms fits the observed interplanar spacings. The observed intensity ratios of the diffraction lines can be explained reasonably well on the basis of the space group P2 1 2 1 2 with four Be atoms occupying 4c positions.},
author = {Vijayakumar, V. and Godwal, B. K. and Vohra, Y. K. and Sikka, S. K. and Chidambaram, R.},
doi = {10.1088/0305-4608/14/5/002},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Vijayakumar et al. - 1984 - On the high-pressure phase transition in beryllium metal.pdf:pdf},
issn = {03054608},
journal = {Journal of Physics F: Metal Physics},
number = {5},
title = {{On the high-pressure phase transition in beryllium metal}},
volume = {14},
year = {1984}
}

@article{Lazicki2012b,
author = {Lazicki, Amy and Dewaele, Agn{\`{e}}s and Loubeyre, Paul and Mezouar, Mohamed},
doi = {10.1103/PhysRevB.86.174118},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Lazicki et al. - 2012 - High-pressure-temperature phase diagram and the equation of state of beryllium.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {17},
pages = {1--10},
title = {{High-pressure-temperature phase diagram and the equation of state of beryllium}},
volume = {86},
year = {2012}
}


@article{Nakano2002b,
author = {Nakano, Kazutaka and Akahama, Yuichi and Kawamura, Haruki},
doi = {10.1088/0953-8984/14/44/334},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Nakano, Akahama, Kawamura - 2002 - X-ray diffraction study of Be to megabar pressure.pdf:pdf},
issn = {09538984},
journal = {Journal of Physics Condensed Matter},
number = {44 SPEC ISS.},
pages = {10569--10573},
title = {{X-ray diffraction study of Be to megabar pressure}},
volume = {14},
year = {2002}
}


@article{McCoy2019a,
author = {McCoy, Chad A. and Knudson, Marcus D. and Desjarlais, Michael P.},
doi = {10.1103/PhysRevB.100.054107},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevB.100.054107.pdf:pdf},
issn = {24699969},
journal = {Physical Review B},
keywords = {doi:10.1103/PhysRevB.100.054107 url:https://doi.or},
number = {5},
pages = {1--13},
publisher = {American Physical Society},
title = {{Sound velocity, shear modulus, and shock melting of beryllium along the Hugoniot}},
volume = {100},
year = {2019}
}

@article{Brown2014a,
abstract = {A magnetohydrodynamic loading technique was used to shocklessly compress beryllium to peak longitudinal stresses of 19-110 GPa and, subsequently, unload in order to determine both the compressive response and also the shear stress supported upon release. Loading strain rates were on the order of 10 6s-1, while the unloading rates were nearly constant at 3 × 105s-1. Velocimetry was used to monitor the ramp and release behavior of a beryllium/lithium fluoride window interface. After applying window corrections to infer in situ beryllium velocities, a Lagrangian analysis was employed to determine the material response. The Lagrangian wavespeed-particle velocity response is integrated to generate the stress-strain path, average change in shear stress over the elastic unloading, and estimates of the shear modulus at peak compression. These data are used to infer the pressure dependence of the flow strength at the unloading rate. Comparisons to several strength models reveal good agreement to 45 GPa, but the data indicate 20{\%}-30{\%} higher strength near 100 GPa. {\textcopyright} 2014 AIP Publishing LLC.},
author = {Brown, J. L. and Knudson, M. D. and Alexander, C. S. and Asay, J. R.},
doi = {10.1063/1.4890232},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/1.4890232.pdf:pdf},
issn = {10897550},
journal = {Journal of Applied Physics},
number = {3},
title = {{Shockless compression and release behavior of beryllium to 110 GPa}},
url = {http://dx.doi.org/10.1063/1.4890232},
volume = {116},
year = {2014}
}
@article{Wang2013a,
abstract = {We have calculated the equations of state, the viscosity and self-diffusion coefficients, and electronic transport coefficients of beryllium in the warm dense regime for densities from 4.0 to 6.0 g/cm3 and temperatures from 1.0 to 10.0 eV by using quantum molecular dynamics simulations. The principal Hugoniot curve is in agreement with underground nuclear explosive and high-power laser experimental results up to ∼20 Mbar. The calculated viscosity and self-diffusion coefficients are compared with the one-component plasma model, using effective charges given by the average-atom model. The Stokes-Einstein relationship, which connects viscosity and self-diffusion coefficients, is found to hold fairly well in the strong coupling regime. The Lorenz number, which is the ratio between thermal and electrical conductivities, is computed via Kubo-Greenwood formula and compared to the well-known Wiedemann-Franz law in the warm dense region. {\textcopyright} 2013 American Physical Society.},
author = {Wang, Cong and Long, Yao and Tian, Ming Feng and He, Xian Tu and Zhang, Ping},
doi = {10.1103/PhysRevE.87.043105},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevE.87.043105.pdf:pdf},
issn = {15393755},
journal = {Physical Review E - Statistical, Nonlinear, and Soft Matter Physics},
number = {4},
pages = {1--6},
title = {{Equations of state and transport properties of warm dense beryllium: A quantum molecular dynamics study}},
volume = {87},
year = {2013}
}




@article{Evans2005a,
abstract = {We report combined x-ray and Raman studies of beryllium in helium and argon pressure media at pressures approaching 200 GPa. Our results are generally consistent with recent studies confirming the stability of the hexagonal close-packed phase to the highest pressures. However, the quasihydrostatic conditions of our studies lead to a stiffer equation of state (K0=109.88, K′0=3.59) and a gradual approach toward a more ideal c∕a ratio of 1.60 at 180 GPa. Combining our Raman and equation of state data, we are able to evaluate the pressure dependence of the elastic shear modulus (C44=109.3, C′44=1.959). We discuss the comparison of our results with measurements using ultrasonic and dynamic techniques.},
author = {Evans, W. J. and Lipp, M. J. and Cynn, H. and Yoo, C. S. and Somayazulu, M. and H{\"{a}}usermann, D. and Shen, G. and Prakapenka, V.},
doi = {10.1103/PhysRevB.72.094113},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Evans et al. - 2005 - X-ray diffraction and Raman studies of beryllium Static and elastic properties at high pressures.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {9},
pages = {1--6},
title = {{X-ray diffraction and Raman studies of beryllium: Static and elastic properties at high pressures}},
volume = {72},
year = {2005}
}




@article{Nellis2003b,
author = {Nellis, W. J. and Mitchell, A. C. and Young, D. A.},
doi = {10.1063/1.1529071},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/1.1529071.pdf:pdf},
issn = {00218979},
journal = {Journal of Applied Physics},
number = {1},
pages = {304--310},
title = {{Equation-of-state measurements for aluminum, copper, and tantalum in the pressure range 80-440 GPa (0.8-4.4 Mbar)}},
volume = {93},
year = {2003}
}


@article{Velisavljevic2002a,
abstract = {The structural and electrical properties of alkaline-earth metal beryllium were studied to 66 GPa using designer diamond anvils. The ambient pressure hexagonal close-packed phase was found to be stable to the highest pressure of 66 GPa and the measured static equation of state differs substantially from the one derived from the existing shock wave data. The electrical resistance data at high pressure shows a gradual decrease in resistance to pressure up to 25 GPa followed by a slight increase to 53 Gpa. The axial ratio (c/a) remains strongly nonideal with c/a = 1.562 at V/V 0  = 0.708, indicating that deviations from nearly free electron behavior are still dominant at high compressions.},
author = {Velisavljevic, Nenad and Chesnut, Gary N. and Vohra, Yogesh K. and Weir, Samuel T. and Malba, Vincent and Akella, Jagannadham},
doi = {10.1103/PhysRevB.65.172107},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Velisavljevic et al. - 2002 - Structural and electrical properties of beryllium metal to 66 GPa studied using designer diamond anvils.pdf:pdf},
issn = {01631829},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {17},
pages = {1721071--1721074},
title = {{Structural and electrical properties of beryllium metal to 66 GPa studied using designer diamond anvils}},
volume = {65},
year = {2002}
}


@article{Cauble1998b,
  title={Absolute equation-of-state data in the 10--40 Mbar (1--4 TPa) regime},
  author={Cauble, R and Perry, TS and Bach, DR and Budil, KS and Hammel, BA and Collins, GW and Gold, DM and Dunn, J and Celliers, P and Da Silva, LB and others},
  journal={Physical review letters},
  volume={80},
  number={6},
  pages={1248},
  year={1998},
  publisher={APS}
}

@article{Boivineau1993a,
abstract = {A submillisecond resistive heating technique under high pressure (0.12 GPa) has been used to measure selected thermophysical properties of both solid and liquid beryllium. Data have been obtained between room temperature and 2900 K. Results on enthalpy, volume expansion, electrical resistivity, and sound velocity measurements are presented. {\textcopyright} 1993 Plenum Publishing Corporation.},
author = {Boivineau, M. and Arl{\'{e}}s, L. and Vermeulen, J. M. and Th{\'{e}}venin, Th},
doi = {10.1007/BF00566042},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Boivineau1993{\_}Article{\_}ThermophysicalPropertiesOfSoli.pdf:pdf},
issn = {0195928X},
journal = {International Journal of Thermophysics},
keywords = {beryllium,electrical resistivity,enthalpy,high pressure,high temperature,isobaric expansion,liquid metals,sound velocity},
number = {3},
pages = {427--439},
title = {{Thermophysical properties of solid and liquid beryllium}},
volume = {14},
year = {1993}
}
@article{Swenson1991a,
abstract = {Linear thermal expansivity measurements from 4.2 to 302 K and heat capacity measurements from 4.6 to 108 K have been made on HIP (hot isostatic pressing) beryllium metal. The heat capacity data are in good agreement with previous data from 1.4 to 30 K for high purity single crystals. Our $\Theta$0 = 1485(5) K also agrees well with that calculated from high-pressure elastic constant results. The linear thermal expansivity decreases rapidly with decreasing temperature from 1.13 × 10-5 K-1 at 293 K, as would be expected for the large $\Theta$0, and becomes very small ({\textless} 10-7 K-1) below 50 K. The expansivities below 108 K are consistent with a constant $\gamma$lat0 = 1.15 and with $\gamma$lat0 = 0.91 from the high-pressure elastic constant results.},
author = {Swenson, C. A.},
doi = {10.1063/1.349336},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/1.349336.pdf:pdf},
issn = {00218979},
journal = {Journal of Applied Physics},
number = {6},
pages = {3046--3051},
title = {{HIP beryllium: Thermal expansivity from 4 to 300 K and heat capacity from 1 to 108 K}},
volume = {70},
year = {1991}
}


@article{Ragan1982b,
abstract = {A shock wave generated by an underground nuclear explosion was used to perform impedance-matching experiments for several different materials at pressures from 1 to 7 TPa. The nearly planar shock passed through a 180-mm-diam by 12-mm-thick molybdenum standard and into stacks of 10-mm-thick samples of the following adjacent pairs of materials: LiD-Be, Be-LiD, Al-Mo, Pb-quartz, W-Mo (low density, 0=8.29 g cm-3), U-Mo, and Fe. An array of 75 electrical contact pins was used to determine the shape of the shock front and the shock velocities in the standard and in the samples with uncertainties ranging from 1.5 to 2.5{\%}. The measured shock velocity of 27.30 km/s (1.5{\%}) in the molybdenum standard corresponds to a pressure of 4.95 TPa (3.5{\%}) based on a theoretical equation of state (EOS) that includes electronic-shell-structure effects. An impedance-matching analysis was performed for each sample stack to obtain Hugoniot data for all samples except those in the U-Mo stack; neutron-induced fission heating in the uranium perturbed the initial state and produced inconclusive results. Predictions, based on the SESAME EOS library, of shock velocities in most samples agree with the experimental results within the uncertainties. For the quartz and low-density molybdenum, the SESAME-predicted shock velocities are too large by 5 to 10{\%}. The following Hugoniot points in pressure (P)-particle-velocity (u) coordinates were determined for the indicated samples: LiD (p=0.946 TPa, u=29.39 km/s), Be (1.46, 22.69); Be (1.79, 25.42), LiD (1.038, 31.23); Al (2.23, 23.89), Mo (4.03, 16.05); Pb (4.80, 17.84), quartz (1.66, 23.64); W (6.51, 15.10), and Mo (0=8.29 g cm-3) (3.68, 18.27). The results for iron have a larger uncertainty but are consistent with the SESAME predictions. {\textcopyright} 1982 The American Physical Society.},
author = {Ragan, Charles E.},
doi = {10.1103/PhysRevA.25.3360},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevA.25.3360.pdf:pdf},
issn = {10502947},
journal = {Physical Review A},
number = {6},
pages = {3360--3375},
title = {{Shock compression measurements at 1 to 7 TPa}},
volume = {25},
year = {1982}
}

@inproceedings{Wise1982b,
author = {Wise, J. L. and Chhabildas, L. C. and Asay, J. R.},
booktitle = {AIP Conference Proceeding Volume 78},
doi = {10.1063/1.33350},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/1.33350.pdf:pdf},
pages = {417--421},
publisher = {AIP},
title = {{Shock compression of beryllium}},
url = {http://aip.scitation.org/doi/abs/10.1063/1.33350},
volume = {417},
year = {1982}
}


@article{Walsh1957b,
author = {Walsh, John M. and Rice, Melvin H. and McQueen, Robert G. and Yarger, Frederick L.},
doi = {10.1103/PhysRev.108.196},
issn = {0031899X},
journal = {Physical Review},
number = {2},
pages = {196--216},
title = {{Shock-wave compressions of twenty-seven metals. equations of state of metals}},
volume = {108},
year = {1957}
}
@article{Gordon1949a,
abstract = {A high temperature precision x-ray camera has been designed and constructed by modification of the familiar back-reflection symmetrical focusing type of camera. The camera, specimen, and furnace are used within a vacuum chamber to avoid oxidation. The apparatus in its present form has been employed at temperatures up to 1000°C, but higher temperatures could be easily attained by making a few minor changes in the furnace materials. The lattice parameters of beryllium have been measured up to 1000°C. The derived coefficients of thermal expansion, both linear and bulk, are presented as a function of temperature. In addition, the data present strong evidence that the hexagonal close packed form of beryllium which exists at room temperature is stable up to at least 1000°C, contrary to several reports in the literature.},
author = {Gordon, Paul},
doi = {10.1063/1.1698252},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/1.1698252.pdf:pdf},
issn = {00218979},
journal = {Journal of Applied Physics},
number = {10},
pages = {908--917},
title = {{A high temperature precision x-ray camera: Some measurements of the thermal coefficients of expansion of beryllium}},
volume = {20},
year = {1949}
}
@article{Wang1991a,
abstract = {For a uniform electron gas of density n=n+n=3/4rs3=ks6/192 and spin polarization =(n-n)/n, we study the Fourier transform c(k,rs,) of the correlation hole, as well as the correlation energy c(rs,)=F0dk c/. In the high-density (rs0) limit, we find a simple scaling relation ksc/g2f(z,), where z=k/gks, g=[(1+)2/3+(1-)2/3]/2, and f(z,1)=f(z,0). The function f(z,) is only weakly dependent, and its small-z expansion -3z/2+4 3 z2/2+... is also the exact small-wave-vector (k0) expansion for any rs or. Motivated by these considerations, and by a discussion of the large-wave-vector and low-density limits, we present two Pad{\'{e}} representations for c at any k, rs, or ,one within and one beyond the random-phase approximation (RPA). We also show that cRPA obeys a generalization of Misawas spin-scaling relation for cRPA, and that the low-density (rs) limit of cRPA is rs-3/4. {\textcopyright} 1991 The American Physical Society.},
author = {Wang, Yue and Perdew, John P.},
doi = {10.1103/PhysRevB.44.13298},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/caratio high pressure/PhysRevB.44.13298.pdf:pdf},
issn = {01631829},
journal = {Physical Review B},
number = {24},
pages = {13298--13307},
title = {{Correlation hole of the spin-polarized electron gas, with exact small-wave-vector and high-density scaling}},
volume = {44},
year = {1991}
}
@article{Kresse1996f,
abstract = {We present a detailed description and comparison of algorithms for performing ab-initio quantum-mechanical calculations using pseudopotentials and a plane-wave basis set. We will discuss: (a) partial occupancies within the framework of the linear tetrahedron method and the finite temperature density-functional theory, (b) iterative methods for the diagonalization of the Konn-Sham Hamiltonian and a discussion of an efficient iterative method based on the ideas of Pulay's residual minimization, which is close to an order N2atoms scaling even for relatively large systems, (c) efficient Broyden-like and Pulay-like mixing methods for the charge density including a new special 'preconditioning' optimized for a plane-wave basis set, (d) conjugate gradient methods for minimizing the electronic free energy with respect to all degrees of freedom simultaneously. We have implemented these algorithms within a powerful package called VAMP (Vienna ab-initio molecular-dynamics package). The program and the techniques have been used successfully for a large number of different systems (liquid and amorphous semiconductors, liquid simple and transition metals, metallic and semi-conducting surfaces, phonons in simple metals, transition metals and semiconductors) and turned out to be very reliable.},
author = {Kresse, G. and Furthm{\"{u}}ller, J.},
doi = {10.1016/0927-0256(96)00008-0},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/1-s2.0-0927025696000080-main (1).pdf:pdf},
issn = {09270256},
journal = {Computational Materials Science},
number = {1},
pages = {15--50},
title = {{Efficiency of ab-initio total energy calculations for metals and semiconductors using a plane-wave basis set}},
volume = {6},
year = {1996}
}
@article{Vanderbilt1990a,
abstract = {These instructions indicate how to prepare a manuscript for rapid publication in GASTROENTEHOLOGY and exemplify the exact format to follow. {\textcopyright} 1977, The Williams {\&} Wilkins Co.. All rights reserved.},
author = {Vanderbilt, David},
doi = {10.1103/PhysRevB.41.7892},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevB.41.7892.pdf:pdf},
issn = {0163-1829},
journal = {Physical Review B},
month = {apr},
number = {11},
pages = {7892--7895},
pmid = {18235770},
title = {{Soft self-consistent pseudopotentials in a generalized eigenvalue formalism}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.41.7892},
volume = {41},
year = {1990}
}
@article{Kresse1999b,
abstract = {The formal relationship between ultrasoft (US) Vanderbilt-type pseudopotentials and Bl{\"{o}}chl's projector augmented wave (PAW) method is derived. It is shown that the total energy functional for US pseudopotentials can be obtained by linearization of two terms in a slightly modified PAW total energy functional. The Hamilton operator, the forces, and the stress tensor are derived for this modified PAW functional. A simple way to implement the PAW method in existing plane-wave codes supporting US pseudopotentials is pointed out. In addition, critical tests are presented to compare the accuracy and efficiency of the PAW and the US pseudopotential method with relaxed core all electron methods. These tests include small molecules (Formula presented) and several bulk systems (diamond, Si, V, Li, Ca, (Formula presented) Fe, Co, Ni). Particular attention is paid to the bulk properties and magnetic energies of Fe, Co, and Ni. {\textcopyright} 1999 The American Physical Society.},
author = {Kresse, G. and Joubert, D.},
doi = {10.1103/PhysRevB.59.1758},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevB.59.1758.pdf:pdf},
issn = {0163-1829},
journal = {Physical Review B},
month = {jan},
number = {3},
pages = {1758--1775},
title = {{From ultrasoft pseudopotentials to the projector augmented-wave method}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.59.1758},
volume = {59},
year = {1999}
}
@article{Kresse1996e,
abstract = {We present an efficient scheme for calculating the Kohn-Sham ground state of metallic systems using pseudopotentials and a plane-wave basis set. In the first part the application of Pulay's DIIS method (direct inversion in the iterative subspace) to the iterative diagonalization of large matrices will be discussed. Our approach is stable, reliable, and minimizes the number of order (Formula presented) operations. In the second part, we will discuss an efficient mixing scheme also based on Pulay's scheme. A special “metric” and a special “preconditioning” optimized for a plane-wave basis set will be introduced. Scaling of the method will be discussed in detail for non-self-consistent and self-consistent calculations. It will be shown that the number of iterations required to obtain a specific precision is almost independent of the system size. Altogether an order (Formula presented) scaling is found for systems containing up to 1000 electrons. If we take into account that the number of k points can be decreased linearly with the system size, the overall scaling can approach (Formula presented). We have implemented these algorithms within a powerful package called VASP (Vienna ab initio simulation package). The program and the techniques have been used successfully for a large number of different systems (liquid and amorphous semiconductors, liquid simple and transition metals, metallic and semiconducting surfaces, phonons in simple metals, transition metals, and semiconductors) and turned out to be very reliable. {\textcopyright} 1996 The American Physical Society.},
author = {Kresse, G. and Furthm{\"{u}}ller, J.},
doi = {10.1103/PhysRevB.54.11169},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevB.54.11169.pdf:pdf},
issn = {1550235X},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {16},
pages = {11169--11186},
pmid = {9984901},
title = {{Efficient iterative schemes for ab initio total-energy calculations using a plane-wave basis set}},
volume = {54},
year = {1996}
}

@article{P.E.Blochl1994c,
author = {P.E.Bl{\"{o}}chl},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/P.E.Bl{\"{o}}chl - 1994 - Projector augmented-wave method.pdf:pdf},
journal = {Physical Review B},
number = {24},
pages = {17953--17979},
title = {{Projector augmented-wave method}},
volume = {50},
year = {1994}
}
@article{Monkhorst1976b,
abstract = {It is again emphasized that for all cubic lattices the method of Monkhorst and Pack generates not only point sets identical to those obtained by Chadi and Cohen, but also intermediate sets with the same properties. In addition, a comparison of these two methods for the hexagonal lattice reveals our method to be more flexible and efficient. {\textcopyright} 1977 The American Physical Society.},
author = {Monkhorst, Hendrik J. and Pack, James D.},
doi = {10.1103/PhysRevB.13.5188},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevB.13.5188.pdf:pdf},
issn = {0556-2805},
journal = {Physical Review B},
month = {jun},
number = {12},
pages = {5188--5192},
title = {{Special points for Brillouin-zone integrations}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.16.1748 https://link.aps.org/doi/10.1103/PhysRevB.13.5188},
volume = {13},
year = {1976}
}
@article{Perdew1996,
author = {Perdew, John P and Burke, Kieron and Ernzerhof, Matthias},
doi = {10.1103/PhysRevLett.77.3865},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Perdew, Burke, Ernzerhof - 1996 - Generalized Gradient Approximation Made Simple.pdf:pdf},
issn = {0031-9007},
journal = {Physical Review Letters},
month = {oct},
number = {18},
pages = {3865--3868},
title = {{Generalized Gradient Approximation Made Simple}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.77.3865},
volume = {77},
year = {1996}
}
@article{Nose1984a,
abstract = {Three recently proposed constant temperature molecular dynamics methods by: (i) Nos{\'{e}} (Mol. Phys., to be published); (ii) Hoover et al. [Phys. Rev. Lett. 48, 1818 (1982)], and Evans and Morriss [Chem. Phys. 77, 63 (1983)]; and (iii) Haile and Gupta [J. Chem. Phys. 79, 3067 (1983)] are examined analytically via calculating the equilibrium distribution functions and comparing them with that of the canonical ensemble. Except for effects due to momentum and angular momentum conservation, method (i) yields the rigorous canonical distribution in both momentum and coordinate space. Method (ii) can be made rigorous in coordinate space, and can be derived from method (i) by imposing a specific constraint. Method (iii) is not rigorous and gives a deviation of order N -1/2 from the canonical distribution (N the number of particles). The results for the constant temperature-constant pressure ensemble are similar to the canonical ensemble case. {\textcopyright} 1984 American Institute of Physics.},
author = {Nos{\'{e}}, Shuichi},
doi = {10.1063/1.447334},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Nose/1.447334.pdf:pdf},
issn = {00219606},
journal = {The Journal of Chemical Physics},
number = {1},
pages = {511--519},
title = {{A unified formulation of the constant temperature molecular dynamics methods}},
volume = {81},
year = {1984}
}
@article{Nose1991,
author = {Nos{\'{e}}, Shuichi},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Nose/103-1.pdf:pdf},
journal = {Progress of Theoretical Physics Supplement},
number = {103},
pages = {1--46},
title = {{Constant Temperature Molecular Dynamics Methods Limitations in simulations in the microcanonical ensemble}},
year = {1991}
}

@article{Polson2000a,
author = {Polson, J. M. and Trizac, E. and Pronk, S. and Frenkel, D.},
doi = {10.1063/1.481102},
file = {:Users/wjz8597/Library/Mobile Documents/3L68KQB4HG{\~{}}com{\~{}}readdle{\~{}}CommonDocuments/Documents/Computational Chemistry/1.481102.pdf:pdf},
issn = {00219606},
journal = {Journal of Chemical Physics},
number = {12},
pages = {5339--5342},
title = {{Finite-size corrections to the free energies of crystalline solids}},
volume = {112},
year = {2000}
}

@article{Frenkel1984,
author = {Frenkel, Daan and Ladd, Anthony J. C.},
doi = {10.1063/1.448024},
file = {:Users/wjz8597/Library/Mobile Documents/3L68KQB4HG{\~{}}com{\~{}}readdle{\~{}}CommonDocuments/Documents/Computational Chemistry/1.448024.pdf:pdf},
issn = {0021-9606},
journal = {The Journal of Chemical Physics},
month = {oct},
number = {7},
pages = {3188--3193},
title = {{New Monte Carlo method to compute the free energy of arbitrary solids. Application to the fcc and hcp phases of hard spheres}},
url = {http://aip.scitation.org/doi/10.1063/1.448024},
volume = {81},
year = {1984}
}


@article{Riffet2020,
author = {Riffet, Vanessa and Amadon, Bernard and Bruzy, Nicolas and Denoual, Christophe},
doi = {10.1103/PhysRevMaterials.4.063609},
issn = {2475-9953},
journal = {Physical Review Materials},
keywords = {doi:10.1103/PhysRevMaterials.4.063609 url:https://},
mendeley-groups = {Beryllium},
month = {jun},
number = {6},
pages = {063609},
publisher = {American Physical Society},
title = {{Role of dislocations in the bcc-hcp transition under high pressure: A first-principles approach in beryllium}},
url = {https://link.aps.org/doi/10.1103/PhysRevMaterials.4.063609},
volume = {4},
year = {2020}
}


@article{Dremov2015,
author = {Dremov, V. V. and Rykounov, A. A. and Sapozhnikov, F. A. and Karavaev, A. V. and Yakovlev, S. V. and Ionov, G. V. and Ryzhkov, M. V.},
doi = {10.1063/1.4923430},
issn = {0021-8979},
journal = {Journal of Applied Physics},
mendeley-groups = {Beryllium},
month = {jul},
number = {3},
pages = {035901},
title = {{Cold melting of beryllium: Atomistic view on Z-machine experiments}},
url = {http://dx.doi.org/10.1063/1.4923430 http://aip.scitation.org/doi/10.1063/1.4923430},
volume = {118},
year = {2015}
}


@inproceedings{Thompson2012,
author = {Thompson, Aidan P. and Lane, J. Matthew D and Desjarlais, Michael},
booktitle = {AIP Conference Proceedings},
doi = {10.1063/1.3686522},
file = {:Users/fgonzalez/Library/Application Support/Mendeley Desktop/Downloaded/Thompson, Lane, Desjarlais - 2012 - AIP Conference Proceedings.pdf:pdf},
isbn = {9780735410060},
issn = {0094243X},
keywords = {MEAM,Molecular dynamics,thermodynamic and mechanical properties},
mendeley-groups = {Beryllium},
pages = {1311--1314},
title = {{Molecular dynamics simulation of dynamic response of beryllium}},
url = {http://aip.scitation.org/doi/abs/10.1063/1.3686522},
volume = {1426},
year = {2012}
}

@article{Karavaev2016,
author = {Karavaev, A V and Dremov, V V and Pravishkina, T A},
doi = {http://dx.doi.org/10.1016/j.commatsci.2016.08.014},
file = {:Users/fgonzalez/Library/Application Support/Mendeley Desktop/Downloaded/Karavaev, Dremov, Pravishkina - 2016 - Computational Materials Science.pdf:pdf},
issn = {0927-0256},
journal = {Computational Materials Science},
keywords = {Liquid-solid coexistence},
mendeley-groups = {Z-method,Melting Iron,Beryllium},
pages = {335--343},
publisher = {Elsevier B.V.},
title = {{Precise calculation of melting curves by molecular dynamics}},
url = {http://www.sciencedirect.com/science/article/pii/S0927025616303846},
volume = {124},
year = {2016}
}


@article{Guo2014,
author = {Guo, Zhi-Cheng and Luo, Fen and Cheng, Yan},
doi = {10.1016/j.commatsci.2013.12.013},
file = {:Users/fgonzalez/Library/Application Support/Mendeley Desktop/Downloaded/Pu et al. - 2015 - Computational Materials Science.pdf:pdf},
issn = {09270256},
journal = {Computational Materials Science},
keywords = {First-principles calculations,Phase transition,Thermodynamic properties},
mendeley-groups = {Beryllium},
month = {mar},
pages = {139--144},
publisher = {Elsevier B.V.},
title = {{Phase transition and thermodynamic properties of beryllium from first-principles calculations}},
url = {http://dx.doi.org/10.1016/j.commatsci.2013.12.013 https://linkinghub.elsevier.com/retrieve/pii/S0927025615000737 https://linkinghub.elsevier.com/retrieve/pii/S0927025613007623},
volume = {84},
year = {2014}
}



@article{Li2014,
author = {Li, Dafang and Zhang, Ping and Yan, Jun},
doi = {10.1038/srep04707},
file = {:Users/fgonzalez/Library/Application Support/Mendeley Desktop/Downloaded/Li, Zhang, Yan - 2014 - Scientific reports.pdf:pdf},
issn = {2045-2322},
journal = {Scientific Reports},
mendeley-groups = {Z-method,Beryllium},
month = {may},
number = {1},
pages = {4707},
pmid = {24759594},
title = {{Ab initio molecular dynamics study of high-pressure melting of beryllium oxide}},
url = {http://www.pubmedcentral.nih.gov/articlerender.fcgi?artid=3998012&tool=pmcentrez&rendertype=abstract http://www.nature.com/articles/srep04707},
volume = {4},
year = {2015}
}



@inproceedings{Coe2020,
author = {Coe, Joshua D and Rudin, Sven P and Maiorov, Boris},
booktitle = {AIP Conference Proceedings},
doi = {10.1063/12.0000902},
file = {:Users/fgonzalez/Library/Application Support/Mendeley Desktop/Downloaded/12.0000902.pdf:pdf},
isbn = {9780735440005},
mendeley-groups = {Beryllium},
pages = {070009},
title = {{Multiphase equation of state and thermoelastic data for polycrystalline beryllium}},
url = {http://aip.scitation.org/doi/abs/10.1063/12.0000902},
volume = {070009},
year = {2020}
}



@article{Gonzalez-Cataldo2016,
author = {Gonz{\'{a}}lez-Cataldo, Felipe and Davis, Sergio and Guti{\'{e}}rrez, Gonzalo},
journal = {Scientific Reports},
month = {may},
number = {October 2014},
pages = {26537},
publisher = {Nature Publishing Group},
title = {{Melting curve of SiO$_2$ at multimegabar pressures: implications for gas giants and super-Earths}},
url = {http://dx.doi.org/10.1038/srep26537 http://www.nature.com/articles/srep26537},
volume = {6},
year = {2016}
}

@article{Soubiran2020,
author = {Soubiran, Fran{\c{c}}ois and Militzer, Burkhard},
doi = {10.1103/PhysRevLett.125.175701},
issn = {0031-9007},
journal = {Physical Review Letters},
keywords = {doi:10.1103/PhysRevLett.125.175701 url:https://doi},
mendeley-groups = {MgO},
month = {oct},
number = {17},
pages = {175701},
publisher = {American Physical Society},
title = {{Anharmonicity and Phase Diagram of Magnesium Oxide in the Megabar Regime}},
url = {https://doi.org/10.1103/PhysRevLett.125.175701 https://link.aps.org/doi/10.1103/PhysRevLett.125.175701},
volume = {125},
year = {2020}
}

@article{Bouchet2019,
author = {Bouchet, J. and Bottin, F. and Recoules, V. and Remus, F. and Morard, G. and Bolis, R. M. and Benuzzi-Mounaix, A.},
doi = {10.1103/PhysRevB.99.094113},
issn = {2469-9950},
journal = {Physical Review B - Condensed Matter and Materials Physics},
keywords = {doi:10.1103/PhysRevB.99.094113 url:https://doi.org},
mendeley-groups = {MgSiO3,MgO},
month = {mar},
number = {9},
pages = {094113},
publisher = {American Physical Society},
title = {{Ab initio calculations of the B1-B2 phase transition in MgO}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.99.094113},
volume = {99},
year = {2019}
}

@article{Simon1953melting,
  title={The melting of iron at high pressures},
  author={Simon, FE},
  journal={Nature},
  volume={172},
  number={4382},
  pages={746--747},
  year={1953},
  publisher={Nature Publishing Group}
}

@inproceedings{Hanshaw2012,
author = {Hanshaw, Heath and Martin, Matthew R. and Desjarlais, Michael and Lemke, Raymond W.},
booktitle = {AIP Conference Proceedings},
doi = {10.1063/1.3686428},
file = {:Users/fgonzalez/Library/Application Support/Mendeley Desktop/Downloaded/1.3686428.pdf:pdf},
isbn = {9780735410060},
issn = {0094243X},
keywords = {Z,aluminum,double shock,quartz},
mendeley-groups = {Beryllium},
pages = {921--924},
title = {{Double shock experiments on the sandia z machine}},
url = {http://aip.scitation.org/doi/abs/10.1063/1.3686428},
volume = {1426},
year = {2012}
}
@article{Migliori2004b,
author = {Migliori, Albert and Ledbetter, Hassel and Thoma, D. J. and Darling, T. W.},
doi = {10.1063/1.1644633},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.1644633.pdf:pdf},
issn = {00218979},
journal = {Journal of Applied Physics},
number = {5},
pages = {2436--2440},
title = {{Beryllium's monocrystal and polycrystal elastic constants}},
volume = {95},
year = {2004}
}
@article{Wilson1998,
abstract = {Capsules with beryllium ablators have long been considered as alternatives to plastic for the National Ignition Facility laser [J. A. Paisner et al., Laser Focus World 30, 75 (1994)]; now the superior performance of beryllium is becoming well substantiated. Beryllium capsules have the advantages of high density, low opacity, high tensile strength, and high thermal conductivity. Three-dimensional (3-D) calculations with the HYDRA code [NTIS Document No. DE-96004569 (M. M. Marinak et al. in UCRL-LR-105821-95-3)] confirm two-dimensional (2-D) LASNEX [G. B. Zimmerman and W. L. Kruer, Comments Plasmas Phys. Controlled Thermonucl. Fusion 2, 51 (1975)] results that particular beryllium capsule designs are several times less sensitive than the CH point design to instability growth from deuterium-tritium (DT) ice roughness. These capsule designs contain more ablator mass and leave some beryllium unablated at ignition. By adjusting the level of copper dopant, the unablated mass can increase or decrease, with a corresponding decrease or increase in sensitivity to perturbations. A plastic capsule with the same ablator mass as the beryllium and leaving the same unablated mass also shows this reduced perturbation sensitivity. Beryllium's low opacity permits the creation of 250 eV capsule designs. Its high tensile strength allows it to contain DT fuel at room temperature. Its high thermal conductivity simplifies cryogenic fielding. {\textcopyright} 1998 American Institute of Physics.},
author = {Wilson, Douglas C. and Bradley, Paul A. and Hoffman, Nelson M. and Swenson, Fritz J. and Smitherman, David P. and Chrien, Robert E. and Margevicius, Robert W. and Thoma, D. J. and Foreman, Larry R. and Hoffer, James K. and Goldman, S. Robert and Caldwell, Stephen E. and Dittrich, Thomas R. and Haan, Steven W. and Marinak, Michael M. and Pollaine, Stephen M. and Sanchez, Jorge J.},
doi = {10.1063/1.872865},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.872865.pdf:pdf},
issn = {1070664X},
journal = {Physics of Plasmas},
number = {5 PART 1},
pages = {1953--1959},
title = {{The development and advantages of beryllium capsules for the National Ignition Facility}},
volume = {5},
year = {1998}
}



@inproceedings{Swift2004b,
  title={Equation of state measurements for beryllium in the ICF capsule regime},
  author={Swift, Damian and Paisley, Dennis and Knudson, Marcus},
  booktitle={AIP Conference Proceedings},
  volume={706},
  pages={119--122},
  year={2004},
  organization={American Institute of Physics}
}


@inproceedings{Chhabildas2009,
author = {Chhabildas, L. C. and Wise, J. L. and Asay, J. R.},
booktitle = {AIP Conference Proceeding Volume 78},
doi = {10.1063/1.33351},
isbn = {7804220553},
pages = {422--426},
publisher = {AIP},
title = {{Reshock and release behavior of beryllium}},
url = {http://aip.scitation.org/doi/abs/10.1063/1.33350 http://aip.scitation.org/doi/abs/10.1063/1.33351},
volume = {422},
year = {1982}
}

@inproceedings{Wise2009,
author = {Wise, J. L. and Chhabildas, L. C. and Asay, J. R.},
booktitle = {AIP Conference Proceeding Volume 78},
doi = {10.1063/1.33350},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.33350.pdf:pdf},
pages = {417--421},
publisher = {AIP},
title = {{Shock compression of beryllium}},
url = {http://aip.scitation.org/doi/abs/10.1063/1.33350},
volume = {417},
year = {1982}
}


@article{DeWijs1998,
abstract = {The melting properties of aluminum are calculated from first-principles molecular-dynamics simulations using density-functional theory in the local-density approximation. We calculate a melting temperature of 890 K at zero pressure, to be compared to the experimental value of 933 K. An elaborate discussion of the techniques employed is presented. The solid- and liquid-state free energies are obtained via coupling constant integration. The respective reference systems are the quasiharmonic crystal and the Lennard-Jones fluid. Good quality of the Brillouin zone sampling is shown to be crucial. The strategy followed is expected to be applicable to a wide range of liquid metals. {\textcopyright} 1998 The American Physical Society.},
author = {de Wijs, Gilles A. and Kresse, Georg and Gillan, Michael J.},
doi = {10.1103/PhysRevB.57.8223},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevB.57.8223.pdf:pdf},
issn = {1550235X},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {14},
pages = {8223--8234},
title = {{First-order phase transitions by first-principles free-energy calculations: The melting of Al}},
volume = {57},
year = {1998}
}


@article{Izvekov2004a,
author = {Izvekov, Sergei and Parrinello, Michele and Bumham, Christian J. and Voth, Gregory A.},
doi = {10.1063/1.1739396},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/TDI/1.1739396.pdf:pdf},
issn = {00219606},
journal = {Journal of Chemical Physics},
number = {23},
pages = {10896--10913},
title = {{Effective force fields for condensed phase systems from ab initio molecular dynamics simulation: A new method for force-matching}},
volume = {120},
year = {2004}
}


@inproceedings{GonzalezMilitzer2020,
archivePrefix = {arXiv},
arxivId = {2002.12163},
author = {Gonz{\'{a}}lez-Cataldo, Felipe and Militzer, Burkhard},
booktitle = {AIP Conference Proceedings},
doi = {10.1063/12.0000793},
eprint = {2002.12163},
file = {:Users/fgonzalez/Library/Application Support/Mendeley Desktop/Downloaded/12.0000793.pdf:pdf},
isbn = {9780735440005},
pages = {090001},
title = {{Thermal and pressure ionization in warm, dense MgSiO$_3$ studied with first-principles computer simulations}},
url = {http://arxiv.org/abs/2002.12163 http://aip.scitation.org/doi/abs/10.1063/12.0000793},
volume = {2272},
year = {2020}
}

@article{Gonzalez-Cataldo2014,
author = {Gonz{\'{a}}lez-Cataldo, Felipe and Wilson, Hugh F. and Militzer, Burkhard},
doi = {10.1088/0004-637X/787/1/79},
issn = {0004-637X},
journal = {The Astrophysical Journal},
keywords = {color figures,dynamical evolution and stability,individual,interiors,jupiter,online-only material,planets and satellites,saturn},
mendeley-groups = {Metallic H,SiO2 Solubility,Free Energy},
month = {may},
number = {1},
pages = {79},
title = {{Ab Initio Free Energy Calculations of the Solubility of Silica in Metallic Hydrogen and Application To Giant Planet Cores}},
url = {http://stacks.iop.org/0004-637X/787/i=1/a=79?key=crossref.8ed04244b9a9a55eefbe9b400819222b},
volume = {787},
year = {2014}
}

@article{Militzer2020,
author = {Militzer, Burkhard and Gonz{\'{a}}lez-Cataldo, Felipe and Zhang, Shuai and Whitley, Heather D and Swift, Damian C and Millot, Marius},
doi = {10.1063/5.0023232},
issn = {0021-9606},
journal = {The Journal of Chemical Physics},
month = {nov},
number = {18},
pages = {184101},
publisher = {AIP Publishing, LLC},
title = {{Nonideal mixing effects in warm dense matter studied with first-principles computer simulations}},
url = {https://doi.org/10.1063/5.0023232 http://aip.scitation.org/doi/10.1063/5.0023232},
volume = {153},
year = {2020}
}

@article{Gonzalez-Cataldo2020,
archivePrefix = {arXiv},
arxivId = {2008.08459},
author = {Gonz{\'{a}}lez-Cataldo, Felipe and Soubiran, Fran{\c{c}}ois and Militzer, Burkhard},
doi = {10.1063/5.0017555},
eprint = {2008.08459},
issn = {1070-664X},
journal = {Physics of Plasmas},
mendeley-groups = {PIMC},
month = {sep},
number = {9},
pages = {092706},
publisher = {AIP Publishing LLC},
title = {{Equation of state of hot, dense magnesium derived with first-principles computer simulations}},
url = {http://aip.scitation.org/doi/10.1063/5.0017555 http://arxiv.org/abs/2008.08459},
volume = {27},
year = {2020}
}


@article{Soubiran2019,
author = {Soubiran, Fran{\c{c}}ois and Gonz{\'{a}}lez-Cataldo, Felipe and Driver, Kevin P and Zhang, Shuai and Militzer, Burkhard},
doi = {10.1063/1.5126624},
issn = {0021-9606},
journal = {The Journal of Chemical Physics},
mendeley-groups = {MgO},
month = {dec},
number = {21},
pages = {214104},
publisher = {AIP Publishing, LLC},
title = {{Magnesium oxide at extreme temperatures and pressures studied with first-principles simulations}},
url = {https://doi.org/10.1063/1.5126624 http://aip.scitation.org/doi/10.1063/1.5126624},
volume = {151},
year = {2019}
}



@article{Gonzalez2020,
author = {Gonz{\'{a}}lez-Cataldo, Felipe and Soubiran, Fran{\c{c}}ois and Peterson, Henry and Militzer, Burkhard},
doi = {10.1103/PhysRevB.101.024107},
issn = {2469-9950},
journal = {Physical Review B},
mendeley-groups = {MgSiO3},
month = {jan},
number = {2},
pages = {024107},
title = {{Path integral Monte Carlo and density functional molecular dynamics simulations of warm dense MgSiO$_3$}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.101.024107},
volume = {101},
year = {2020}
}


@inproceedings{Gonzalez-Cataldo2018,
author = {Gonz{\'{a}}lez-Cataldo, Felipe and Corvacho, Fernando and Guti{\'{e}}rrez, Gonzalo},
booktitle = {Journal of Physics: Conference Series},
doi = {10.1088/1742-6596/1043/1/012038},
file = {:Users/fgonzalez/Library/Application Support/Mendeley Desktop/Downloaded/Gonz{\'{a}}lez-Cataldo, Corvacho, Guti{\'{e}}rrez - 2018 - Journal of Physics Conference Series.pdf:pdf},
issn = {1742-6588},
mendeley-groups = {LPMD,Melting Si},
month = {jun},
pages = {012038},
title = {{Melting curve of Si by means of the Z-method}},
url = {http://stacks.iop.org/1742-6596/1043/i=1/a=012038?key=crossref.9e5375dd24819db67a210b37d1a22de3},
volume = {1043},
year = {2018}
}



@Book{allen-tildesley-87,
   Author = {Allen, M.P. and Tildesley, D.J.},
   Title = {{Computer Simulation of Liquids}},
   Publisher = {Oxford: Clarendon Pr},
   Year = {1987}
}


@book{dfrenkel96:mc,
  abstract = {An advanced text on the physics and computation of
                  atomistic simulations. Chapter titles are:
                  introduction; statistical mechanics; Monte Carlo
                  simulations; molecular dynamics simulations; Monte
                  Carlo simulations in various ensembles; molecular
                  dynamics in various ensembles; free energy
                  calculations; the Gibbs ensemble; other methods to
                  study coexistence; free energies of solids; free
                  energy of chain molecules; long-range interactions;
                  biased Monte Carlo schemes; accelerating Monte Carlo
                  sampling; tackling time-scale problems; rare events;
                  dissipative particle dynamics. Appendices are
                  entitled: (the) Lagrangian and Hamiltonian;
                  non-Hamiltonian dynamics; linear response theory;
                  statistical errors; integration schemes; saving CPU
                  time; reference states; statistical mechanics of the
                  Gibbs ``ensemble''; overlapping distribution for
                  polymers; some general purpose algorithms; small
                  research projects; hints for programming.},
  added-at = {2013-03-21T02:24:53.000+0100},
  address = {San Diego},
  annote = {Series editors: D. Frenkel, M. Klein, M. Parrinello                  and B. Smit. First edition published in 1996.},
  author = {Frenkel, Daan and Smit, Berend},
  biburl = {https://www.bibsonomy.org/bibtex/27058bda2c1d06e4718bf4fe7a9e5b1d0/drmatusek},
  edition = {Second},
  interhash = {3e1272dc52ef1545e92ab3973adf0f18},
  intrahash = {7058bda2c1d06e4718bf4fe7a9e5b1d0},
  keywords = {Carlo Monte dynamics fortran mechanics molecular physics programming statistical},
  publisher = {Academic Press},
  series = {Computational Science Series},
  timestamp = {2013-03-21T02:24:54.000+0100},
  title = {Understanding Molecular Simulation: From Algorithms to
                  Applications},
  volume = 1,
  year = 2002
}


@article{Militzer2021,
  title = {First-principles equation of state database for warm dense matter computation},
  author = {Militzer, Burkhard and Gonz\'alez-Cataldo, Felipe and Zhang, Shuai and Driver, Kevin P. and Soubiran, Fran\ifmmode \mbox{\c{c}}\else \c{c}\fi{}ois},
  journal = {Phys. Rev. E},
  volume = {103},
  issue = {1},
  pages = {013203},
  numpages = {13},
  year = {2021},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.103.013203},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.103.013203}
}

@inproceedings{knudson2012megaamps,
  title={Megaamps, megagauss, and megabars: Using the Sandia Z Machine to perform extreme material dynamics experiments},
  author={Knudson, Marcus D},
  booktitle={AIP Conference Proceedings},
  volume={1426},
  pages={35--42},
  year={2012},
  organization={American Institute of Physics}
}

@article{Baskes1987a,
abstract = {The embedded-atom method, a semiempirical theory of metal bonding, is investigated as a method to calculate the bonding in a covalent material. A simple first-neighbor embedded-atom method model is sufficient to explain the geometry and structure of many metastable phases of silicon, but not its shear behavior. To obtain realistic shear behavior of silicon, an angle-dependent electron density is included to model the effects of bond bending. This model uses only the experimental bulk properties of silicon. Calculated properties of metastable phases and point defects are presented. {\textcopyright} 1987 The American Physical Society.},
author = {Baskes, M. I.},
doi = {10.1103/PhysRevLett.59.2666},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevLett.59.2666.pdf:pdf},
issn = {00319007},
journal = {Physical Review Letters},
number = {23},
pages = {2666--2669},
title = {{Application of the Embedded-Atom Method to Covalent Materials: A Semiempirical Potential for Silicon}},
volume = {59},
year = {1987}
}
@article{Baskes1989a,
abstract = {Semiempirical potentials for silicon, germanium, and their alloys are derived with use of the modified-embedded-atom-method formalism. Following Baskes [Phys. Rev. Lett. 59, 2666 (1987)], it is found that the host electron density which is a linear superposition of atomic densities in the embedded-atom method (EAM) must have an angular modification in order to properly describe the bond-bending forces in the diamond-cubic structure. The angular dependence of this host electron density was found to be in qualitative agreement with the density of a first-principles calculation. As in the EAM, the potential functions are determined by using the measured lattice constants, sublimation energies, elastic constants, and alloying energies of silicon and germanium. In addition, first-principles calculations of structural energies are used. The potentials are used to calculate the energetics and geometrics of point defects, surfaces, metastable structures, and small clusters. In all cases, the calculations have been compared to first-principles calculations and experiment when available. The calculations predict that the vacancy mechanism is the dominant diffusion mechanism in both silicon and germanium. Surface energies and relaxations of the low-index faces of Si and Ge are compared with first-principles calculations. {\textcopyright} 1989 The American Physical Society.},
author = {Baskes, M. I. and Nelson, J. S. and Wright, A. F.},
doi = {10.1103/PhysRevB.40.6085},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevB.40.6085.pdf:pdf},
issn = {01631829},
journal = {Physical Review B},
number = {9},
pages = {6085--6100},
title = {{Semiempirical modified embedded-atom potentials for silicon and germanium}},
volume = {40},
year = {1989}
}
@article{Baskes1992,
abstract = {In a comprehensive study, the modified embedded-atom method is extended to a variety of cubic materials and impurities. In this extension, all functions are analytic and computationally simple. The basic equations of the method are developed and applied to 26 elements: ten fcc, ten bcc, three diamond cubic, and three gaseous materials. The materials modeled include metals, semiconductors, and diatomic gases, all of which exhibit different types of bonding. Properties of these materials, including equation of state, elastic moduli, structural energies and lattice constants, simple defects, and surfaces, are calculated. The formalism for applying the method to combinations of these elements is developed and applied to the calculation of dilute heats of solution. In all cases, comparison is made to experiment or higher-level calculations when possible. {\textcopyright} 1992 The American Physical Society.},
author = {Baskes, M. I.},
doi = {10.1103/PhysRevB.46.2727},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/VirtualMelting/MEAM/PhysRevB.46.2727.pdf:pdf},
issn = {01631829},
journal = {Physical Review B},
number = {5},
pages = {2727--2742},
title = {{Modified embedded-atom potentials for cubic materials and impurities}},
volume = {46},
year = {1992}
}
@article{He2013,
abstract = {We perform large-scale molecular dynamics simulations to study shock-induced melting transition of idealized hexagonal columnar nanocrystalline Cu. The as-constructed nanocrystalline Cu consists of unrotated (reference) and rotated columnar crystals, relative to the columnar axis. Shock loading is applied along three principal directions of the columnar Cu: two transverse (zigzag and armchair) and one longitudinal directions. Dynamic local melting processes are highly anisotropic with respect to the shock directions. For the transverse directions, hotspot effect and disparate dynamic responses of grains with different orientations may lead to partial or complete premelting of the initially rotated grains, which in turn leads to transient supercooling and heterogeneous recrystallization, and thus, the formation of nanocrystalline solids with modified grain structures or solid-liquid mixtures, depending on the extent of supercooling. With increasing shock strengths, the reference grains melt heterogeneously at interfaces and homogeneously inside. Conversely, "bulk" premelting of the rotated grains is absent for the longitudinal direction, except for grain boundary melting. The progression of recrystallization or heterogenous melting diminishes and eventually eliminates the transient premelting or superheating of the system via latent heat and thermal diffusion. Premelting or superheating appears unlikely for bulk melting or well-defined Hugoniot states, if the thermal and mechanical equilibria are achieved, and the thermodynamic melting curve coincides with the partial melting Hugoniot states of a polycrystalline solid. {\textcopyright} 2013 AIP Publishing LLC.},
author = {He, A. M. and Duan, S. Q. and Shao, J. L. and Wang, P. and Luo, S. N.},
doi = {10.1063/1.4818336},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/VirtualMelting/1.4818336.pdf:pdf},
issn = {00219606},
journal = {Journal of Chemical Physics},
number = {7},
title = {{Local and bulk melting of shocked columnar nanocrystalline Cu: Dynamics, anisotropy, premelting, superheating, supercooling, and re-crystallization}},
volume = {139},
year = {2013}
}

@article{Budzevich2012,
author = {Budzevich, Mikalai M. and Zhakhovsky, Vasily V. and White, Carter T. and Oleynik, Ivan I.},
doi = {10.1103/PhysRevLett.109.125505},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/VirtualMelting/PhysRevLett.109.125505.pdf:pdf},
issn = {00319007},
journal = {Physical Review Letters},
number = {12},
pages = {1--5},
title = {{Evolution of shock-induced orientation-dependent metastable states in crystalline aluminum}},
volume = {109},
year = {2012}
}
@article{He2014,
abstract = {Solid-liquid phase transitions in single crystal Cu during shock and subsequent release are studied with large-scale classical molecular dynamics simulations. During shock compression, although the equilibrium states far behind shock front converge to the same Hugoniot, the pathways from metastable states right behind the shock front to the final equilibrium states and the resulting microstructures are orientation-dependent. Premelting is followed by recrystallization of supercooled melt into a polycrystalline solid for the [110] and [111] shocks, and a superheated, more ordered, solid is observed prior to shock melting for the [100] shock. The differences in the microstructure in the behind-shock region in turn give rise to different release melting behaviors (including premelting and superheating) along different release paths for these loading orientations. {\textcopyright} 2014 AIP Publishing LLC.},
author = {He, A. M. and Wang, P. and Shao, J. L. and Duan, S. Q. and Zhao, F. P. and Luo, S. N.},
doi = {10.1063/1.4871230},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/VirtualMelting/1.4871230.pdf:pdf},
issn = {10897550},
journal = {Journal of Applied Physics},
number = {14},
title = {{Solid-liquid phase transitions in single crystal Cu under shock and release conditions}},
volume = {115},
year = {2014}
}
@article{Levitas2012,
author = {Levitas, Valery I. and Ravelo, Ramon},
doi = {10.1073/pnas.1203285109},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/VirtualMelting/Font2015{\_}Article{\_}AMathematicalModelForNanoparti.pdf:pdf},
issn = {00278424},
journal = {Proceedings of the National Academy of Sciences of the United States of America},
keywords = {High strain-rate plasticity,Relaxation of non-hydrostatic stresses,Thermodynamics under uniaxial straining},
number = {33},
pages = {13204--13207},
title = {{Virtual melting as a new mechanism of stress relaxation under high strain rate loading}},
volume = {109},
year = {2012}
}
@article{Simak2000,
abstract = {A study was carried out to explore the structural competition between the high symmetry fcc and low symmetry bct structure for the IIIA metals Al, Ga, and In. It was found that the competition originates from electronic properties. As a result, the high pressure behavior of the metals appears reversed to the corresponding-states rule.},
author = {Simak, S. I. and H{\"{a}}ussermann, U. and Ahuja, R. and Lidin, S. and Johansson, B.},
doi = {10.1103/PhysRevLett.85.142},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/caratio/1.1698252-annotated.pdf:pdf},
issn = {00319007},
journal = {Physical Review Letters},
number = {1},
pages = {142--145},
title = {{Gallium and indium under high pressure}},
volume = {85},
year = {2000}
}
@article{Haussermann2001a,
abstract = {The origin of the (formula presented) variation in hcp divalent metals (Be, Mg, Zn, and Cd), which ranges from 1.568 to 1.886, has been investigated by first-principles full-potential calculations in the framework of the density functional theory. We find that the ideal hcp structure (formula presented) is electronically unstable to (formula presented) distortions for all elements, however the distortion driving band energy is countered by the electrostatic part of the total energy, which favors the ideal close packing. In particular, Zn and Cd with (formula presented) ratios (formula presented) ideal follow the bonding principle of optimum hybridization between s and p valence bands, a situation similar to the metallic elements in the neighboring group-IIIa in the Periodic Table. For Mg the electronic instability is not effective because the electrostatic part of the total energy dominates over the band energy. However, under expansion a distortion to (formula presented) ratios (formula presented) ideal occurs. Finally, Be represents a special case. Typically of second-row elements, s and p valence bands mix intimately which creates an electronic structure quite distinguished from the other divalent metals. A (formula presented) distortion cannot improve (formula presented) band hybridization but (formula presented) bonding is increased for (formula presented) ideal. {\textcopyright} 2001 The American Physical Society.},
author = {H{\"{a}}ussermann, U. and Simak, S. I.},
doi = {10.1103/PhysRevB.64.245114},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevB.64.245114.pdf:pdf},
issn = {1550235X},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {24},
pages = {1--10},
title = {{Origin of the (formula presented) variation in hexagonal close-packed divalent metals}},
volume = {64},
year = {2001}
}

@article{Pistorius1976,
author = {Pistorius, Carl W.F.T.},
doi = {10.1016/0079-6786(76)90012-1},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Exp/1-s2.0-0079678676900121-main.pdf:pdf},
issn = {00796786},
journal = {Progress in Solid State Chemistry},
number = {PART 1},
pages = {1--151},
title = {{Phase relations and structures of solids at high pressures}},
volume = {11},
year = {1976}
}


@inproceedings{mcmahan1982alpha,
  title={{The $\alpha$-$\beta$ transition in $T= O$ high pressure beryllium}},
  author={McMahan, AK},
  booktitle={AIP Conference Proceedings},
  volume={78},
  pages={340--344},
  year={1982},
  organization={American Institute of Physics}
}


@article{Meyer-Ter-Vehn1988,
abstract = {This paper is concerned with the effect of atomic-shell structure on the cold pressure of highly compressed matter up to 1 Gbar and above. The method is to compare band-structure calculations based on augmented spherical waves with results of the quantum-statistical model. Elements treated explicitly are Li, He, Be, Al, and K. No indication for anomalies due to pressure ionization is found. However, an oscillatory behavior of cold-pressure curves is systematically obtained due to isostructural electronic transitions. They are traced back to pressure-induced band shifts and electron redistribution from bands of low angular momentum (typically s and p waves) to bands of higher angular momentum (typically d and f waves). The shifts are shown to occur generally when squeezing normal matter with extended atoms into highly degenerate matter. The anomalies are particularly pronounced for alkali metals: Strong pressure flattening is found for Li at fivefold compression and 510 Mbar, and very sharply for K somewhat below fivefold compression and 500 kbar. The oscillations are much weaker for Be and Al. Metallization of He is obtained at 12.1 g/cm3 and 110 Mbar. For Be, a structural hcp bcc transition at 2 Mbar is predicted. {\textcopyright} 1988 The American Physical Society.},
author = {Meyer-Ter-Vehn, J. and Zittel, W.},
doi = {10.1103/PhysRevB.37.8674},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Theoretical Predictions/hybridisation/PhysRevB.37.8674.pdf:pdf},
issn = {01631829},
journal = {Physical Review B},
number = {15},
pages = {8674--8688},
title = {{Electronic structure of matter at high compression: Isostructural transitions and approach of the fermi-gas limit}},
volume = {37},
year = {1988}
}

@article{Lam1984,
abstract = {Beryllium is known to undergo a HCP-BCC transition at about 1530K and ambient pressure. This transition is studied theoretically by comparing the Gibbs free energies for the HCP, FCC and BCC modifications of Be. The static lattice energy is calculated using the ab initio pseudopotential method. The photon energy and entropy are estimated from the calculated elastic constants. A mechanism for this transition is proposed based on the results of the calculations. At high temperature, the BCC modification is found to be stabilised by the large entropy for this phase caused by the presence of soft phonon modes. Possible pressure-induced phase transitions are examined. At about 1-2 Mbar the FCC and BCC phases are both more stable than the HCP phase. The regions of FCC and BCC stability lie too close to be separated in the present calculation.},
author = {Lam, P. K. and Chou, M. Y. and Cohen, M. L.},
doi = {10.1088/0022-3719/17/12/006},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/P{\_}K{\_}Lam{\_}1984{\_}J.{\_}Phys.{\_}C{\_}{\_}Solid{\_}State{\_}Phys.{\_}17{\_}2065.pdf:pdf},
issn = {00223719},
journal = {Journal of Physics C: Solid State Physics},
number = {12},
pages = {2065--2073},
title = {{Temperature- and pressure-induced crystal phase transitions in Be}},
volume = {17},
year = {1984}
}
@article{francois1965conference,
  title={Conference Internationale sur la Metallurgie du Beryllium},
  author={Francois, M and Contre, M},
  journal={Universite de France, Grenoble, Paris},
  year={1965}
}
@techreport{abey1984pressure,
  title={Pressure phase lines and enthalpies for the. cap alpha.-. beta. and. beta.-liquid transitions in beryllium},
  author={Abey, Albert},
  year={1984},
  institution={Lawrence Livermore National Lab., CA (USA)}
}

@article{Olijnyk2000,
abstract = {Raman spectra of Be were studied at room temperature at pressures up to 23 GPa. The transverse-optical (TO) zone-centre phonon mode of hcp Be could be observed to maximum pressure. Neither new modes nor anomalies in the pressure shift were observed in the pressure range of 8.6-14.5 GPa where a phase transition has been reported. The TO mode frequency and its pressure dependence are discussed in terms of the elastic properties of Be.},
author = {Olijnyk, H. and Jephcoat, A. P.},
doi = {10.1088/0953-8984/12/41/317},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Exp/H{\_}Olijnyk{\_}2000{\_}J.{\_}Phys.{\_}{\_}Condens.{\_}Matter{\_}12{\_}8913.pdf:pdf},
issn = {09538984},
journal = {Journal of Physics Condensed Matter},
number = {41},
pages = {8913--8918},
title = {{Raman spectra of beryllium to 23 GPa}},
volume = {12},
year = {2000}
}
@article{kadas2007structural,
  title={Structural stability of $\beta$-beryllium},
  author={K{\'a}das, Krisztina and Vitos, Levente and Johansson, B{\"o}rje and Koll{\'a}r, J},
  journal={Physical Review B},
  volume={75},
  number={3},
  pages={035132},
  year={2007},
  publisher={APS}
}
@article{Peterson2014,
abstract = {Defects on inertial confinement fusion capsule surfaces can seed hydrodynamic instability growth and adversely affect capsule performance. The dynamics of shocks launched during the early period of x-ray driven National Ignition Facility (NIF) implosions determine whether perturbations will grow inward or outward at peak implosion velocity and final compression. In particular, the strength of the first shock, launched at the beginning of the laser pulse, plays an important role in determining Richtmyer-Meshkov (RM) oscillations on the ablation front. These surface oscillations can couple to the capsule interior through subsequent shocks before experiencing Rayleigh-Taylor (RT) growth. We compare radiation hydrodynamic simulations of NIF implosions to analytic theories of the ablative RM and RT instabilities to illustrate how early time laser strength can alter peak velocity growth. We develop a model that couples the RM and RT implosion phases and captures key features of full simulations. We also show how three key parameters can control the modal demarcation between outward and inward growth.},
author = {Peterson, J. L. and Clark, D. S. and Masse, L. P. and Suter, L. J.},
doi = {10.1063/1.4896708},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Application/1.4896708.pdf:pdf},
issn = {10897674},
journal = {Physics of Plasmas},
number = {9},
title = {{The effects of early time laser drive on hydrodynamic instability growth in National Ignition Facility implosions}},
url = {http://dx.doi.org/10.1063/1.4896708},
volume = {21},
year = {2014}
}
@article{Duff2015c,
abstract = {Thermodynamic properties of ZrC are calculated up to the melting point (Tmelt≈3700K), using density functional theory (DFT) to obtain the fully anharmonic vibrational contribution, and including electronic excitations. A significant improvement is found in comparison to results calculated within the quasiharmonic approximation. The calculated thermal expansion is in better agreement with experiment and the heat capacity reproduces rather closely a CALPHAD estimate. The calculations are presented as an application of a development of the upsampled thermodynamic integration using Langevin dynamics (UP-TILD) approach. This development, referred to here as two-stage upsampled thermodynamic integration using Langevin dynamics (TU-TILD), is the inclusion of tailored interatomic potentials to characterize an intermediate reference state of anharmonic vibrations on a two-stage path of thermodynamic integration between the original DFT quasiharmonic free energy and the fully anharmonic DFT free energy. This approach greatly accelerates the convergence of the calculation, giving a factor of improvement in efficiency of ∼50 in the present case compared to the original UP-TILD approach, and it can be applied to a wide range of materials.},
author = {Duff, Andrew Ian and Davey, Theresa and Korbmacher, Dominique and Glensk, Albert and Grabowski, Blazej and Neugebauer, J{\"{o}}rg and Finnis, Michael W.},
doi = {10.1103/PhysRevB.91.214311},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevB.91.214311.pdf:pdf},
issn = {1550235X},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {21},
pages = {1--8},
title = {{Improved method of calculating ab initio high-temperature thermodynamic properties with application to ZrC}},
volume = {91},
year = {2015}
}
@article{bzel1966physics,
  title={Physics of shock waves and high temperature hydrodinamic phenomena Academic Press},
  author={BZel’dovic, Ya and Raizer, Yu P},
  journal={New York},
  year={1966}
}
@article{Monserrat2013b,
abstract = {A unified approach is used to study vibrational properties of periodic systems with first-principles methods and including anharmonic effects. Our approach provides a theoretical basis for the determination of phonon-dependent quantities at finite temperatures. The low-energy portion of the Born-Oppenheimer energy surface is mapped and used to calculate the total vibrational energy including anharmonic effects, electron-phonon coupling, and the vibrational contribution to the stress tensor. We report results for the temperature dependence of the electronic band gap and the linear coefficient of thermal expansion of diamond, lithium hydride, and lithium deuteride.},
author = {Monserrat, Bartomeu and Drummond, N. D. and Needs, R. J.},
doi = {10.1103/PhysRevB.87.144302},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Monserrat, Drummond, Needs - 2013 - Anharmonic vibrational properties in periodic systems Energy, electron-phonon coupling, and stress.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {14},
pages = {1--10},
title = {{Anharmonic vibrational properties in periodic systems: Energy, electron-phonon coupling, and stress}},
volume = {87},
year = {2013}
}

@article{wallace1972thermodynamics,
  title={Thermodynamics of crystals},
  author={Wallace, Duane C},
  journal={American Journal of Physics},
  volume={40},
  number={11},
  pages={1718--1719},
  year={1972},
  publisher={American Association of Physics Teachers}
}
@article{rudindensity,
  title={Density Functional Theory Calculations on EOS and Phase Stability of Beryllium},
  author={Rudin, Sven P and Jones, MD and Johnson, JD},
  journal={Joint 20th AIRAPT--43th EHPRG, June}
}
@article{flyvbjerg1989error,
  title={Error estimates on averages of correlated data},
  author={Flyvbjerg, Henrik and Petersen, Henrik Gordon},
  journal={The Journal of Chemical Physics},
  volume={91},
  number={1},
  pages={461--466},
  year={1989},
  publisher={American Institute of Physics}
}
@article{Graf2004,
abstract = {The lattice vibrations are determined in the quasi-harmonic approximation for elemental Au and Cu to twice their normal density by first-principles electronic band-structure calculations. It is found for these materials that the important moments of the phonon density of states can be obtained to high accuracy from short-ranged force constant models. We discuss the implications for the Grueneisen parameters on the basis of calculated phonon moments and their approximations by using bulk moduli and Debye-Waller factors.},
author = {Graf, Matthias J.},
doi = {10.1063/1.1780185},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/GruneisenPhononMoment/1.1780185.pdf:pdf},
isbn = {0735401810},
number = {August 2004},
pages = {65--68},
title = {{High-Pressure Debye-Waller and Gr{\"{u}}neisen Parameters of Gold and Copper}},
volume = {65},
year = {2004}
}


@article{Navascues2010,
author = {Navascu{\'{e}}s, G. and Velasco, E.},
issn = {0021-9606},
journal = {The Journal of Chemical Physics},
mendeley-groups = {Free Energy},
month = {apr},
number = {13},
pages = {134106},
title = {{Free-energy correction due to center-of-mass constraint in crystals}},
url = {http://aip.scitation.org/doi/10.1063/1.3372805},
volume = {132},
year = {2010}
}



@article{anderson2000calculated,
  title={Calculated melting curves for phases of iron},
  author={Anderson, Orson L and Isaak, Donald G},
  journal={American Mineralogist},
  volume={85},
  number={2},
  pages={376--385},
  year={2000},
  publisher={Mineralogical Society of America}
}
@article{gilvarry1956lindemann,
  title={The Lindemann and Gr{\"u}neisen laws},
  author={Gilvarry, John James},
  journal={Physical Review},
  volume={102},
  number={2},
  pages={308},
  year={1956},
  publisher={APS}
}
@article{mermin1965thermal,
  title={Thermal properties of the inhomogeneous electron gas},
  author={Mermin, N David},
  journal={Physical Review},
  volume={137},
  number={5A},
  pages={A1441},
  year={1965},
  publisher={APS}
}
@article{baroni2001phonons,
  title={Phonons and related crystal properties from density-functional perturbation theory},
  author={Baroni, Stefano and De Gironcoli, Stefano and Dal Corso, Andrea and Giannozzi, Paolo},
  journal={Reviews of modern Physics},
  volume={73},
  number={2},
  pages={515},
  year={2001},
  publisher={APS}
}

@article{hellman2011lattice,
  title={Lattice dynamics of anharmonic solids from first principles},
  author={Hellman, Olle and Abrikosov, IA and Simak, SI},
  journal={Physical Review B},
  volume={84},
  number={18},
  pages={180301},
  year={2011},
  publisher={APS}
}


@article{Migliori2004c,
author = {Migliori, Albert and Ledbetter, Hassel and Thoma, D. J. and Darling, T. W.},
doi = {10.1063/1.1644633},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/Exp/1.1644633.pdf:pdf},
issn = {00218979},
journal = {Journal of Applied Physics},
number = {5},
pages = {2436--2440},
title = {{Beryllium's monocrystal and polycrystal elastic constants}},
volume = {95},
year = {2004}
}

@article{lyon1992sesame,
  title={Sesame: the Los Alamos National Laboratory equation of state database},
  author={Lyon, Stanford P},
  journal={Los Alamos National Laboratory report LA-UR-92-3407},
  year={1992}
}
@article{PhysRevLett.104.121101,
  title = {Sequestration of Noble Gases in Giant Planet Interiors},
  author = {Wilson, Hugh F. and Militzer, Burkhard},
  journal = {Phys. Rev. Lett.},
  volume = {104},
  issue = {12},
  pages = {121101},
  numpages = {4},
  year = {2010},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.104.121101},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.104.121101}
}
@article{Grabowski2009a,
abstract = {We propose a fully ab initio based integrated approach to determine the volume and temperature dependent free-energy surface of nonmagnetic crystalline solids up to the melting point. The approach is based on density-functional theory calculations with a controlled numerical accuracy of better than 1 meV/atom. It accounts for all relevant excitation mechanisms entering the free energy including electronic, quasiharmonic, anharmonic, and structural excitations such as vacancies. To achieve the desired accuracy of {\textless}1 meV/atom for the anharmonic free-energy contribution without losing the ability to perform these calculations on standard present-day computer platforms, we develop a numerically highly efficient technique: we propose a hierarchical scheme-called upsampled thermodynamic integration using Langevin dynamics-which allows for a significant reduction in the number of computationally expensive ab initio configurations compared to a standard molecular dynamics scheme. As for the vacancy contribution, concentration-dependent pressure effects had to be included to achieve the desired accuracy. Applying the integrated approach gives us direct access to the free-energy surface F (V,T) for aluminum and derived quantities such as the thermal expansion coefficient or the isobaric heat capacity and allows a direct comparison with experiment. A detailed analysis enables us to tackle the long-standing debate over which excitation mechanism (anharmonicity vs vacancies) is dominant close to the melting point. {\textcopyright} 2009 The American Physical Society.},
author = {Grabowski, B. and Ismer, L. and Hickel, T. and Neugebauer, J.},
doi = {10.1103/PhysRevB.79.134106},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/PhysRevB.79.134106.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {13},
pages = {1--16},
title = {{Ab initio up to the melting point: Anharmonicity and vacancies in aluminum}},
volume = {79},
year = {2009}
}

@article {phonopy,
     Journal = {Scr. Mater.},
     Year = {2015},
     Title = {First principles phonon calculations in materials science},
     Author = {Togo, A and Tanaka, I},
     Pages = {1--5},
     Volume = {108},
     Month = {Nov}
}
@article{sun2010lattice,
  title={Lattice thermal conductivity: Computations and theory of the high-temperature breakdown of the phonon-gas model},
  author={Sun, Tao and Allen, Philip B},
  journal={Physical Review B},
  volume={82},
  number={22},
  pages={224305},
  year={2010},
  publisher={APS}
}
@article{zhang2014phonon,
  title={Phonon quasiparticles and anharmonic free energy in complex systems},
  author={Zhang, Dong-Bo and Sun, Tao and Wentzcovitch, Renata M},
  journal={Physical review letters},
  volume={112},
  number={5},
  pages={058501},
  year={2014},
  publisher={APS}
}
@article{carreras2017dynaphopy,
  title={Dynaphopy: A code for extracting phonon quasiparticles from molecular dynamics simulations},
  author={Carreras, Abel and Togo, Atsushi and Tanaka, Isao},
  journal={Computer Physics Communications},
  volume={221},
  pages={221--234},
  year={2017},
  publisher={Elsevier}
}


@article{Musella2019,
abstract = {Using ab initio molecular dynamics simulations, we calculate the physical properties of MgO at conditions extending from the ones encountered in the Earth mantle up to the ones anticipated in giant planet interiors such as Jupiter. We pay particular attention to the high-pressure melting temperature throughout this large density range as this is a key ingredient for building accurate planetary interior models with a realistic description of their inner cores. We compare our simulation results with previous ab initio calculations that have been so far limited to the pressure range corresponding to the Earth mantle and the B1-B2 transition around 6 Mbar. We provide our results for both the equation of state and high-pressure melting curve in parametric forms for direct use in planetary models. Finally, we compare our predictions of the high-pressure melting temperature with various planetary interior profiles to deduce the state of differentiated layer within the core made of MgO in differentiated cores of various types of planets and exoplanets.},
archivePrefix = {arXiv},
arxivId = {1805.12439},
author = {Musella, R. and Mazevet, S. and Guyot, F.},
doi = {10.1103/PhysRevB.99.064110},
eprint = {1805.12439},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Core formation/MgO/PhysRevB.99.064110.pdf:pdf},
issn = {24699969},
journal = {Physical Review B},
keywords = {doi:10.1103/PhysRevB.99.064110 url:https://doi.org/10.1103/PhysRevB.99.064110},
number = {6},
pages = {1--8},
publisher = {American Physical Society},
title = {{Physical properties of MgO at deep planetary conditions}},
volume = {99},
year = {2019}
}

@article{Taniuchi2018,
abstract = {The melting curve of MgO is extended up to 4 TPa, corresponding to the Jovian core pressure, based on the one-step thermodynamic integration method implemented on ab initio molecular dynamics. The calculated melting temperatures are 3100 and 16 000 K at 0 and 500 GPa, respectively, which are consistent with previous experimental results, and 20 600 K at 3900 GPa, which is inconsistent with a recent experimental extrapolation, which implies the molten Jovian core. A quite small Clapeyron slope () of is found at 3900 GPa due to comparable densities of the liquid and B2 phases under extreme compression. The Mg-O coordination number in the liquid phase is saturated at around 7.5 above 1 TPa and remains smaller than that in the B2 phase (8) even at 4 TPa, suggesting no density crossover between liquid and crystal and thus no further denser crystalline phases. Dynamical properties (atomic diffusivity and viscosity) are also investigated along the melting curve to understand these behaviors in greater detail.},
author = {Taniuchi, Takashi and Tsuchiya, Taku},
doi = {10.1088/1361-648X/aaac96},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Core formation/MgO/Taniuchi{\_}2018{\_}J.{\_}Phys.{\_}{\_}Condens.{\_}Matter{\_}30{\_}114003.pdf:pdf},
issn = {1361648X},
journal = {Journal of Physics Condensed Matter},
keywords = {MgO,ab initio calculation,melting curve,thermodynamic integration},
number = {11},
pmid = {29393072},
publisher = {IOP Publishing},
title = {{The melting points of MgO up to 4 TPa predicted based on ab initio thermodynamic integration molecular dynamics}},
volume = {30},
year = {2018}
}


@book{german1996sintering,
  title={Sintering theory and practice},
  author={German, Randall M},
  year={1996}
}

@book{yefimov2009handbook,
  title={Handbook of non-ferrous metal powders: technologies and applications},
  author={Yefimov, NA},
  year={2009},
  publisher={Elsevier}
}
@article{Miyanishi2015,
abstract = {Magnesium oxide has been experimentally and computationally investigated in the warm-dense solid and liquid ranges from 200 GPa to 1 TPa along the principal Hugoniot. The linear approximation between shock velocity and particle velocity is validated up to a shock velocity of 15 km/s from the experimental data, this suggesting that the MgO B1 structure is stable up to the corresponding shock pressure of ∼350 GPa. Moreover, our Hugoniot data, combined with ab initio simulations, show two crossovers between MgO Hugoniot and the extrapolation of the linear approximation line, occurring at a shock pressures of approximately 350 and 650 GPa, with shock temperatures of 8000 and 14 000 K, respectively. These crossover regions are consistent with the solid-solid (B1-B2) and the solid-liquid (B2-melt) phase boundaries predicted by the ab initio calculations.},
author = {Miyanishi, K. and Tange, Y. and Ozaki, N. and Kimura, T. and Sano, T. and Sakawa, Y. and Tsuchiya, T. and Kodama, R.},
doi = {10.1103/PhysRevE.92.023103},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Core formation/MgO/PhysRevE.92.023103.pdf:pdf},
issn = {15502376},
journal = {Physical Review E - Statistical, Nonlinear, and Soft Matter Physics},
number = {2},
pages = {1--5},
title = {{Laser-shock compression of magnesium oxide in the warm-dense-matter regime}},
volume = {92},
year = {2015}
}
@article{Root2015,
abstract = {The moon-forming impact and the subsequent evolution of the proto-Earth is strongly dependent on the properties of materials at the extreme conditions generated by this violent collision. We examine the high pressure behavior of MgO, one of the dominant constituents in Earth's mantle, using high-precision, plate impact shock compression experiments performed on Sandia National Laboratories' Z Machine and extensive quantum calculations using density functional theory (DFT) and quantum Monte Carlo (QMC) methods. The combined data span from ambient conditions to 1.2 TPa and 42 000 K, showing solid-solid and solid-liquid phase boundaries. Furthermore our results indicate that under impact the solid and liquid phases coexist for more than 100 GPa, pushing complete melting to pressures in excess of 600 GPa. The high pressure required for complete shock melting has implications for a broad range of planetary collision events.},
author = {Root, Seth and Shulenburger, Luke and Lemke, Raymond W. and Dolan, Daniel H. and Mattsson, Thomas R. and Desjarlais, Michael P.},
doi = {10.1103/PhysRevLett.115.198501},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Core formation/MgO/PhysRevLett.115.198501.pdf:pdf},
issn = {10797114},
journal = {Physical Review Letters},
number = {19},
pages = {1--6},
title = {{Shock Response and Phase Transitions of MgO at Planetary Impact Conditions}},
volume = {115},
year = {2015}
}
@article{Cebulla2014,
abstract = {We determined the phase diagram of magnesium oxide with finite-temperature density functional theory molecular dynamics simulations up to temperatures and pressures as relevant for the deep interior of super-Earths and in rocky cores of giant planets such as Jupiter. The equation of state data, the Hugoniot, and a ramp compression curve are computed and compared to earlier results from diamond anvil cell and (decaying) shock wave experiments. In addition, the dynamical electrical conductivity and the reflectivity along the experimental Hugoniot curve are calculated in order to characterize electronic structure changes under compression. The structural properties of MgO are identified using pair correlation functions and self-diffusion coefficients. The solid-solid coexistence line is calculated by comparing the free enthalpies of the B1 and the B2 phase. The free energy of the solid phases is determined via thermodynamic relations using the ab initio simulation results and phonon calculations in the harmonic approximation. Our results indicate that the solid B2 phase of MgO does not occur in the interior of the Earth but may play an important role in super-Earths and in rocky planetary cores. {\textcopyright} 2014 American Physical Society.},
author = {Cebulla, Daniel and Redmer, Ronald},
doi = {10.1103/PhysRevB.89.134107},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Core formation/MgO/PhysRevB.89.134107.pdf:pdf},
issn = {1550235X},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {13},
pages = {1--10},
title = {{Ab initio simulations of MgO under extreme conditions}},
volume = {89},
year = {2014}
}
@article{Boates2013,
abstract = {The phase diagrams of MgSiO3 and MgO are studied from first-principles theory for pressures and temperatures up to 600 GPa and 20 000 K. Through the evaluation of finite-temperature Gibbs free energies, using density-functional theory within the generalized gradient approximation as well as with hybrid exchange-correlation functionals, we find evidence for a vast pressure-temperature regime where molten MgSiO3 decomposes into liquid SiO2 and solid MgO, with a volume change of approximately 1.2{\%}. The demixing transition is driven by the crystallization of MgO—the reaction only occurs below the high-pressure MgO melting curve. The predicted transition pressure at 10 000 K is in close proximity to an anomaly reported in recent laser-driven shock experiments of MgSiO3. We also present new results for the high-pressure melting curve of MgO and its B1-B2 solid phase transition, with a triple point at 364 GPa and 12 000 K.},
author = {Boates, Brian and Bonev, Stanimir A.},
doi = {10.1103/PhysRevLett.110.135504},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Boates, Bonev - 2013 - Demixing instability in dense molten MgSiO3and the phase diagram of MgO.pdf:pdf},
issn = {00319007},
journal = {Physical Review Letters},
number = {13},
pages = {1--5},
title = {{Demixing instability in dense molten MgSiO3and the phase diagram of MgO}},
volume = {110},
year = {2013}
}
@article{Belonoshko2010a,
abstract = {Recent laser-initiated strong shockwave measurements at Livermore provide the opportunity for verification of the MgO phase diagram at extreme pressures and temperatures. This calls for a comprehensive study of the MgO phase diagram. The phase diagram is obtained by ab initio molecular dynamics (two phase and Z method) and phonon-based thermodynamic calculations. Energies and forces are computed from first principles projector augmented wave method. The B1 transforms to B2 phase at about 490 GPa. Melting temperatures of B1 are consistent with the two-phase melting curve (Alfe, 2005). The triple point B1-B2-liquid is located at about 2.4 Mbar and 9000 K. The melting curve of the B2 phase rises rather steeply from the triple point. The Hugoniot is likely to cross the B1-B2 boundary first and then to cross the melting curve of B2, therefore, the melting curve of periclase is not relevant for the Hugoniot. MgO melts between 11.3 and 12.5 thousand K and 4.3 and 5 Mbar along the Hugoniot from the B2 phase. The two-phase melting curves of B1 computed with various semiempirical potentials are remarkably close to each other and are consistent with the B1 first principles melting curve at low pressure. This suggests the MgO melting temperatures to be in the close proximity of this determination. The search for new phases of MgO by first principles metadynamics has not produced unknown phases. Therefore, the suggested discontinuity of the Hugoniot at 170 GPa and 3000 K remains enigmatic.},
author = {Belonoshko, A. B. and Arapan, S. and Martonak, R. and Rosengren, A.},
doi = {10.1103/PhysRevB.81.054110},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Belonoshko et al. - 2010 - MgO phase diagram from first principles in a wide pressure-temperature range.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {5},
pages = {1--9},
title = {{MgO phase diagram from first principles in a wide pressure-temperature range}},
volume = {81},
year = {2010}
}
@article{Alfe2005a,
abstract = {We report diffusion Monte Carlo (DMC) calculations on MgO in the rock-salt and CsCl structures. The calculations are based on Hartree-Fock pseudopotentials, with the single-particle orbitals entering the correlated wave function being represented by a systematically convergeable cubic-spline basis. Systematic tests are presented on system-size errors using periodically repeating cells of up to over 600 atoms. The equilibrium lattice parameter of the rocksalt structure obtained within DMC is almost identical to the Hartree-Fock result, which is close to the experimental value. The DMC result for the bulk modulus is also in good agreement with the experimental value. The B1-B2 transition pressure (between the rocksalt and CsCl structures) is predicted to be just below 600 GPa, which is beyond the experimentally accessible range, in accord with other predictions based on Hartree-Fock and density functional theories. {\textcopyright} 2005 The American Physical Society.},
author = {Alf{\`{e}}, D. and Alfredsson, M. and Brodholt, J. and Gillan, M. J. and Towler, M. D. and Needs, R. J.},
doi = {10.1103/PhysRevB.72.014114},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Core formation/MgO/PhysRevB.72.014114.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {1},
pages = {1--7},
title = {{Quantum Monte Carlo calculations of the structural properties and the B1-B2 phase transition of MgO}},
volume = {72},
year = {2005}
}


@article{Militzer2013d,
author = {Militzer, Burkhard},
doi = {10.1016/j.hedp.2012.11.006},
issn = {15741818},
journal = {High Energy Density Physics},
keywords = {ab initio simulations,density functional molecular dynamics},
mendeley-groups = {MgSiO3},
month = {mar},
number = {1},
pages = {152--157},
publisher = {Elsevier Ltd},
title = {{Ab initio investigation of a possible liquid–liquid phase transition in MgSiO3 at megabar pressures}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S1574181812001322},
volume = {9},
year = {2013}
}

@article{Davies2020,
arxivId = {2002.00998},
author = {Davies, E. J. and Carter, P. J. and Root, S. and Kraus, R. G. and Spaulding, D. K. and Stewart, S. T. and Jacobsen, S. B.},
doi = {10.1029/2019JE006227},
eprint = {2002.00998},
file = {:Users/fgonzalez/Library/Application Support/Mendeley Desktop/Downloaded/2019JE006227.pdf:pdf},
issn = {21699100},
journal = {Journal of Geophysical Research: Planets},
keywords = {impacts,isentrope,melting,shock wave physics,thermodynamics,vaporization},
mendeley-groups = {Diamond},
number = {2},
pages = {1--17},
title = {{Silicate Melting and Vaporization During Rocky Planet Formation}},
volume = {125},
year = {2020}
}


@article{Swift2008,
  title={Shock formation and the ideal shape of ramp compression waves},
  author={Swift, Damian C and Kraus, Richard G and Loomis, Eric N and Hicks, Damien G and McNaney, James M and Johnson, Randall P},
  journal={Physical Review E},
  volume={78},
  number={6},
  pages={066115},
  year={2008},
  publisher={APS}
}
@article{desgranges2007controlling,
  title={Controlling polymorphism during the crystallization of an atomic fluid},
  author={Desgranges, Caroline and Delhommelle, Jerome},
  journal={Physical review letters},
  volume={98},
  number={23},
  pages={235502},
  year={2007},
  publisher={APS}
}
@article{sadigh2021metastable,
  title={Metastable--solid phase diagrams derived from polymorphic solidification kinetics},
  author={Sadigh, Babak and Zepeda-Ruiz, Luis and Belof, Jonathan L},
  journal={Proceedings of the National Academy of Sciences},
  volume={118},
  number={9},
  year={2021},
  publisher={National Acad Sciences}
}

@article{turnbull1950formation,
  title={Formation of crystal nuclei in liquid metals},
  author={Turnbull, D},
  journal={Journal of Applied Physics},
  volume={21},
  number={10},
  pages={1022--1028},
  year={1950},
  publisher={American Institute of Physics}
}

@article{Sun2018,
author = {Sun, Tao and Brodholt, John and Li, Yunguo and Vo{\v{c}}adlo, Lidunka},
doi = {10.1103/PhysRevB.98.224301},
issn = {2469-9950},
journal = {Physical Review B - Condensed Matter and Materials Physics},
mendeley-groups = {Melting Iron},
number = {22},
pages = {224301},
title = {{Melting properties from <i>ab initio</i> free energy calculations: Iron at the Earth's inner-core boundary}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.98.224301},
volume = {98},
year = {2018}
}
@article{sun2004crystal,
  title={Crystal-melt interfacial free energies in metals: fcc versus bcc},
  author={Sun, DY and Asta, M and Hoyt, JJ and Mendelev, MI and Srolovitz, DJ},
  journal={Physical Review B},
  volume={69},
  number={2},
  pages={020102},
  year={2004},
  publisher={APS}
}@article{Lazicki2012b,
abstract = {X-ray diffraction of beryllium in a laser-heated diamond anvil cell provides experimental insight into its behavior at high pressure and temperature. We measure the cold compression of Be in helium and NaCl pressure media up 192 GPa, and its thermal expansion up to 82 GPa and 2630 K. The new measurements form a P−V−T{\textless}math{\textgreater}{\textless}mrow{\textgreater}{\textless}mi{\textgreater}P{\textless}mo{\textgreater}-{\textless}mi{\textgreater}V{\textless}mo{\textgreater}-{\textless}mi{\textgreater}T data set which is fit by the Vinet-Debye form to establish a Be experimental equation of state. We compare the results to several theoretical models. The crystal structure of Be is determined up to 205 GPa and 4000 K; no evidence for the predicted high-temperature transition to a cubic phase is found. Finally, the maximum temperature stability of the solid phase along isobaric heating ramps gives a lower bound for the melting curve.},
author = {Lazicki, Amy and Dewaele, Agn{\`{e}}s and Loubeyre, Paul and Mezouar, Mohamed},
doi = {10.1103/PhysRevB.86.174118},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Lazicki et al. - 2012 - High-pressure-temperature phase diagram and the equation of state of beryllium.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {17},
pages = {1--10},
title = {{High-pressure-temperature phase diagram and the equation of state of beryllium}},
volume = {86},
year = {2012}
}
@article{Velisavljevic2002a,
abstract = {The structural and electrical properties of alkaline-earth metal beryllium were studied to 66 GPa using designer diamond anvils. The ambient pressure hexagonal close-packed phase was found to be stable to the highest pressure of 66 GPa and the measured static equation of state differs substantially from the one derived from the existing shock wave data. The electrical resistance data at high pressure shows a gradual decrease in resistance to pressure up to 25 GPa followed by a slight increase to 53 Gpa. The axial ratio (c/a) remains strongly nonideal with c/a = 1.562 at V/V 0  = 0.708, indicating that deviations from nearly free electron behavior are still dominant at high compressions.},
author = {Velisavljevic, Nenad and Chesnut, Gary N. and Vohra, Yogesh K. and Weir, Samuel T. and Malba, Vincent and Akella, Jagannadham},
doi = {10.1103/PhysRevB.65.172107},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Velisavljevic et al. - 2002 - Structural and electrical properties of beryllium metal to 66 GPa studied using designer diamond anvils.pdf:pdf},
issn = {01631829},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {17},
pages = {1721071--1721074},
title = {{Structural and electrical properties of beryllium metal to 66 GPa studied using designer diamond anvils}},
volume = {65},
year = {2002}
}
@article{Nakano2002b,
author = {Nakano, Kazutaka and Akahama, Yuichi and Kawamura, Haruki},
doi = {10.1088/0953-8984/14/44/334},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Nakano, Akahama, Kawamura - 2002 - X-ray diffraction study of Be to megabar pressure.pdf:pdf},
issn = {09538984},
journal = {Journal of Physics Condensed Matter},
number = {44 SPEC ISS.},
pages = {10569--10573},
title = {{X-ray diffraction study of Be to megabar pressure}},
volume = {14},
year = {2002}
}
@article{Evans2005a,
abstract = {We report combined x-ray and Raman studies of beryllium in helium and argon pressure media at pressures approaching 200 GPa. Our results are generally consistent with recent studies confirming the stability of the hexagonal close-packed phase to the highest pressures. However, the quasihydrostatic conditions of our studies lead to a stiffer equation of state (K0=109.88, K′0=3.59) and a gradual approach toward a more ideal c∕a ratio of 1.60 at 180 GPa. Combining our Raman and equation of state data, we are able to evaluate the pressure dependence of the elastic shear modulus (C44=109.3, C′44=1.959). We discuss the comparison of our results with measurements using ultrasonic and dynamic techniques.},
author = {Evans, W. J. and Lipp, M. J. and Cynn, H. and Yoo, C. S. and Somayazulu, M. and H{\"{a}}usermann, D. and Shen, G. and Prakapenka, V.},
doi = {10.1103/PhysRevB.72.094113},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Evans et al. - 2005 - X-ray diffraction and Raman studies of beryllium Static and elastic properties at high pressures.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {9},
pages = {1--6},
title = {{X-ray diffraction and Raman studies of beryllium: Static and elastic properties at high pressures}},
volume = {72},
year = {2005}
}
@article{Martin1959,
author = {Martin, A.J. and Moore, A.},
doi = {10.1016/0022-5088(59)90045-1},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Unknown - 1959 - to sudden changes in furnace voltage , and also served to cut down convection currents in the argon atmosphere . Heati.pdf:pdf},
issn = {00225088},
journal = {Journal of the Less Common Metals},
month = {apr},
number = {2},
pages = {85--93},
title = {{The structure of beryllium, with particular reference to temperatures above 1200°C}},
url = {https://linkinghub.elsevier.com/retrieve/pii/0022508859900451},
volume = {1},
year = {1959}
}
@article{Ming1984a,
abstract = {In situ high-pressure X-ray diffraction data for polycrystalline beryllium to 28.3 GPA at ambient temperature show that beryllium is transformed from the HCP phase (I) into a slightly distorted HCP phase (II) at pressures between 8.6 and 14.5 GPa. The volume change for the transition is extremely small ( approximately 0.4{\%}); the effect of pressure on the c/a ratio for both the Be(I) and Be(II) phases is also very small.},
author = {Ming, L. C. and Manghnani, M. H.},
doi = {10.1088/0305-4608/14/1/001},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/L{\_}C{\_}Ming{\_}1984{\_}J.{\_}Phys.{\_}F{\_}{\_}Met.{\_}Phys.{\_}14{\_}L1.pdf:pdf},
issn = {03054608},
journal = {Journal of Physics F: Metal Physics},
number = {1},
title = {{Isothermal compression and phase transition in beryllium to 28.3 GPa}},
volume = {14},
year = {1984}
}
@article{Lu2017b,
abstract = {Beryllium (Be) is an important material with wide applications ranging from aerospace components to x-ray equipment. Yet a precise understanding of its phase diagram remains elusive. We have investigated the phase stability of Be using a recently developed hybrid free energy computation method that accounts for anharmonic effects by invoking phonon quasiparticles. We find that the hcp → bcc transition occurs near the melting curve at 0 {\textless} P {\textless} 11 GPa with a positive Clapeyron slope of 41 ± 4 K / GPa , which is more consistent with recent experimental measurements. This work also demonstrates the validity of this theoretical framework based on the phonon quasiparticle to study the structural stability and phase transitions in strongly anharmonic materials.},
author = {Lu, Y. and Sun, T. and Zhang, Ping and Zhang, P. and Zhang, D. B. and Wentzcovitch, R. M.},
doi = {10.1103/PhysRevLett.118.145702},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Lu et al. - 2017 - Premelting hcp to bcc Transition in Beryllium.pdf:pdf},
issn = {10797114},
journal = {Physical Review Letters},
number = {14},
title = {{Premelting hcp to bcc Transition in Beryllium}},
url = {https://journals.aps.org/prl/pdf/10.1103/PhysRevLett.118.145702},
volume = {118},
year = {2017}
}
@article{Palanivel2000,
abstract = {High-pressure electronic properties of Be have been investigated theoretically be means of ab initio electronic structure calculations. The calculations have been carried out by the semi-relativistic full-potential, linear muffin-tin orbital (FPLMTO) method, within the local density approximation. The crystal structure stability among the hcp, bcc and orthorhombic (distorted hcp) phases has been studied as a function of compression. The bcc structure is found to be energetically stable at pressures above 180 GPa. From the results of our calculations, the orthorhombic phase cannot occur as an intermediate phase between the ambient pressure hcp phase and the high-pressure bcc structure. Our work thus suggests the need for more accurate high-pressure x-ray data.},
author = {Palanivel, B. and Rao, R. S. and Godwal, B. K. and Sikka, S. K.},
doi = {10.1088/0953-8984/12/41/309},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/Anharmonicity Beryllium/B{\_}Palanivel{\_}2000{\_}J.{\_}Phys.{\_}{\_}Condens.{\_}Matter{\_}12{\_}8831.pdf:pdf},
issn = {09538984},
journal = {Journal of Physics Condensed Matter},
number = {41},
pages = {8831--8836},
title = {{On the relative stability of orthorhombic and hcp phases of beryllium at high pressures}},
volume = {12},
year = {2000}
}
@article{Sinko2005a,
abstract = {Ab initio electronic-structure calculations, based on the density-functional theory and the full-potential linear-muffin-tin-orbital method, were used to predict crystal-sructure phase stabilities and elastic constants of beryllium under compression. Specific energies, pressures, elastic constants, and Debye temperatures for three crystal structures, hcp, bcc, and fcc, were calculated over a wide volume range. In agreement with experiments and previous theoretical calculations, the hcp ground state is obtained at ambient conditions and the bcc ground state is found at high pressure and ambient temperature, with the predicted hcp→bcc phase transition at about 2.7 Mbar. A possible phase diagram of beryllium, including hcp, bcc, and fcc phases is constructed in the (P,T) plane.},
author = {Sin'ko, G. V. and Smirnov, N. A.},
doi = {10.1103/PhysRevB.71.214108},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Sin'ko, Smirnov - 2005 - Relative stability and elastic properties of hcp, bcc, and fcc beryllium under pressure.pdf:pdf},
issn = {1098-0121},
journal = {Physical Review B},
month = {jun},
number = {21},
pages = {214108},
title = {{Relative stability and elastic properties of hcp, bcc, and fcc beryllium under pressure}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.71.214108},
volume = {71},
year = {2005}
}
@article{Robert2006a,
abstract = {The electronic and structural properties of beryllium were investigated under high pressure using first principle pseudopotential calculations within the generalized gradient approximation (GGA). Our results including pressures, elastic constants, Debye temperatures for two crystal structures ($\alpha$ hexagonal close packed and $\beta$ body-centred cubic) are compared with the experimental and other theoretical data over a wide density range. Calculated phonon spectra allow us to explain the anomalous behavior of the hcp-bcc transition under pressure. An equation of state (EOS) for the hep phase at finite temperatures is derived taking into account the anharmonicity effects of thermal lattice vibrations. The resulting 300 K isotherm and Hugoniot curve, as well as the evolution of the shear modulus under pressure and temperature, are in good agreement with available experimental and theoretical data. {\textcopyright} EDP Sciences.},
author = {Robert, G. and Sollier, A.},
doi = {10.1051/jp4:2006134039},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/jp4134039.pdf:pdf},
isbn = {2868839444},
issn = {11554339},
journal = {Journal De Physique. IV : JP},
pages = {257--262},
title = {{Equation of state and elastic properties of beryllium from first principles calculations}},
volume = {134},
year = {2006}
}
@article{Luo2012,
abstract = {We investigate the phase transition, elastic constants, phonon dispersion curves, and thermal properties of beryllium (Be) at high pressures and high temperatures using density functional theory. By comparing the Gibbs free energy, in the quasiharmonic approximation (QHA), of hexagonal-closed-packed (hcp) with those of the face-centered cubic (fcc) and body-centered-cubic (bcc) we find that the hcp Be is stable up to 390 GPa, and then transforms to the bcc Be. The calculated phonon dispersion curves are in excellent agreement with experiments. Under compression, the phonon dispersion curves of hcp Be do not show any anomaly or instability. At low pressure the phonon dispersion of bcc Be display imaginary along $\Omega$-N in the T 1 branches. Within the quasiharmonic approximation, we predict the thermal equation of state and other properties including the thermal expansion coefficient, Hugoniot curves, heat capacity, Gr{\"{u}}neisen parameter, and Debye temperature. {\textcopyright} 2012 American Institute of Physics.},
author = {Luo, Fen and Cai, Ling Cang and Chen, Xiang Rong and Jing, Fu Qian and Alf, Dario},
doi = {10.1063/1.3688344},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Luo et al. - 2012 - Ab initio calculation of lattice dynamics and thermodynamic properties of beryllium.pdf:pdf},
issn = {00218979},
journal = {Journal of Applied Physics},
number = {5},
title = {{Ab initio calculation of lattice dynamics and thermodynamic properties of beryllium}},
volume = {111},
year = {2012}
}
@article{Song2007,
abstract = {We extend the mean-field potential (MFP) approach for evaluating the vibrational contribution of the lattice ion of high-symmetry metals, and present a modified MFP approach which can be applied to low-symmetry or complex structure crystals. Based on the modified MFP approach in which the effect of the structural parameters on the free energy is taken into account, a first-principles scheme for calculating thermodynamic properties of a crystal dependent on the crystal structure is developed. By taking hexagonal close-packed beryllium as a prototype, we demonstrate that our scheme is suitable for investigating the structural properties and equation of state of low-symmetry crystals. {\textcopyright} 2007 The American Physical Society.},
author = {Song, Hai Feng and Liu, Hai Feng},
doi = {10.1103/PhysRevB.75.245126},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Song, Liu - 2007 - Modified mean-field potential approach to thermodynamic properties of a low-symmetry crystal Beryllium as a prototype.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {24},
pages = {1--7},
title = {{Modified mean-field potential approach to thermodynamic properties of a low-symmetry crystal: Beryllium as a prototype}},
volume = {75},
year = {2007}
}
@article{Benedict2009,
abstract = {We describe the construction of a three-phase equation of state for elemental beryllium. The phases considered are: the ambient hcp phase, the high-temperature bcc phase, and the liquid. The free energies of the solid phases are constructed from cold, ion-thermal, and electron-thermal components derived from ab initio electronic structure-based calculations. We find that the bcc phase is unstable near ambient conditions and that even at high pressures at which the bcc phase is stable, the bcc-hcp energy barrier can be as small as a few hundred kelvins. The liquid free energy is based on a model of Chisolm and Wallace and is constrained by using the melt curve (determined by ab initio two-phase simulations) as a reference. The high-temperature plasma limit is addressed with an average-atom-in-jellium model. Comparisons to experimental results, both for the ambient hcp phase and for the phase diagram as a whole, are discussed.},
author = {Benedict, Lorin X. and Ogitsu, Tadashi and Trave, Andrea and Wu, Christine J. and Sterne, Philip A. and Schwegler, Eric},
doi = {10.1103/PhysRevB.79.064106},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Benedict et al. - 2009 - Calculations of high-pressure properties of beryllium Construction of a multiphase equation of state.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {6},
pages = {1--9},
title = {{Calculations of high-pressure properties of beryllium: Construction of a multiphase equation of state}},
volume = {79},
year = {2009}
}
@article{Robert2010,
abstract = {Based on ab initio calculations, we provide a consistent modeling in pressure and temperature of the solid phases of beryllium, including theoretical phase diagram, multiphase equation of state (EOS), and elastic moduli. The quasiharmonic approximation (QHA) allows us to determine the whole theoretical phase diagram: at room temperature, QHA predicts the hexagonal compact ($\alpha$-hcp) phase as the most stable structure up to 400 GPa, where a transition toward the body-centered-cubic ($\beta$-bcc) phase occurs. However, the QHA does not account for the low-pressure-high-temperature bcc phase found experimentally. Combining frozen phonon and density-functional perturbation theory methods, we show that soft phonon modes as reservoirs of entropy may stabilize the low-pressure bcc phase. However the thermodynamic stability of this phase has still to be established. We provide the QHA multiphase EOS in analytic form and an evaluation of the uncertainties on the QHA solid-solid and solid-liquid phase boundaries. Then, we calculate the density and temperature dependence of elastic constants by determining the free energies of strained structures. Consistency between the polycrystalline (i.e., averaged over the elastic constants) and the EOS isothermal bulk moduli is achieved for both phases. Our results are in fair agreement with the most recent experimental data and permit us to raise questions on some experimental moduli.},
author = {Robert, G. and Legrand, P. and Bernard, S.},
doi = {10.1103/PhysRevB.82.104118},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Robert, Legrand, Bernard - 2010 - Multiphase equation of state and elastic moduli of solid beryllium from first principles.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {10},
title = {{Multiphase equation of state and elastic moduli of solid beryllium from first principles}},
url = {https://journals.aps.org/prb/pdf/10.1103/PhysRevB.82.104118},
volume = {82},
year = {2010}
}
@article{Xian2019b,
author = {Xian, Jia Wei and Yan, Jun and Liu, Hai Feng and Sun, Tao and Zhang, Gong Mu and Gao, Xing Yu and Song, Hai Feng},
doi = {10.1103/PhysRevB.99.064102},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Xian et al. - 2019 - Effect of anharmonicity on the hcp to bcc transition in beryllium at high-pressure and high-temperature conditions.pdf:pdf},
issn = {24699969},
journal = {Physical Review B},
keywords = {doi:10.1103/PhysRevB.99.064102 url:https://doi.org},
number = {6},
pages = {1--12},
publisher = {American Physical Society},
title = {{Effect of anharmonicity on the hcp to bcc transition in beryllium at high-pressure and high-temperature conditions}},
volume = {99},
year = {2019}
}
@article{Ming1984a,
abstract = {In situ high-pressure X-ray diffraction data for polycrystalline beryllium to 28.3 GPA at ambient temperature show that beryllium is transformed from the HCP phase (I) into a slightly distorted HCP phase (II) at pressures between 8.6 and 14.5 GPa. The volume change for the transition is extremely small ( approximately 0.4{\%}); the effect of pressure on the c/a ratio for both the Be(I) and Be(II) phases is also very small.},
author = {Ming, L. C. and Manghnani, M. H.},
doi = {10.1088/0305-4608/14/1/001},
file = {:Users/wjz8597/Documents/Mendeley{\_}Papers/L{\_}C{\_}Ming{\_}1984{\_}J.{\_}Phys.{\_}F{\_}{\_}Met.{\_}Phys.{\_}14{\_}L1.pdf:pdf},
issn = {03054608},
journal = {Journal of Physics F: Metal Physics},
number = {1},
title = {{Isothermal compression and phase transition in beryllium to 28.3 GPa}},
volume = {14},
year = {1984}
}
@article{Vijayakumar1984b,
abstract = {The metal beryllium (Be) has been studied under high pressure using an electrical resistivity technique with in situ pressure calibration. A sluggish phase transition at 12 GPa is observed which the authors identify as the HCP to distorted HCP phase transition reported in a recent high-pressure X-ray diffraction study. However, a reanalysis of the X-ray data on the high-pressure phase Be(II) indicates that a smaller orthorhombic cell with four atoms fits the observed interplanar spacings. The observed intensity ratios of the diffraction lines can be explained reasonably well on the basis of the space group P2 1 2 1 2 with four Be atoms occupying 4c positions.},
author = {Vijayakumar, V. and Godwal, B. K. and Vohra, Y. K. and Sikka, S. K. and Chidambaram, R.},
doi = {10.1088/0305-4608/14/5/002},
file = {:Users/wjz8597/Library/Application Support/Mendeley Desktop/Downloaded/Vijayakumar et al. - 1984 - On the high-pressure phase transition in beryllium metal.pdf:pdf},
issn = {03054608},
journal = {Journal of Physics F: Metal Physics},
number = {5},
title = {{On the high-pressure phase transition in beryllium metal}},
volume = {14},
year = {1984}
}

